Stopping Times of Boundaries: Relaxation and Continuity

We study the properties of the free boundaries and the corresponding hitting times in the context of optimal stopping in discrete time. We first prove the continuity of the map from the boundaries to the expected value of the corresponding stopping policy both in the supremum norm and also in a weaker, novel topology induced by the relaxed $L^\infty$ metric that we introduce. The latter is particularly useful when the optimal stopping boundary is only proved to be semicontinuous. Secondly, we study the connection between the hitting times, and their relaxations as widely employed in recent numerical methods. All these results together with the universal approximation capability of neural networks and the notion of inf/sup convolution are then used to provide a convergence analysis for the algorithm in [Reppen, Soner, and Tissot-Daguette, Neural Optimal Stopping Boundary, 2025] for the numerical resolution of the exercise regions arising in the analysis of Bermudan type option.

==> Approximation.tex <==
\section{Approximation of semicontinuous  Stopping Boundaries} \label{sec:lscBoundary} 




==> FBConv.tex <==
\section{Introduction}

 The  optimal stopping problem, given {in its} simplest form  by
\begin{equation}\label{eq:OS0}
  \sup \left\{ v(\tau) := \E^{\Q}[ \varphi(\tau,X_{\tau})] \ : \ \tau = \text{ stopping time}\right\},
\end{equation}
for a {stochastic} process $X $ and  
a reward function $\varphi$,  
plays a central role in stochastic  optimal control and has applications  
{in numerous quantitative fields}. 
{In mathematical statistics, the theory of optimal stopping 
can be utilized to address sequential tests, such as the quickest detection of a Wiener process} 
\cite{ShiryaevStat, PeskirShiryaev}. 
In mathematical finance, optimal stopping problems emerge naturally from 
the pricing of American or Bermudan contingent claims 
\cite{elKarouiPardouxQuenez,Karatzas,PeskirShiryaev,Schweizer}. 
In this context, $\varphi$ is  the payoff of the claim, $X$ describes 
the price evolution of the underlying asset, and the optimal value in 
\eqref{eq:OS0} gives the initial price of the contract. 
{While the initial} motivation of this paper is to provide 
a convergence study of the neural (optimal stopping) boundary
algorithm of  \cite{ReppenSonerTissotDF,ReppenSonerTissotFB},
{our analysis is essentially applicable to all scenarios 
where the exit times play a central role. Consequently,
we present our findings in this broader context, then
analyze the mentioned algorithm using these general results.}

{The unifying structure is the approximate parameterization of 
the \textit{stopping boundaries} 
by feedforward artificial neural networks,
and  the central question revolves around their asymptotic effectiveness.
In fact, the algorithm developed in \cite{ReppenSonerTissotFB}
computes the \textit{stopping} (or \textit{exercise}) \textit{region} 
for Bermudan options. 
Following \cite{ReppenSonerTissotFB},
we assume that in an appropriate coordinate system
the optimal stopping region is an epigraph (or a hypograph) 
of a function $f^{\diamond}$, and consequently, }
the hitting time of  $f^{\diamond}$ is  optimal for \eqref{eq:OS0}. 
Hence, we can restrict the set of stopping times in \eqref{eq:OS0} to hitting times of boundaries.
Namely,
\begin{equation}\label{eq:OS0f}
  \sup \left\{ v(\tau_f) := \E^{\Q}[ \varphi(\tau_f,X_{\tau_f})] \ : \ f = \text{ stopping boundary} \right\},
\end{equation}
where $\tau_f$ is the hitting time of the epigraph (or hypograph) of $f$.
{In the neural boundary algorithm, networks approximate $f^{\diamond}$,
and the convergence analysis of this method
relies mainly on the properties of the relaxation of the hitting times,
and the continuity of the map from the boundaries 
to the expected value of the corresponding stopping policy,
as proved in \cref{sec:relaxation,sec:continuity}, respectively.}

{It is well-known that, training with 
stochastic gradient descent of loss functions 
computed via hitting times results in vanishing gradient,
and as in the \textit{deep optimal stopping} of  \cite{Becker1,Becker2} and in \cite{ReppenSonerTissotFB},
relaxed stopping must be introduced.
Relegating the} 
technical details to \cref{sec:relaxation}, 
the relaxed version of problem \eqref{eq:OS0}  is given by,
\begin{equation}\label{eq:relax0}
    \sup\left\{ v(\mu) := \E^{\Q}\left[\int \varphi(t,X_{t}) \mu(dt) \right] \ : \ \mu =  \text{ random probability measure}\right\}.
\end{equation}

Also called \textit{convexification} \cite{Acikmese} or \textit{compactification}     
\cite{ElKaroui}, relaxation procedures such as \eqref{eq:relax0} are 
classically used in stochastic control problems to prove the existence of an optimal solution \cite{FlemingDomokos,Haussmann_Lepeltier,McShane}. 
Indeed, {relaxation convexifies the problem allowing 
for numerous methods and tools for its analysis. 
Moreover, as we prove in  \cref{prop:relaxOS},
both  \eqref{eq:OS0} and \eqref{eq:relax0} achieve the same optimal value. 
Indeed, this holds essentially in all other} contexts; 
see, e.g.,  \cite{Gyongy,Hobson} and \cite[Lemma 1.5.2.]{Krylov} 
for continuous time  optimal stopping, and 
\cite{ElKaroui,FlemingDomokos,Haussmann_Lepeltier} for general stochastic optimal control.  

In the neural optimal stopping boundary method,
the stopping policy is relaxed by introducing a \textit{fuzzy} region around the boundary
{with a small width  $\varepsilon>0$}. 
The stopping decision remains the same  outside the fuzzy region, while inside, 
the former is replaced by stopping intensities  proportional to the signed distance to the boundary. 
This procedure generates   \textit{relaxed} hitting times of boundaries$-$namely random  
probability measures supported  on the set of exercise dates. 
The relaxed problem \eqref{eq:relax0} thus becomes
\begin{equation}\label{eq:relax1}
\sup\left\{ v(\mu_f^\varepsilon) := \E^{\Q}\left[\int \varphi(t,X_{t}) 
{\mu_f^\varepsilon}(dt) \right] \ : \   {\mu_f^\varepsilon} =  \text{relaxed hitting time of $f$}\right\}.
\end{equation}
As shifting the boundary ever so slightly changes the stopping intensities inside the fuzzy region, the above relaxation makes stochastic gradient methods applicable. The fuzzy region is akin to the \textit{mushy zone} between two phases (typically solid and liquid) in phase-field models \cite{B-mushy,Soner,V-mushy}. The introduction of a  fuzzy  region is critical in other deep learning algorithms as well,  such as  occupation networks in  computer vision  \cite{OccupancyNN} or deep level-set functions for solving Stefan problems  \cite{SST}. 

{Our central results of continuity are proved in 
\cref{sec:continuity}}. In particular, \cref{thm:unifcontV,thm:lscV} establish the continuity
of the value functional $\frakF \ni f \mapsto v(\tau_f)$, 
where $\frakF$ is a set of stopping boundaries. 
{Formally, these results are
in the following form.}

\begin{theorem*}\label{thm:unifcontV0}
\textnormal{\textbf{(Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}} 
Let $\mathfrak{m}$ be a metric on $\frakF$. Then for all $\delta>0$, there exists $\iota  >0$ satisfying 
\begin{equation}\label{eq:unifcontV}
\forall f,f' \in \frakF \ \text{ such that } \  \mathfrak{m}( f,f') \le \iota \ \Longrightarrow   \ |v(\tau_{f}) - v(\tau_{f'})| \le \delta. 
\end{equation}
\end{theorem*}
\noindent
{Indeed, while \cref{thm:unifcontV} employs the supremum norm,
a weaker topology induced by the 
\textit{relaxed $L^{\infty}$ distance}  (see   \cref{def:relaxedSupDist})
is considered
in \cref{thm:lscV}
to accommodate  boundaries that are only semi-continuous}.
The relaxed $L^{\infty}$ distance  compares  boundaries $f,f'\in \frakF$  uniformly but after a transformation of the domain, 
as in the Skorokhod $J1$ distance  for càdlàg processes.
An immediate corollary, \cref{cor:relaxUnif}, 
is the convergence  of the value \eqref{eq:relax1}
associated to the relaxed stopping times
to the value using the same interface  as the width $\varepsilon$ of the fuzzy region tends to zero.   

 In \cref{sec:NOSB}, we combine the above results and provide a convergence 
 analysis of the \textit{neural optimal stopping boundary} algorithm \cite{ReppenSonerTissotFB}. 
Briefly, this algorithm looks for a \textit{neural stopping boundary}, 
namely a \textit{feedforward neural network} $g^{\theta}$   
such that 
$$
{v(\mu_{g^\theta}^\varepsilon)} \approx v(\tau_{g^{\theta}}) \approx \sup_{f\in \frakF}
v(\tau_f) \  = v(\tau_{f^{\diamond}}).
$$ 
The parameter vector $\theta$ is then trained by 
maximizing the relaxed reward $v(\mu_{g^\theta}^\varepsilon)$ using stochastic gradient ascent.  
{The following result  (also see \cref{thm:convCont}) implies
the  convergence of the algorithm employed in \cite{ReppenSonerTissotFB}.}
\begin{theorem*}\label{thm:convCont0} \textnormal{\textbf{(Convergence)}}
For all  $\delta>0$,  there exists $\varepsilon>0$ and a feedforward  
neural network  $g^{\theta}$ such that ${v(\mu_{g^{\theta}}^\varepsilon)}\ge v(\tau_{f^{\diamond}}) - \delta$. 
\end{theorem*}
\noindent
When the optimal stopping boundary $f^{\diamond}$ is continuous, 
one can apply the celebrated Universal Approximation 
Theorem \cite{Cybenko,Hornik} stating  that any continuous function can be 
approximated arbitrarily well by  feedforward neural networks in  compact sets. 
{This together} with the continuity of $f \mapsto v(\tau_f)$,
{implies the above result.}
{However}, the optimal stopping boundary $f^{\diamond}$ 
may fail to be continuous, preventing the use of the Universal Approximation Theorem. 
{Nevertheless,  under mild assumptions, the stopping boundary is  
shown to be semicontinuous in \cref{prop:lscBdry}.  
Motivated by this, we first extend in \cref{thm:LSCUAT} the Universal Approximation Theorem 
by proving that semicontinuous functions can be 
approximated by neural networks  in the 
relaxed $L^{\infty}$ distance introduced in  Definition \ref{def:relaxedSupDist}.
This is achieved through inf-sup convolutions
recalled in \cref{sec:convLSC}, 
which is an effective regularization 
tool widely used in the theory of viscosity solutions
(see, for example,  \cite[Section V.5]{FS} and \cite{LasryLions}).
This approximation together
with  \cref{thm:lscV} and the semicontinuity of $f^\diamond$
enables us to prove the above 
theorem. 
Incidentally, we suggest that the universal approximation
proved in \cref{thm:LSCUAT},}
is an interesting result in its own right 
and can be applied to other tasks  involving the approximation of  semicontinuous functions.

There is a recent body of literature on the convergence of deep learning methods in stochastic optimal control:  \citet{Hure} study the convergence  of discrete time stochastic control problems involving policy and/or value iteration; \citet{LapeyreLelong} prove the convergence of the Longstaff-Schwartz algorithm \cite{LSMC} using neural networks to approximate the continuation value; 
\citet{Gonon} sheds light on the expressivity and maximal size  of   neural networks to produce optimal stopping rules.  
{Additionally,}  \cite[Proposition 4]{Becker1} of the \textit{deep optimal stopping} paper 
 provies the near optimality of deep stopping strategies. 
 {A common property used in all these papers is dynamic programming,
 while} the neural optimal stopping boundary algorithm 
  \cite{ReppenSonerTissotFB} constructs an optimal stopping rule in a forward fashion.
  Consequently, our convergence analysis  necessitates 
  other techniques and tools, and differs greatly from previous works.  

\textbf{Structure of the paper.} In \cref{sec:OS}, we introduce the optimal stopping problem,  our main structural assumption on the exercise region, and give financial examples. In \cref{sec:relaxation}, we define the fuzzy region and construct relaxed stopping rules. \cref{sec:continuity} establishes the  continuity of the map $f\mapsto v(\tau_f)$ as well as important consequences. In \cref{sec:NOSB}, we prove the convergence of the neural optimal stopping boundary method in the continuous and semicontinuous case, respectively.  \cref{sec:conclusion} provides  concluding remarks and \cref{app:relaxedproblem} contains the proof of \cref{prop:relaxOS}. 



\section{Optimal stopping}\label{sec:OS}
 Let $\calT \subset [0,\infty)$  a  finite subset of  time indices containing $0$ and
$(\Omega, \F = (\calF_t)_{t \in \calT},\Q)$ a filtered probability space. 
The state $X = (X_t)_{t\in \calT}$
is an $\F$-adapted, Markov process which take values in a Euclidean space $\calX$. We assume for concreteness that $\F$ is the  filtration generated by $X$.
 Given a \emph{reward (or payoff) function} $\varphi:\calT \times \calX \to \R$,  the associated \emph{optimal stopping problem}  is to 
\begin{equation}
\label{eq:OS}
\text{maximize}
\ \ 
v(\tau):=  \E^{\Q}[ \varphi(\tau,X_{\tau})],
\qquad
\text{over}\  \tau \, \in \, \vartheta(\calT),
\end{equation} 
where 
$\vartheta(\calT)$ is the set of 
$\calT$-valued $\F$-stopping times.
Problem $\eqref{eq:OS}$ is well-defined (and non-trivial) if   $\max_{t\in \calT}|\varphi(t,X_t)| \in L^1(\Q)$. We write $v^{\diamond}$ for the optimal  value of \eqref{eq:OS}. %We write $\tau^{\diamond}$ for the optimal stopping time,  with  corresponding value  $v^{\diamond} = v(\tau^{\diamond})$. 
The following assumption on $\varphi$ and the dynamics of $X$ will prove useful.  

\begin{asm}%{\rm{\bf{(Growth and continuity)}}}
\label{asm:growth}
There exists $a>0$ 
such that 
$\varphi(t,\cdot) \in \calL_a \ \forall \ t \in \calT$, where 
\be
\label{e.lca}
\calL_{a}:= \left\{ \phi \in \calC(\calX;\R) \ : \ 
|\phi(x) | \le C[1+|x|^a]\ \
\text{for some}\ C>0 \right\}.
\ee
Moreover, $\phi \in \calL_a$ implies that 
$K_{t,s} \phi \in \calL_a$ $\forall \  t, s \in \calT$, $t<s$, with the transition semigroup
\begin{equation}\label{eq:semigroup}
    K_{t,s} \phi(x)=
\E[ \phi(X_{s}) \mid X_{t}=x], \quad x\in \calX.
\end{equation}

\end{asm}
Allowing the second component of  $K_{\cdot,\cdot}$  in \eqref{eq:semigroup} to be a stopping time,  
define  the value function  
\begin{equation}
    v^{\diamond}(t,x)= \sup_{t \le  \tau \in \vartheta(\calT )}
K_{t,\tau} \varphi(\cdot, x) \ , 
\end{equation}%\mathds{1}_{\{\tau\ge t\}}
and stopping region
$\calS_t = \{x\in \calX  :   \varphi(t,x) = v^{\diamond}(t,x)\}, \ t\in \calT. $
We then have the following result, proved in \cite{ReppenSonerTissotFB}. 
\begin{proposition}
\label{prop:closedStopRegion} Under Assumption \ref{asm:growth},
the value function $v(t,\cdot)$ belongs to $ \calL_a$ for each $ t\in \calT$. In particular, $v^{\diamond}(t,\cdot)$ is continuous and the stopping region $\calS_t$ is a relatively closed subset of $\calX$
.
\end{proposition}

Similar to   \cite{ReppenSonerTissotFB}, we make the following structural  assumption  %on the stopping region,
yielding the existence of a  \textit{stopping boundary} (or \textit{free boundary})   delimiting the stopping region in a problem specific coordinate system.

\begin{asm}%{\rm{\bf{(Existence of a stopping boundary)}}}
\label{asm:star}
There exist  measurable functions
$$
\alpha: \calX \to \R_+,
\quad
\Xi: \calX \to \calE := \Xi(\calX),
\quad
 f^{\diamond}: \calT \times \ \calE \to [0,\infty],
 $$
 % \begin{align*}
 % &\alpha: \calX \to \R_+, \\ 
 % &\Xi: \calX \to \calE := \Xi(\calX), \\ 
 %     &f^{\diamond}: \calT \times \ \calE \to [0,\infty],
 % \end{align*}
 such that $A = (\Xi,\alpha): \calX \to  \calE \times \R_+$ is a homeomorphism
 and for every $t \in \calT$,
\be
\label{e.st}
\calS_t = \{  x \in  \calX \ :\
\eta \left(f^{\diamond}(t,\Xi(x))-\alpha(x)\right) \le 0  \}, \qquad \eta \in \{-1,1\}. 
\ee 
\end{asm}
 Under the above assumption, the \textit{optimal stopping boundary} is thus given by 
\begin{align}\label{eq:stopBdry}
    f^{\diamond}(t,\xi) = \begin{cases} 
    \inf\{a \ge 0 \ : \ A^{-1}(\xi,a) \in \calS_t\}, & \eta = 1, \\[0.5em]
    \sup\{a \ge 0 \ : \ A^{-1}(\xi,a) \in \calS_t\}, & \eta = -1.
    \end{cases}
\end{align}
\begin{figure}[t]
\caption{Stopping region of a max-call option on two symmetric assets. The upper connected component becomes an epigraph through $(\alpha,\Xi)$.  Figures adapted from \cite{ReppenSonerTissotFB}.  } %\bb{OR MIN CALL}
\vspace{-2mm}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \caption{Stopping region in $\calX$}
    \includegraphics[height=2.0in,width=2.3in]{Figures/vizMaxCall.pdf}
    \label{fig:X}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \caption{Stopping region through $(\alpha,\Xi)$}
    \includegraphics[height=2.0in,width=2.3in]{Figures/vizMaxCallHomeo.pdf}
    \label{fig:homeo}
\end{subfigure}
\label{fig:homeomorphism}
\end{figure}  
\noindent
Consequently, the time $t$ section of the stopping region is the epigraph  of $f^{\diamond}(t,\cdot)$ when  $\eta =1$; see \cref{fig:homeomorphism}. Similarly, $\calS_t$ is the hypograph of $f^{\diamond}(t,\cdot)$ when $\eta =-1$. We refer the reader to \cite{BroadieDetemple} for further  information on the structure  of the stopping region and to \cite{Laurence} for a deep proof of the regularity of the boundary.  Additionally, classical books \cite{Velichkov,Petrosyan}  provide  a thorough treatment of the free boundary regularity in one-phase problems and respectively, in obstacle problems. 
For completeness, next we prove the following  simple properties  of $f^{\diamond}$. 
\begin{proposition} \label{prop:lscBdry}
    For every $t\in \calT$, the map $\xi \mapsto f^{\diamond}(t,\xi)$ is lower (respectively upper) semicontinuous when  $\eta =1$ (resp. $\eta = -1$). Moreover, if the payoff function $\varphi$ is convex in $x$, then $f^{\diamond}$ is locally Lipschitz continuous. % \bb{(convex if $\eta=1$ and concave if $\eta=-1$?).} 
\end{proposition}
\begin{proof}
   Fix $t\in \calT$ and prove the result for $\eta=1$. Similar arguments can be applied for the case   $\eta=-1$.  
    Let $\xi \in \calE$ and $(\xi_n) \subset \calE$ such that $\xi_n \to \xi$ and fix $\varepsilon >0$. In light of $\eqref{eq:stopBdry}$,    there exists $a_n \in \R_{+}$ such that $x_n := A^{-1}(\xi_n,a_n)\in \calS_t$ and $f^{\diamond}(t,\xi_n) \ge a_n - \varepsilon$ for every $n\in \N$.  Defining $a = \limsup_{n\to \infty} a_n,$ then %$\liminf_{n\to \infty} f^{\diamond}(t,\xi_n) \ge a - \varepsilon.$
    \begin{equation*}
        \liminf_{n\to \infty} f^{\diamond}(t,\xi_n) \ge a - \varepsilon. 
    \end{equation*}
    Next, the continuity of $A^{-1}$ yields  $\lim_{k\to \infty} x_{n_k} = x := A^{-1}(\xi,a) $ for a subsequence $(n_k)$ such that $a_{n_k} \to a$.  As $(x_{n_k}) \subset \calS_t$ and  $\calS_t$ is closed (see \cref{prop:closedStopRegion}), then  $x \in \calS_t$. Therefore $a \ge f^{\diamond}(t,\xi)$, giving  
    $\liminf_{n\to \infty} f^{\diamond}(t,\xi_n) \ge f^{\diamond}(t,\xi) - \varepsilon.$ 
   Letting $\varepsilon\to 0$ indeed shows the lower semicontinuity of  $\xi \mapsto f^{\diamond}(t,\xi)$. 
    
For the second assertion, it is shown in \cite{BroadieDetemple} that the convexity of  $x \mapsto \varphi(t,x)$ carries over to $\calS_t$.  In particular,  $f^{\diamond}$ is   locally Lipschitz continuous.
\end{proof}

In the remainder of the paper, 
to simplify the exposition we assume  that $\eta =1$, and the case $\eta = -1$ follows \emph{mutadis mutandis}.  The optimal stopping boundary $f^{\diamond}(t,\xi)$ is therefore  lower semicontinuous (l.s.c.)~in $\xi$ for all $t\in \calT$, and we set 
$$
\frakF := \{f:\calT \times \ \calE \to [0,\infty], \;  f(t,\cdot) \text{ l.s.c. } \forall t \ \in \calT\}.
$$ 
To each $f\in \frakF$, we associate the \emph{stopping region}
\begin{equation}
    \frakS_t(f) = \{x\in \calX \ : \ \alpha(x) \ge f(t,\Xi(x)) \},
\end{equation}
and  the \emph{hitting time}
$\tau_f = \inf\{t \in \calT  :  X_t \in \frakS_t(f)\}$.  Assumption \ref{asm:star} implies in particular that it is enough to consider hitting times of  boundaries to achieve the optimal value in  \eqref{eq:OS}. Namely,
$$
v^{\diamond} = \sup_{f\in \frakF}v(\tau_f)  = v(\tau_{f^{\diamond}}),
$$  
as already shown in \cite[Lemma 2.3]{ReppenSonerTissotFB}. Problem \eqref{eq:OS} is therefore  equivalent to finding $f\in \frakF$ such that $\frakS_t(f) = \calS_t$ for all $t \in \calT$. %Indeed, \cref{asm:star} guarantees the existence of an optimal  boundary 

\subsection{Financial examples}
Suppose that $X = (X^1,\ldots,X^m)$ describes the price process of $m\ge 2$ financial assets. The state space is  therefore  $\calX = \R^m_+$.   Moreover,  consider payoff functions of the form 
\begin{equation}
\varphi(t,x) = e^{-rt}(\alpha(x)-\kappa)^+,
\end{equation}
where $r\ge 0$ is a constant interest rate, $\kappa>0$ is the \textit{strike} of the option,  and $\alpha:\calX\to \R$ is a statistic of the underlying prices.  
For this class of contracts,    Assumption \ref{asm:star} holds  with  $\eta=1$, and the homeomorphism $A = (\Xi,\alpha)$,  $\Xi(x)=\frac{x}{\alpha(x)}$. See Theorem 4.1 in \cite{ReppenSonerTissotFB} for a  complete  statement. %The stopping region and its image through $(\alpha,\Xi)$ is displayed in \cref{fig:homeomorphism} for a max-call option (see \cref{ex:maxcall}) on $m=2$ symmetric assets. %Similarly, one can consider payoffs of the form $\varphi(t,x) = e^{-rt}(\kappa - \alpha(x))^+$ and apply the same homeomorphism. 

\begin{example}\label{ex:maxcall}
     Consider a \textit{max-call option}, which is obtained by choosing  $\alpha(x)  = \max_{i=1,...,m}x^i$. Hence $\varphi$ is convex in $x$, and \cref{prop:lscBdry} tells us that the stopping boundary is locally Lipschitz continuous.   Moreover, we have the latent space   $\calE =  \{\xi \in [0,1]^m  :  \max_{i=1,...,m}\xi_i=1  \}$; see  Assumption \ref{asm:star}. In particular, it is compact. Interestingly, the stopping region consists of $m$ connected components, as can be seen in \cref{fig:X} in the case of $m=2$ assets. The right panel (\cref{fig:homeo}) displays  the image through $(\alpha,\Xi)$ of the upper connected component of the stopping region in \cref{fig:X}. 
     
     Max-call options are popular benchmark examples for numerical methods addressing high-dimensional optimal stopping problems; see \cite[Section 8]{ReppenSonerTissotFB} and the references therein. Indeed,  the maximum function in the payoff makes the problem  truly high-dimensional in the sense that the process $\alpha(X)$ cannot be replaced by a one-dimensional diffusion with identical law. 
\end{example}

\begin{example} \label{ex:minmax} 

If $\alpha(x) = \min_{i=1,...,m}x^i$, then the associated contract is  a so-called \textit{min-call option}.  
Note that the payoff $\varphi(t,x)$ is \textit{not} convex in $x$, leading to pathological properties of the stopping region as  
 studied by \citet{DetempleMin} in the case $m=2$. In particular,   $\partial \calS_t$ contains a nonempty singular set, namely an isolated segment on the diagonal $\{x_1 = x_2\}$. 
Setting $\Xi(x) = \frac{x_1 \vee x_2}{x_1 \wedge x_2} \in \calE = [1,\infty)$ for simplicity, this implies that   $\calE \ni  \xi \to f^{\diamond}(t,\xi)$ is discontinuous at $\xi = 1$, hence strictly (lower) semicontinuous. % The lower semicontinuity of the stopping boundary  may therefore  be strict, even for seemingly simple examples. 
\end{example}

\section{Relaxed stopping rules}\label{sec:relaxation}

%Consequently, $v(\tau_{f^{\diamond}}) = v(\tau^{\diamond})  = v^{\diamond} $. % as well.  

To find an optimal boundary with stochastic gradient techniques as  in \cref{sec:NOSB}, the optimal stopping problem needs to be relaxed. Indeed, the map $f \mapsto \tau_f(\omega)$ is piecewise constant for $\Q$-almost every $\omega \in \Omega$ as the hitting time of $f$, taking values in the discrete set $\calT$,   is typically unchanged when  the stopping  boundary varies slightly. This in turn leads to severe vanishing gradient problems. We overcome this difficulty by approximating $\tau_f(\omega)$ by a sequence of relaxed  stopping rules based on \textit{fuzzy regions} parametrized by $\varepsilon>0$, 
\begin{equation}\label{eq:fuzzy1S}
\frakB_t^{\varepsilon}(f) := \frakS_t(f-\varepsilon) \setminus \frakS_t(f) = \{x\in \calX \ : \ d(t,x;f) \in (0, \varepsilon] \}, 
\end{equation}
where $d:\calT\times \calX \times \frakF \to [0,\infty]$ is the distance from $x$ to $\frakS_t(f)$ in the coordinate system $(\alpha,\Xi)$,
\begin{equation}\label{eq:distFct}
    d(t,x;f) =   (f(t,\Xi(x)) - \alpha(x))^{+}, \quad (t,x,f)\in \calT \times \calX \times \frakF,  
\end{equation} 
and an illustration is given in the left panel of \cref{fig:fuzzy&phaseIndicator}. 

We continue by first defining the general relaxed stopping rules, and then  the specific one induced by the fuzzy region. Let $\calP(\calT)$ be the set of probability measures on $\calT$ and $\underline{\vartheta}(\calT)$ denotes the set of $\calP(\calT)-$valued  random variables $$\mu(\omega) = \sum_{t\in \calT} P_t(\omega) \delta_t, \quad \omega \in \Omega, \qquad (\delta_t: \text{Dirac measure at $t$})$$ 
such that the process $(P_t)_{t\in \calT}$ is  $\F$-adapted. 
%such that the process $$t\mapsto \mu(\omega)(\calT_t), \quad  \calT_t := \calT \cap \ [0,t],$$ is  $\F$-adapted. %$ \omega \mapsto \mu(\omega)(\{t\})$ is $\calF_t-$measurable for all $t\in \calT$. 
In this context, $\underline{\vartheta}(\calT)$ is the set of \textit{relaxed} (or \textit{randomized}) $\F$-stopping times taking values in $\calT$. If we identify $\tau \in \vartheta(\calT)$ with %the Dirac measure 
$\delta_{\tau} \in \underline{\vartheta}(\calT)$, then   $\underline{\vartheta}(\calT)$ contains all  $\F$-stopping times. Indeed, this procedure is effectively  a \textit{convexification} of the stopping times as every relaxed stopping rule is  a random convex combination of the Dirac measures $(\delta_t)_{t\in \calT}$.  
We can now define the value functional
\begin{equation}\label{eq:relaxValue}
v(\mu) = \E^{\Q}\left[\int_{\calT} \varphi(t,X_{t}) \mu(dt) \right],\quad  \mu \in \underline{\vartheta}(\calT).
\end{equation}
%If $\mu = \sum_{t\in \calT} P_t \delta_t$, then \eqref{eq:relaxValue} reads 
%$$v(\mu) = \E^{\Q}\left[\sum_{t\in \calT} P_t \varphi(t,X_t) \right]. $$
The \emph{relaxed optimal stopping problem} amounts to maximizing $v(\mu)$ over all $\mu \in \underline{\vartheta}(\calT)$. 
Importantly,  the  relaxed  problem and classical one   \eqref{eq:OS} achieve the same optimal value as we prove in the next proposition. 
Similar results in continuous time can be found in \cite{Gyongy}, \cite{Hobson} and \cite[Lemma 1.5.2]{Krylov}. %, that is $\sup_{\mu \in \underline{\vartheta}(\calT)} v(\mu) = v^{\diamond}$. 

\begin{proposition}\label{prop:relaxOS}
Let $v^{\diamond}$ be the  value of the classical optimal stopping problem \eqref{eq:OS}. 
Then, 
\begin{equation}\label{eq:OSvsRelax}
      \sup_{\mu \in \underline{\vartheta}(\calT)} v(\mu)  = v^{\diamond}.
\end{equation}
 Moreover, any maximizer $\mu^{\diamond}$
 of $ \mu \mapsto v(\mu)$ is a  stopping time, i.e. $\mu^{\diamond} = \delta_{\tau^{\diamond}} $ for some $\tau^{\diamond} \in \vartheta(\calT)$. 
\end{proposition}
\begin{proof}
See \cref{app:relaxedproblem}.
\end{proof}
  
We next construct a relaxed stopping rule from a given boundary $f\in \frakF$ and a fuzziness parameter $\varepsilon>0$. Set $\calT_{t-} = \calT \cap \  [0,t)\ $ for $t>0$ and $\calT_{0-} = \varnothing$, and recursively define the $[0,1]-$valued  stochastic process $P^{\varepsilon}_f = (P_{f,t}^{\varepsilon})_{t\in \calT}$  representing  stopping probabilities by,
\begin{align}\label{eq:stopProb}
     P^{\varepsilon}_{f,t} = \underbrace{p_{f,t}^{\varepsilon}}_{\text{stop at $t$}} \ \ \underbrace{\Big(1- \sum_{s \in \calT_{t-}} P_{f,s}^{\varepsilon}  \Big)}_{\text{continue until $t$}}, \qquad 
     p_{f,t}^{\varepsilon} = (\chi^{\varepsilon}\circ d)(t,X_t;f), 
\end{align}
with the relaxed phase indicator function $\chi^{\varepsilon}(\delta) = (1 - \delta/\varepsilon)^+ \wedge 1$. 
Specifically, $\chi^{\varepsilon}$ is equal to one in the stopping region $\frakS_t(f)$, it is linearly decreasing in the fuzzy region $\frakB_t^{\varepsilon}(f)$, and is zero otherwise. The right panel of \cref{fig:fuzzy&phaseIndicator} displays the composition $\chi^{\varepsilon} \circ d$ in the space $\Xi(\calX) \times \alpha(\calX)$. 
We can now define the relaxed stopping rule associated to $f$ as 
\begin{equation}\label{eq:relaxedRule}
    \mu^{\varepsilon}_f(\omega) = \sum_{t\in \calT} P^{\varepsilon}_{f,t}(\omega) \  \delta_{t}. 
\end{equation}

\begin{figure}[t]
\caption{Left panel: fuzzy region (purple) separating the interior of the continuation region (blue) from the stopping region (red). Right panel: Illustration of $\chi^{\varepsilon} \circ d(\cdot; f)$ in the coordinates $(\Xi,\alpha)$, where $d(\cdot; f)$ is the distance function to $\frakS_t(f)$ and  $\chi^{\varepsilon}(\delta) = (1 - \delta/\varepsilon)^+ \wedge 1$.} 
\vspace{-1mm}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[height=2.0in,width=2.5in]{Figures/fuzzy_Bdry_Paper.pdf}
    \label{fig:fuzzybrdy}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
         \includegraphics[height = 2.0in,width = 2.5in]{Figures/fuzzy_3D_Paper.png}
     \label{fig:hFunction}
\end{subfigure}
\label{fig:fuzzy&phaseIndicator}
\end{figure}  
\noindent
Using \eqref{eq:stopProb}, we directly verify that $\mu_f^{\varepsilon}(\calT) = 1$. Additionally, as for each $t$, $P^{\varepsilon}_{f,t}$ depends only on $\{X_s \ : \ s \in \calT\cap \  [0,t] \}$, $P^{\varepsilon}_{f}$ is adapted to $\F$. Hence,  $\mu_f^{\varepsilon}$ is a relaxed $\F-$stopping time.

To complete the approximation, in \cref{cor:relaxUnif} we prove the following convergence which was already argued in \cite[Lemma B.1]{ReppenSonerTissotFB},
\begin{equation}\label{eq:relaxConv}
    v(\mu_{f}^{\varepsilon}) \longrightarrow v(\tau_{f}) \quad \text{as } \ \varepsilon \downarrow 0.
\end{equation}
That is, the value of the relaxed stopping rule  $\mu_f^{\varepsilon}$ converges to the expected reward  from  the hitting time of $f$ when the fuzzy parameter $\varepsilon$ decreases to zero. 

The above result is  a byproduct of the continuity of  $f\mapsto v(\tau_f)$, proved in the next section.   
Towards our main results \cref{thm:unifcontV,thm:lscV}, we start with a  
continuity lemma for relaxed stopping rules with respect to  
the \textit{total variation distance} of probability measures, 
$$  \textnormal{TV}(\mu,\mu') = \frac{1}{2}\sum_{t\in \calT} |\mu(\{t\}) - \mu'(\{t\})|\in [0,1], \qquad \mu, \mu' \in \calP(\calT).$$
Note that when  $\mu,\mu' \in \underline{\vartheta}(\calT)$, then  $\textnormal{TV}(\mu,\mu')$ is the random variable  $ \omega \mapsto \textnormal{TV}(\mu(\omega),\mu'(\omega))$. 
\begin{lemma}\label{lem:TV}
Under Assumption \ref{asm:growth}, there exists $C \in (0,\infty)$ depending on  $\varphi$ such that 
\begin{equation}
    |v(\mu)-v(\mu')| \le C \ \lVert \textnormal{TV}(\mu,\mu') \rVert_{L^2(\Q)}, \quad \forall \ \mu,\mu' \in \underline{\vartheta}(\calT). 
\end{equation}
In particular, 
$|v(\tau)-v(\tau')| \le C \Q(\tau \ne \tau')^{1/2}$  for any stopping times $\tau, \tau' \in  \vartheta(\calT)$.
\end{lemma}
\begin{proof}
      Define  $\Phi =  \sum_{t\in \calT} |\varphi(t,X_{t})| $ and  
      recall from Assumption \ref{asm:growth} that   $\varphi(t,\cdot) \in  \calL_a$ for some $a>0$. Since  $\phi 
    \in \calL_{a}$ implies $\phi^2 
    \in \calL_{2a}$, we obtain for some constant $C\in (0,\infty)$ that   
$$\E[\Phi^2] \le |\calT|  \sum_{t\in \calT} \E^{\Q}[\varphi(t,X_{t})^2] =   |\calT|  \sum_{t\in \calT} \underbrace{K_{0,t}\varphi^2(t,x_0)}_{\in \  \calL_{2a}} \le  C\sum_{t\in \calT}  [1+|x_0|^{2a}] < \infty. $$ 
Thus  $\Phi \in L^2(\Q)$. Next, observe that 
\begin{align*}
    |v(\mu) - v(\mu')| \le \E^{\Q}\left[  \int_0^T |\varphi(t,X_{t})|\  |\mu-\mu'|(dt) \right]
    \le 2 \E^{\Q}\left[  \Phi\  \text{TV}(\mu,\mu') \right].
\end{align*}
As $\text{TV}(\mu,\mu') \le 1 \in L^2(\Q)$, the result follows from the Cauchy-Schwarz inequality and  setting $C =  2 \lVert\Phi \rVert_{L^{2}(\Q)}$. For the second claim, it suffices to observe that  $\text{TV}(\delta_{\tau},\delta_{\tau'}) = \mathds{1}_{\{\tau \ne \tau'\}}$. 
\end{proof}

\begin{remark} Set $\overline{\textnormal{TV}}_2(\mu,\mu') := \lVert \textnormal{TV}(\mu,\mu') \lVert_{L^2(\Q)}$ for relaxed stopping rules $\mu,\mu' \in  \underline{\vartheta}(\calT)$. Then,  \cref{lem:TV} states that $ \mu \mapsto v(\mu)$ is Lipschitz continuous with respect to $\overline{\textnormal{TV}}_2$. 
\end{remark}

\section{Continuity of the value functional}\label{sec:continuity}
%and consequences
First, we need a distributional assumption on  the process  $\alpha(X) = (\alpha(X_t))_{t\in \calT}$. 
\begin{asm}\label{asm:absCont}
For every $t\in \calT$, the law of $\alpha(X_t)$ % $\Q(\alpha(X_t) \in \cdot )$ 
is absolutely continuous with respect to the Lebesgue measure  on $\R_+$. The cumulative distribution function $a \mapsto  \Q(\alpha(X_t)\in [0,a]) $ admits therefore a modulus of continuity $\rho_t:[0,\infty] \to [0,1]$. 
\end{asm}
We are now ready to  state our first  continuity result. Throughout, we adopt the notation $\calK \subset \subset \calE$ if $\calK$ is a compact subset of $\calE$. 
\begin{theorem}\label{thm:unifcontV}
\textnormal{\textbf{(Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}}
   Let  $C \in (0,\infty)$ given in \cref{lem:TV} and fix $\delta > 0$. Then under Assumptions \ref{asm:absCont},  
    there exists a compact set $\calK \subset \subset \calE$  such that for all $\iota >0$ and  $f,f'\in \frakF$, 
    \begin{equation}\label{eq:unifcontV}
        \lVert f - f' \rVert_{L^{\infty}(\calT \times \calK)}\le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho (\iota) + \delta},
    \end{equation}
    where $\rho_t$ is the modulus of continuity of $a \mapsto \Q(\alpha(X_t) \in [0,a] )$  and $\rho(\iota) = \sum_{t\in\calT} \rho_t(\iota) $. 
\end{theorem}

\begin{remark}\label{rem:bdedDensity}
If Assumption \ref{asm:absCont} holds and for all $t\in \calT$, 
 the density $\phi_t(x)dx := \Q(\alpha(X_t)\in dx)$  is  bounded,  then the cumulative distribution function of $\alpha(X_t)$ is Lipschitz continuous. In particular, its modulus of continuity satisfies $\rho_t(\iota) \le  \lVert \phi_t \rVert_{L^{\infty}(\R)} \iota$. Defining $c = \sum_{t\in \calT}\lVert \phi_t \rVert_{L^{\infty}(\R)}$, we can thus rewrite the right side of \eqref{eq:unifcontV} more explicitly   as 
    \begin{equation} \label{eq:valueLip}
        |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{c \ \iota + \delta}, 
    \end{equation}
   whenever $\lVert f - f' \rVert_{L^{\infty}(\calT \times \calK)}\le \iota$. 
\end{remark}

\begin{figure}[t]
    \centering
    \caption{Illustration of  
    the symmetric difference between the stopping regions $\frakS_t(f)$ and  $\frakS_t(f')$ (purple region) contained in the interval $[f \wedge f',f \wedge f'+\iota)$ (orange region); see proof of \cref{thm:unifcontV}. The stopping decisions with respect to $f$ and $f'$ coincide in the red (stop) and blue (continue) region. }
    \vspace{-1mm}
    \includegraphics[width = 2.7in,height = 2.0in]{Figures/Viz_Lemma_Paper.pdf}
    
    \label{fig:symdiff}
\end{figure}

\begin{proof} (\cref{thm:convCont}) \underline{\textit{Step ${1}$.}} 
 Since $\calE = \Xi(\calX)$   is locally compact (being the continuous image of a Euclidean space), 
 every finite Borel measure on it 
 is tight. 
Hence,  there exists $\calK \subset \subset \calE$ such that 
 \begin{equation}\label{eq:OmegaK}
   \Q(\Omega_{\calK}) \ge 1-\delta, \quad \Omega_{\calK} := \{\omega \in \Omega \ : \ \Xi(X_t(\omega)) \in \calK  \; \ \forall t\in \calT\}.
\end{equation} 
 \underline{\textit{Step ${2}$.}} Fix $\iota>0$ and $f,f'\in \frakF$ such that   $\lVert f - f' \rVert_{L^{\infty}(\calT \times \calK)}\le \iota$. Using \cref{lem:TV}, then 
$$|v(\tau_{f})-v(\tau_{f'})| \le C \Q(\tau_{f} \ne \tau_{f'})^{1/2},$$
so it remains to find the appropriate upper bound for $\Q(\tau_{f} \ne \tau_{f'})$.   
      First, note that the event $  \{\tau_{f} \ne \tau_{f'}\}$ is contained in   
      $$\tilde{\Omega} = \{\omega \in \Omega  : X_t(\omega) \in \frakS_t(f) \triangle \frakS_t(f')   \ \text{ for some } t\in \calT\}.  $$   
Indeed, for $\omega \notin \tilde{\Omega}$,
the sets $\{t \in \calT  :  X_t(\omega) \in  \frakS_t(f) \}$ and $\{t \in \calT  : X_t(\omega) \in  \frakS_t(f') \}$  are identical. Hence $\tau_{f}(\omega) = \tau_{f'}(\omega)$, which shows that $\Omega \setminus \tilde{\Omega} \subseteq \{\tau_f = \tau_{f'}\}$. 
Next, notice that 
\begin{align*}
     x &\in \frakS_t(f) \triangle \frakS_t(f')   \, \Longleftrightarrow \alpha(x) \in I_{f,f'}(t,\Xi(x)), \quad x \in \calX, 
\end{align*}
with the interval $I_{f,f'}(t,\xi) := [(f \wedge f')(t,\xi), (f \vee f')(t,\xi))$.   
Since $\lVert f - f' \rVert_{L^{\infty}(\calT \times \calK)}\le \iota$, then  
 $I_{f,f'}(t,\xi)$ has  length at most  $\iota$ %$|f(t,\xi)-f'(t,\xi)|  \le \iota$ 
 for every $(t,\xi) \in \calT \times \calK$. See \cref{fig:symdiff} for an illustration.   
Using Assumption \ref{asm:absCont} and recalling that 
$\rho_t$ is the modulus of continuity of $a \mapsto \Q(\alpha(X_t) \in [0,a] )$, then 
\begin{equation}\label{eq:absCont}
    \Q(\alpha(X_t) \in [a,a+\iota))   \le  \rho_t(\iota), \quad \forall a\in \R_+.
\end{equation}

We conclude from \eqref{eq:absCont} and 
the union bound  that 
\begin{align*}
    \Q( \tilde{\Omega} \cap   \Omega_{\calK})
    \le \sum_{t\in \calT} \Q(\{\alpha(X_t)\in \calI(t,\Xi(X_t))\} \cap \Omega_{\calK}  )
    \le \sum_{t\in \calT} \rho_t(\iota) 
    &=  \rho(\iota).
\end{align*}
Combining Step 1 with the above observations, we finally  obtain
\begin{equation*}
  \Q(\tau_{f} \ne  \tau_{f'}) \le   \Q(\{\tau_{f} \ne  \tau_{f'}\} \cap \Omega_{\calK})  + \Q(\Omega \setminus \Omega_{\calK}) \le  \Q( \tilde{\Omega} \cap   \Omega_{\calK})  + \delta 
    \le \rho(\iota) + \delta . 
\end{equation*}  
\end{proof} 

We have the following corollary of \cref{thm:unifcontV}, already stated in \eqref{eq:relaxConv}, proving the  convergence of the values obtained by the relaxed stopping rules to the strict ones. 
\begin{corollary}
    \label{cor:relaxUnif}
Under Assumptions \ref{asm:growth} and \ref{asm:absCont}, for all $\varepsilon >0$ and  $f\in \frakF$, 
    \begin{equation}\label{eq:relaxUnif}
   |v(\mu_{f}^{\varepsilon}) - v(\tau_{f})| \le C\sqrt{\rho (\varepsilon)} ,
\end{equation}
    with $\rho, C$ given in \cref{thm:unifcontV,lem:TV}, respectively. % and  $C \in (0,\infty)$ in \cref{lem:TV}.  
\end{corollary}

\begin{remark}
Under the additional assumption given in \cref{rem:bdedDensity}, equation  \eqref{eq:relaxUnif} becomes, 
    \begin{equation} \label{eq:relaxUnif2}
        |v(\mu_{f}^{\varepsilon}) - v(\tau_{f})| \le \tilde{C}\sqrt{\varepsilon}, 
    \end{equation}
    where $\tilde{C} = C c$ and $c$ defined in \cref{rem:bdedDensity}. We therefore obtain a rate of convergence equal to $1/2$ for the value associated to $\mu_f^{\varepsilon}$ as $\varepsilon \to 0$. 
    \end{remark}

 \begin{proof} (\cref{cor:relaxUnif}) 
  In view of \cref{lem:TV},  $|v(\mu_{f}^{\varepsilon}) - v(\tau_{f})| \le C  \| \textnormal{TV}(\mu_{f}^{\varepsilon},\delta_{\tau_f}) \lVert_{L^2(\Q)}.$ 
  Also by the definition of $\mu_{f}^{\varepsilon}$ in  \eqref{eq:relaxedRule} and the fact that  $\delta_{\tau_f}$ is a (random)  Dirac measure,  the total variation distance simplifies to 
\begin{align}
     \text{TV}(\mu_{f}^{\varepsilon},\delta_{\tau_f}) &= \frac{1}{2} \Big[ 1 - P_{f,\tau_{f}}^{\varepsilon} +  \sum_{t\in \calT\setminus\{\tau_{f}\}} P_{f,t}^{\varepsilon} \Big] = 1 - P_{f,\tau_{f}}^{\varepsilon} \le \mathds{1}_{\{\mu_{f}^{\varepsilon} \ \ne \ \delta_{\tau_{f}}\}} \quad \Q-\text{a.s.} 
\end{align}
     We now claim that  $\{\tau_{(f-\varepsilon)} = \tau_{f}\} \subseteq  \{\mu_{f}^{\varepsilon} = \delta_{\tau_{f}}\}$. Indeed,  if  $\tau_{(f-\varepsilon)}(\omega) = \tau_{f}(\omega)$,  the discrete path $(X_{t}(\omega))_{t\in \calT}$ never enters the fuzzy region  $\frakB_t^{\varepsilon}(f) = \frakS_t(f-\varepsilon) \setminus \frakS_t(f)$ prior to $\tau_f(\omega)$. Thus, the relaxed stopping rule 
     $\mu_f^{\varepsilon}(\omega)$ coincide with $\tau_f(\omega)$. Consequently, %we have 
     $$  
     \lVert \textnormal{TV}(\mu_{f}^{\varepsilon},\delta_{\tau_f}) \lVert_{L^2(\Q)}^2  \le \Q(  \mu_{f}^{\varepsilon} \ \ne \ \delta_{\tau_{f}}) \le   \Q(  \tau_{(f-\varepsilon)} \ne \tau_{f}  ). 
     $$
  We now follow Step 2 in the proof of \cref{thm:unifcontV}  with  $f' = f-\varepsilon$, $\iota =\varepsilon$ to conclude that  $\Q(  \tau_{f-\varepsilon} \ne \tau_{f}  ) \le \rho(\varepsilon)$. We note that as $\lVert f-f'\rVert_{L^{\infty}(\calT\times \calE)} = \varepsilon$, no localization is needed here as done in the proof of \cref{thm:unifcontV}.  
 \end{proof}

 \subsection{Relaxed $L^{\infty}$ distance and second continuity result} \label{sec:relaxLinfty}

The continuity result in \cref{thm:unifcontV} only applies when boundaries are close in the $L^{\infty}$ sense. Although reasonable for continuous boundaries, this condition is typically too restrictive for semicontinuous boundaries. We therefore introduce a weaker topology. 
   
\begin{definition}\label{def:relaxedSupDist} Given a compact set $\calK \subset \subset \calE$,  the \textit{relaxed $L^{\infty}$ distance} (in $\calK$)  is given by 
 \begin{equation} \label{eq:relaxDistH}
      {d}_{\calK}(h,h') = \sup_{r>0} \ \inf_{\psi \in \Psi_{r}^{\calK} }\ \lVert h\circ \psi -  h'\circ \psi \rVert_{L^\infty(\calK)}, \quad h,h': \calE\to \R,  
 \end{equation}
with the closed ball $\Psi_{r}^{\calK} = \{\psi: \calK \to \calK \ : \ \lVert \psi - \text{id} \rVert_{L^{\infty}(\calK) }\le r \}$ and identity map $\text{id}(\xi) = \xi$. For  $f,f'\in 
\frakF$, we define similarly %the \textit{space-time relaxed $L^{\infty}$ distance} as
\begin{equation}\label{eq:relaxDistF}
    d_{\calK,\calT}(f,f') = \max_{t \in \calT}  \ {d}_{\calK}(f(t,\cdot),f'(t,\cdot)). 
\end{equation}
\end{definition}
It is immediate that  $d_{\calK}$ is dominated by the $L^{\infty}$ metric. Strictly speaking, ${d}_{\calK}$ is not a distance, as neither the triangular inequality  nor the positivity axiom are satisfied. This is nevertheless a natural notion for  semicontinuous functions and closely related to the definition of \textit{inf convolutions} discussed in \cref{sec:convLSC}. Importantly, we prove in \cref{thm:lscV} that the space-time relaxed $L^{\infty}$ distance $d_{\calK,\calT}$ yields a continuity result  extending \cref{thm:unifcontV} to boundaries which are only lower semicontinuous. 

 In the above definition, transformations $\psi:\calK \to \calK$ echoes the  reparametrization maps appearing in the classical Skorokhod $J1$ distance for càdlàg processes. 
 On the other hand, a notable difference is that unlike the Skorokhod metric,  $\psi$ may not be invertible as we shall see in the proof of \cref{lem:infCovApprox}. 
 We finally stress that relaxed $L^{\infty}$ distance may be defined for general  subsets that are not necessarily compact. For our purposes, however, $d_{\calK}$ and $d_{\calK,\calT}$ will be exclusively used for compact sets, whence the assumption.  

We can now adapt \cref{thm:unifcontV} to obtain a continuity result of $f\mapsto v(\tau_f)$ with respect to  the relaxed $L^{\infty}$ distance. 

\begin{theorem}\label{thm:lscV}\textnormal{\textbf{(Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}}
   Let  $C \in (0,\infty)$ given in \cref{lem:TV} and fix $\delta > 0$. Then under Assumptions \ref{asm:absCont},  
    there exists 
 $\calK \subset \subset \calE$  such that for all $\iota >0$ and  $f, f'\in \frakF$, 
    $$d_{\calK,\calT}(f,f')\le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho (\iota) + \delta}, $$
    with $\rho(\iota) = \sum_{t\in\calT} \rho_t(\iota)$,  and  $(\rho_t)_{t\in \calT}$ the moduli of continuity of $(a \mapsto \Q(\alpha(X_t) \in [0,a] ))_{t\in \calT}$.   
\end{theorem}

\begin{proof}  Let $\delta'$ be arbitrary. As in Step 1 in the proof of  \cref{thm:unifcontV}, there exists   $\calK \subset \subset \calE$  such that 
 \begin{equation*}
   \Q(\Omega_{\calK}) \ge 1-\delta', \quad \Omega_{\calK} = \{\omega \in \Omega \ : \ \Xi(X_t(\omega)) \in \calK  \; \ \forall t\in \calT\}.
\end{equation*} 
       \underline{\textit{Step ${1}$.}} 
Let $f,f' \in \frakF$ such that $d_{\calK,\calT}(f,f')\le \iota$. From the definition of $d_{\calK,\calT}$,  we can construct   a sequence $\{\psi_k:\calT\times \calK\to \calK\}_{k\ge 1 }$ such that $
    |f(t,\psi_k(t,\xi)) - f'(t,\psi_k(t,\xi))|\le \iota$ for all $\xi \in \calK$ and $\psi_k(t,\cdot) \in \Psi_{1/k}^{\calK}$ $\forall \ t \in \calT$. 
In other words, 
\begin{align}
    &\lVert f\circ \psi_k -  f'\circ \psi_k  \rVert_{L^{\infty}(\calT \times \calK)} \le \iota, \quad  \ k\ge 1, \label{eq:unifPsi}\\[0.7em] 
     &\lVert \psi_k(t,\cdot) - \text{id} \rVert_{L^{\infty}(\calK)} \le 1/k, \qquad\forall \ t\in \calT. \qquad (\text{$\text{id}(\xi) = \xi$})\label{eq:psiId}
\end{align}
Next, let $\calX_{\calK}  = \{x \in \calX \ : \ \Xi(x) \in \calK\}$ %\Xi^{-1}(\calK)$ 
and  consider the transformations 
$$\phi_k: \calT \times \calX_{\calK} \to \calX_{\calK},\quad \phi_k(t,x) = A^{-1}(\alpha(x),\psi_k(t,\Xi(x))) , \quad k\ge 1. $$
In light of \eqref{eq:psiId}, observe that $\phi_k(t,x) \to A^{-1}(\alpha(x),\Xi(x)) = x$ pointwise in $\calX_{\calK}$  since $A^{-1}$ is continuous. Noting  that $\omega \in \Omega_{\calK}$ if and only if $X_t(\omega) \in \calX_{\calK}$,   
the bounded convergence theorem yields for every $B\in \calB(\calX)$,
\begin{equation}\label{eq:BCTPsi}
    \lim_{k\to \infty}\Q(\{\phi_k(t,X_t)\in B\}\cap \Omega_{\calK}) 
    = \Q(\{X_t\in B\}\cap \Omega_{\calK}), \quad \forall \ t \in \calT.
\end{equation}
Thus for fixed  $\gamma>0$ and $t\in \calT$, there exists $ k\ge 1$ such that 
\begin{equation}\label{eq:boundPsi}
  \Q(\{\phi_{k}(t,X_t)\in B\}\cap \Omega_{\calK}) \ge  \Q(\{X_t\in B\}\cap \Omega_{\calK}) - \gamma.
\end{equation}

 \underline{\textit{Step ${2}$.}} Recall that   
      $$\{\tau_{f} \ne \tau_{f'}\} \subseteq  \tilde{\Omega} = \{\omega \in \Omega  : X_t(\omega) \in \frakS_t(f) \triangle \frakS_t(f')   \ \text{ for some } t\in \calT\}.  $$      
Choosing $B = \frakS_t(f) \triangle \frakS_t(f')$ for each $t\in \calT$ and $\gamma = \frac{\delta'}{|\calT|}$ in \eqref{eq:boundPsi}, we have for $k$ large enough  that  
\begin{align}\label{eq:obs1}
    \Q(\tilde{\Omega}\cap \Omega_{\calK}) &\le \delta' + \sum_{t\in \calT} \Q(\{\phi_{k}(t,X_t) \in \frakS_t(f) \triangle \frakS_t(f') \}\cap \Omega_{\calK}).
\end{align}
Defining $I_{f,f'}(t,\xi) = [(f \wedge f')(t,\xi), (f \vee f')(t,\xi))$ as in the proof of \cref{thm:unifcontV}, observe that 
\begin{align*}
     \phi_k(t,x) &\in \frakS_t(f) \triangle \frakS_t(f')   \, \Longleftrightarrow \alpha(x) \in I_{f,f'}(t,\psi_k(t,\Xi(x))), \quad x \in \calX. 
\end{align*}
   Because of \eqref{eq:unifPsi},  $I_{f,f'}(t,\psi_k(t,\xi))$ has length at most $\iota$ for all $(t,\xi) \in \calT \times \calK$. Together with the absolute continuity of $\Q(\alpha(X_t) \in \cdot)$, this yields
\begin{equation}\label{eq:obs2}
    \sum_{t\in \calT} \Q(\{\phi_{k}(t,X_t) \in \frakS_t(f) \triangle \frakS_t(f') \}\cap \Omega_{\calK}) \le \sum_{t\in \calT}\rho_t(\iota) = \rho(\iota).
\end{equation}
From \eqref{eq:obs1},\eqref{eq:obs2}, and  the rationale in the proof of  \cref{thm:unifcontV}, we conclude with $\delta' = \frac{\delta}{2}$ that 
 $$|v(\tau_f)-v(\tau_{f'})|\le C\Q(\tau_f \ne \tau_{f'})^{1/2} \le C\left[\Q(\tilde{\Omega} \cap \Omega_{\calK}) + \delta'\right]^{1/2} \le C\sqrt{\rho(\iota)+ \delta}.$$
\end{proof}

\section{Application to neural  stopping boundaries} \label{sec:NOSB}

%\subsection{Universal Approximators and Stochastic Optimization}
%\label{sec:UAP_SO}
We apply the above results to study the convergence of the \textit{Neural Optimal Stopping Boundary method}   \cite{ReppenSonerTissotFB} which is now outlined. Under a suitable coordinate system  $(\alpha,\Xi)$ as in Assumption \ref{asm:star}, the algorithm looks for a \textit{neural stopping boundary}, namely a feedforward neural network $g^{\theta}: \calT \times \calE \to \R_+ $  in a (sufficiently large) hypothesis space $\frakN$ % = \{g^{\theta}: \calT \times \calE \to \R_+ \ : \ \theta \in \Theta\}$ 
such that $$v(\tau_{g^{\theta}}) \approx \sup_{f\in \frakF}
v(\tau_f) \  = v^{\diamond}.$$ %Because of this approximation  capability and available libraries such as Tensorflow and Pytorch to efficiently "train" the parameters, neural networks give a natural choice for $\frakN$. 
Additional details on the  architecture and  size of the neural networks 
for this problem are given in \cite{ReppenSonerTissotFB}.
The parameter vector $\theta$ is thereafter trained using stochastic gradient ascent. As explained at the beginning of \cref{sec:relaxation}, the  stopping rule needs to be relaxed to avoid vanishing gradient issues. 
For some fixed fuzzy region width $\varepsilon>0$, we therefore 
aim to 
\begin{equation}
\label{eq:OSNNRelax}
\text{maximize}
\ \ 
v(\mu_g^{\varepsilon}) =  \E^{\Q}\left[ \int_{\calT}\varphi(t,X_{t})\mu_g^{\varepsilon}(dt)\right]
\qquad
\text{over}\  g\in \frakN,
 %\sup_{g\in \frakN} v(\mu_g^{\varepsilon}), 
\end{equation} 
with the relaxed stopping rule $\mu_g^{\varepsilon}$ given in \eqref{eq:relaxedRule}.  
The vanishing gradient problem is henceforth resolved and owing to well-known convergence results in stochastic optimization \cite{RobbinsMonro,RobbinsSiegmund}, we can find for every $\gamma > 0$ %using stochastic gradient ascent 
an 
$\gamma-$\textit{maximizer} 
$g^{\varepsilon,\gamma} \in \frakN$, that is %  of the relaxed problem with fuzzy parameter $\varepsilon$, that is  
\begin{equation}\label{eq:fuzzytraining}
   v(\mu^{\varepsilon}_{g^{\varepsilon,\gamma}})\ge \sup_{g \in \frakN} \  v(\mu^{\varepsilon}_g) - \gamma.  
\end{equation} 
Finally, the value of the optimal stopping problem is computed using  the strict stopping rule $\tau_{g^{\varepsilon,\gamma}}$ instead of  $\mu^{\varepsilon}_{g^{\varepsilon,\gamma}}$. %$v(\tau_{g^{\varepsilon,\gamma}})$. 
The method is summarized in  \cref{alg:NOSB}. 
For further details, see Appendix C in \cite{ReppenSonerTissotFB}.  The goal of this section is to show that $
   v(\tau_{g^{\varepsilon,\gamma}})$ can be made arbitrarily close to the optimal value $ v^{\diamond} 
$ when   $\varepsilon, \gamma$ are small enough. 

\begin{remark}\label{rem:MC}
When computing the value associated to the trained stopping rule, say $\tau_{g}$,  an additional inaccuracy comes  from the Monte Carlo simulations of the process; see step III in \cref{alg:NOSB}. There is nevertheless a clear  control of this error.  Indeed, it is classical that 
$$|v(\tau_{g}) - \hat{v}_J(\tau_{g})| = \calO(J^{-1/2}),$$
 when the random reward $\varphi(\tau_{g},X_{\tau_{g}})$ is  square integrable. Under Assumption \ref{asm:absCont}, this is indeed the case (see also the proof of \cref{lem:TV}). 
   % In the analysis, we omit the Monte Carlo error when analyzing the convergence   of the trained boundary $v(\tau_{g^{\varepsilon,\gamma}})$  (see step III in \cref{alg:NOSB}). This is because 
\end{remark}


 
\begin{remark}
In \cite{ReppenSonerTissotFB},  a two-sided fuzzy region is considered, namely 
  $ \{ x\in \calX \ : \  |d(t,x;f)| < \varepsilon \},$ 
where $d(t,\cdot;f)$ is the  \textit{signed distance function} to  $\partial \frakS_t(f)$. 
Although the two representations are equivalent, one-sided fuzzy regions are  more practical towards a convergence analysis.
\end{remark}

\begin{algorithm}[t]
\caption{Neural Optimal Stopping Boundary Algorithm (summary) }\label{alg:NOSB}

\vspace{1mm}
\textbf{Given}: $\varphi=$ payoff, $ \calT =$ exercise dates, $\Theta=$ parameter set, $I =  \#$ training iterations,  $\zeta=$ learning rate process,  $\varepsilon=$ fuzzy region width, $B = $ batch size, $J= \#$ simulations for the value  \\[-0.8em]  \hrule

\begin{itemize}
 \setlength \itemsep{-0.1em}
\item[I.] \textbf{Initialize} $\theta_0 \in \Theta$
\item[II.] For $i = 0,\ldots,I-1$:
    \begin{enumerate}
    \setlength \itemsep{0.5em}
        \item \textbf{Simulate} $X(\omega_b) = \{X_t(\omega_b)\}_{t\in \calT}$, $\omega_b \in \Omega $, $b=1,\ldots, B$
        \item \textbf{Compute}  $ \hat{v}_B(\mu^{\varepsilon}_{g^{\theta_i}}) :=\frac{1}{B}\sum\limits_{b=1}^B \int_{\calT}  \varphi(t,X_{t}(\omega_b)) \ \mu^{\varepsilon}_{g^{\theta_i}}(\omega_b)(dt) $ % $ \hat{v}(\mu^{\varepsilon}_{g^{\theta_i}}) :=\frac{1}{B}\sum\limits_{j=1}^B \sum\limits_{t\in \calT} P_{g^{\theta_i},t}^{\varepsilon}(\omega_j) \ \varphi(t,X_{t}(\omega_j)) $
\item \textbf{Gradient step}: $\theta_{i+1} = \theta_{i} + \zeta_i \nabla_\theta \hat{v}_B(\mu^{\varepsilon}_{g^{\theta_i}}) $
   \end{enumerate}
\item[III.] \textbf{Return} $g = g^{\theta_{I}}$ and $\hat{v}_J(\tau_{g}) := \frac{1}{J}\sum\limits_{j=1}^J \varphi(\tau_{g}(\omega_j),X_{\tau_{g}}(\omega_j)), \  \omega_j \in \Omega $, $\ j=1,\ldots, J$
\end{itemize}
\vspace{-3mm}
\end{algorithm}

\subsection{Convergence analysis: continuous boundaries}

We first outline our strategy to prove convergence of the Neural Optimal Stopping Boundary method when the optimal stopping boundary $f^{\diamond}$ is continuous. First, the hypothesis space $\frakN$ (neural networks in this case) must satisfy a universal approximation property; see Assumption \ref{asm:UAP} below. Thus, there exists $g^{\diamond} \in \frakN$ arbitrarily close to $f^{\diamond}$ in compact sets. We can  therefore invoke our first continuity result  (\cref{thm:unifcontV}) to ensure that the values of the stopping strategies $\tau_{f^{\diamond}}$, $\tau_{g^{\diamond}}$ are close as well. Next, we relax the problem and use \cref{cor:relaxUnif}  to guarantee that $v(\mu^{\varepsilon}_{g^{\diamond}}) \approx  v(\tau_{g^{\diamond}})$ for small fuzzy parameter $\varepsilon$. We then train the neural boundary  %from classical results in stochastic optimization \cite{RobbinsMonro,RobbinsSiegmund} 
to construct $g^{\varepsilon,\gamma} \in \frakN$ such that $v(\mu^{\varepsilon}_{g^{\diamond}}) \approx v(\mu^{\varepsilon}_{g^{\varepsilon,\gamma}})$ and finally  conclude that $v(\mu_{g^{\varepsilon,\gamma}}^{\varepsilon}) \approx  v(\tau_{g^{\varepsilon,\gamma}})$  in view of   \cref{cor:relaxUnif}.  The above steps can be summarized as follows: %in the following sequence:
\begin{align*}
    v^{\diamond} &= v(\tau_{f^{\diamond}}) && \\  
&\approx v(\tau_{g^{\diamond}}) && \longleftarrow \ \textnormal{approximation and continuity (Assumption \ref{asm:UAP} and \cref{thm:unifcontV})}\\ 
&\approx  v(\mu_{g^{\diamond}}^{\varepsilon}) && \longleftarrow \ \textnormal{relaxation (\cref{cor:relaxUnif})} \\ 
&\approx  v(\mu_{g^{\varepsilon,\gamma}}^{\varepsilon}) && \longleftarrow \ \textnormal{stochastic optimization  \cite{RobbinsMonro,RobbinsSiegmund}} \\ 
&\approx v(\tau_{g^{\varepsilon,\gamma}}). && \longleftarrow \ \textnormal{relaxation (\cref{cor:relaxUnif})}
\end{align*}
We start with the approximation of $f^{\diamond}$. Let $\frakF_c  = \{f \in \frakF :  f(t,\cdot) \in \calC(\calE) \; \forall t\in \calT\}$ denotes the set of continuous boundaries and consider  a  hypothesis space $\frakN \subset \frakF_c$ satisfying the following assumption which can be seen as the \textit{universal approximation property}. 
\begin{asm}\label{asm:UAP}
For all 
$f\in \frakF_c$, compact set  $\calK \subset \subset \calE$  and $\iota >0$, there exists  $g\in \frakN$ such that  
\begin{equation}\label{eq:UAP}
    \lVert f - g \rVert_{L^{\infty}(\calT \times \calK )} \le \iota. 
\end{equation}
\end{asm}

We refer to elements in a family $\frakN \subset \frakF_c$ such that 
Assumption \ref{asm:UAP} holds as \textit{universal approximators}. The Stone-Weierstrass theorem gives an example of  universal approximators, namely the polynomials. This class, however, is  numerically unsuitable when the Hausdorff dimension of $\calE$ becomes large. In our case, $\frakN$ is evidently the family of all feedforward neural networks $g^\theta:\calT\times \  \calE \to \R_+$ with finite-dimensional parameter vector $\theta$. %s $\theta \in \R^{p}$ for some $p\in \N$. 
Assumption \ref{asm:UAP} follows classically from the 
 Universal Approximation Theorem (UAT) for neural networks \cite{Cybenko,Hornik}. 
 %Importantly, neural networks do not suffer much from the  curse of dimensionality; see, e.g., \cite{Gonon}. 

% If the optimal boundary $f^{\diamond}$ belongs to $\frakF_c$, we can  invoke the universal approximation property of $\frakN$ giving the existence of $g^{\diamond}$ arbitrarily close to $f^{\diamond}$ in some compact set. 
% This is no longer the case when $f^{\diamond}$ is  strictly lower semicontinuous; a remedy will be given in \cref{sec:lscBoundary}. 
In this section, we assume that $f^{\diamond}(t,\xi)$ is  continuous in $\xi$, i.e. $f^{\diamond} \in \frakF_c$. We can therefore directly use $f^{\diamond}$ in Assumption \ref{asm:UAP}. Together with the results from \cref{sec:continuity}, the next convergence theorem follows naturally. 
\begin{theorem}\label{thm:convCont}
   Consider $\frakN \subset \frakF_c$  satisfying Assumption \ref{asm:UAP}, $f^{\diamond}\in \frakF_c$, and suppose that Assumption  \ref{asm:absCont} holds.  Then, for every $\delta >0$,   there exists $\varepsilon=\varepsilon(\delta), \gamma=\gamma(\delta)>0$  such that any $g^{\varepsilon,\gamma} \in \frakN$ with the property $ v(\mu^{\varepsilon}_{g^{\varepsilon,\gamma}}) \ge \underset{g \in   \frakN}{\sup} \  v(\mu^{\varepsilon}_g) - \gamma$ also satisfies,
   \begin{equation}\label{eq:UpperBound}
    v(\tau_{g^{\varepsilon,\gamma}})\ge v^{\diamond} - \delta.  
\end{equation} 
\end{theorem}

\begin{proof} \underline{\textit{Step ${1}$.}}  Let $\delta'>0 $ be arbitrary. From  \cref{thm:unifcontV}, there exist $\delta''>0$, $\calK\subseteq \calE$ compact,  and $\iota>0$ such that
\begin{equation}\label{eq:contV}
    \lVert f - f' \rVert_{L^{\infty}(\calT \times \calK)}\le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho(\iota) + \delta''}\le \delta'. 
\end{equation}
Invoking Assumption \ref{asm:UAP}, there exists   $g^{\diamond} \in \frakN$ such that 
$\lVert f^{\diamond} - g^{\diamond} \rVert_{L^{\infty}(\calT \times \calK)}\le \iota. $
We conclude  from \cref{thm:unifcontV}  that $v(\tau_{g^{\diamond}}) \ge v^{\diamond} - \delta'$. \\[-1em]

   \underline{\textit{Step ${2}$.}} Define  $v^{\varepsilon} =\underset{g \ \in \  \frakN}{\sup} \  v(\mu^{\varepsilon}_g),$ \  $\varepsilon >0$.  For any  $f \in \frakF$, \cref{cor:relaxUnif} implies that 
    $v(\mu^{\varepsilon}_f) \to v(\tau_f)$  as $\varepsilon \to 0$. 
    In particular, taking $f=g^{\diamond}$ from Step 1 yields 
    $$\liminf_{\varepsilon \to 0 } v^{\varepsilon} \ge  \liminf_{\varepsilon \to 0 } v(\mu_{g^{\diamond}}^{\varepsilon}) = v(\tau_{g^{\diamond}}) . $$
    Thus, one can pick $ \bar{\varepsilon}  >0$ such that $v^{\varepsilon} \ge v(\tau_{g^{\diamond}})  - \delta'$ for all $\varepsilon \in (0,\bar{\varepsilon})$. \\[-1em]
    
     \underline{\textit{Step ${3}$.}}  Using again \cref{cor:relaxUnif}, there exists  $ \ \varepsilon \in (0,\bar{\varepsilon})$ such that for all $f \in \frakF$,    \begin{equation}\label{eq:step3}
      |v(\tau_{f}) - v(\mu^{\varepsilon}_{f})| \le C\sqrt{\rho(\varepsilon)} \le  \delta'.
     \end{equation} 
     Consequently, if  $g^{\varepsilon,\gamma} \in \frakN$ is a $\gamma-$maximizer of $v^{\varepsilon}$, then 
     $$v(\tau_{g^{\varepsilon,\gamma}}) \ge v(\mu^{\varepsilon}_{g^{\varepsilon,\gamma}}) - \delta' \ge v^{\varepsilon} - \gamma-\delta'. $$
   \underline{\textit{Step ${4}$.}}
Collecting the above inequalities, we obtain
\begin{align*}
    v(\tau_{g^{\varepsilon,\gamma}})  
    \ge v^{\varepsilon} - \gamma-\delta'  
    \ge  v(\tau_{g^{\diamond}}) - \gamma - 2 \delta'
    \ge v^{\diamond}- \gamma - 3\delta'.
\end{align*}
We can therefore set $\delta' = \gamma = \frac{\delta}{4}$.  
\end{proof}

\subsection{Convergence analysis: semicontinuous boundaries}\label{sec:convLSC}

This section consider optimal boundaries $f^{\diamond} = f^{\diamond}(t,\xi)$ that are only lower continuous in $\xi$. To project $f^{\diamond}$ onto $\frakN$, we  first carefully construct a sequence of \textit{continuous} boundaries converging to $f^{\diamond}$. These continuous boundaries can thereafter be approximated by elements in $\frakN$. To construct such sequence,  we utilize the notion of \textit{inf/sup convolution},  which is central in the theory of viscosity solutions; see \cite[Section V.5]{FS} and \cite{LasryLions}.   

Let $h:\calE \to \R$ be a lower semicontinuous function and define its \textit{inf convolution}  as
\begin{equation}\label{eq:infconvDef}
      h_\delta(\xi) := \inf_{\xi' \in  \calE}\left[h(\xi') + \frac{1}{\delta} |\xi'-\xi|^2 \right] \le h(\xi), \quad \delta >0. 
\end{equation}
    It is easily seen that $h_\delta$ is semiconcave, hence continuous.    
For $f \in \frakF$, the inf convolution of $f$ is understood as $f_{\delta}(t,\cdot) = f(t,\cdot)_{\delta}$   for each $t\in \calT$.  The next proposition shows that $f_{\delta} \uparrow f$ as $\delta \to 0$ as illustrated in \cref{fig:infconv}. In particular, the hitting time $\tau_{f_{\delta}}$ of   $\frakS(f_{\delta})$ increases to $\tau_{f}$.    

\begin{figure}[t]
    \centering
    \caption{Inf convolution of $f(t,\cdot)$ for some $t\in \calT$. The monotonicity of $\delta \to f_{\delta}$ implies that the hitting time $\tau_{f_{\delta}}$ %of the moving epigraph $(\frakS_t(f_{\delta})$ 
    increases  to $\tau_{f}$ (pathwise) as $\delta \downarrow 0$.  }
    \includegraphics[width = 2.9in,height = 2.0in]{Figures/infConvFillPaper.pdf}
    \label{fig:infconv}
\end{figure}

\begin{proposition}\label{prop:lsc}
    Let $h: \calE \to \R$ be lower semicontinuous and $h_\delta$ be its inf convolution with parameter $\delta$ as in \eqref{eq:infconvDef}. 
    Then  $h_\delta \uparrow h$ pointwise. 
\end{proposition}
\begin{proof}
It is clear that $h_\delta$ increases with $\delta$, hence any sequence $(h_{\delta_l})$ with $ \delta_{l} \downarrow 0$  is non-decreasing. 
Let $\xi_l$ be a $\delta_l-$minimizer of $h_{\delta_l}(\xi)$, i.e. $h(\xi_l) + \frac{1}{\delta_l} |\xi - \xi_l|^2 \le h_{\delta_l}(\xi)+ \delta_l$. Then, 
    $$h(\xi) \ge h_{\delta_l}(\xi) \ge h(\xi_l) + \frac{1}{\delta_l} |\xi - \xi_l|^2 -\delta_l\ge \frac{1}{\delta_l} |\xi - \xi_l|^2 -\delta_l,$$
    which implies that $|\xi - \xi_l|^2 \le \delta_l (\delta_l + h(\xi))$. Therefore $\xi_l \to \xi$, and  the lower semicontinuity of $h$ gives
    $$h(\xi) \le \liminf_{l\to \infty} h(\xi_l)\le \liminf_{l\to \infty} \left[ h(\xi_l) + \frac{1}{\delta_l} |\xi - \xi_l|^2 \right]\le \liminf_{l\to \infty} \left[ h_{\delta_l}(\xi) + \delta_l \right]\le h(\xi). $$
\end{proof}
More can be said when restricting l.s.c. boundaries to a compact set. Accordingly, we define
\begin{equation}\label{eq:infconvCpctDef}
      h_{\delta}^{\calK} (\xi) := \inf_{\xi' \in \ \calK}\left[h(\xi') + \frac{1}{\delta} |\xi'-\xi|^2 \right], \quad \delta >0, \quad \xi \in \calK \subset \subset \calE. 
\end{equation}
The inf convolution of $f \in \frakF$ in $\calK$ is understood as $f_{\delta}^{\calK}(t,\cdot) = f(t,\cdot)_{\delta}^{\calK}$   for each $t\in \calT$.  
Since $\xi' \mapsto h(\xi') + \frac{1}{\delta} |\xi'-\xi|^2$ is also l.s.c., it attains its minimum on  $\calK$.   
This leads us to the following corollary. Throughout, we write $B_{r}(\xi)$   for the  closed ball  of radius $r\ge 0$ centered at $\xi \in \calE$.   
\begin{corollary}\label{cor:lsc}
    Let  $\calK \subset \subset \calE$ and $h:\calE \to \R$ be a lower semicontinuous function such that $ M := \lVert h  \rVert_{L^{\infty}(\calK)} < \infty$. Then for all $\delta>0$, $\xi \in \calK$, any minimizer achieving $h_{\delta}^{\calK}(\xi)$ in \eqref{eq:infconvCpctDef} is contained in $B_{\sqrt{\delta M}}(\xi)$. 
\end{corollary}
\begin{proof}
Let $\xi_{\delta} \in \calK$ be any minimizer in \eqref{eq:infconvCpctDef}, i.e. $h_{\delta}^{\calK}(\xi)  = h(\xi_{\delta}) + \frac{1}{\delta} |\xi_{\delta}-\xi|^2$. Then
    $$M\ge h(\xi) \ge h_{\delta}^{\calK}(\xi)  =  h(\xi_{\delta}) + \frac{1}{\delta} |\xi_{\delta}-\xi|^2 \ge \frac{1}{\delta} |\xi_{\delta}-\xi|^2. $$\end{proof}


\begin{remark}
    When the stopping region is the hypograph of the optimal boundary ($\eta =-1$ in \ref{asm:star}) one can employ \textit{sup convolutions} instead, that is
        $$h^{\delta}(\xi) := \sup_{\xi' \in \ \calE}\left[h(\xi') - \frac{1}{\delta} |\xi'-\xi|^2 \right] \ge h(\xi), \quad \delta >0. $$
        We may also define the restriction $h^{\delta,\calK}$ to some compact set $\calK$. This case is simpler since u.s.c functions are automatically bounded above in compact sets. 
\end{remark}

The next lemma states that inf convolutions approximate lower semicontinuous functions arbitrarily well with respect to the relaxed $L^\infty$ distance seen in \cref{def:relaxedSupDist}.  


\begin{lemma}\label{lem:infCovApprox}
          Let $\iota >0$ and $\calK \subset \subset \calE$. If  $f \in \frakF$  bounded in $\calT\times \calK$, then there exists $\delta>0$ such that 
          $d_{\calK,\calT}(f,f_{\delta}^{\calK}) \le \iota.$
\end{lemma}
\begin{proof}
    Let $\iota >0$ and $r >0$ be arbitrary. Since $\calK$ is compact, one can choose $(\xi^i)_{i=1}^{I} \subseteq  \calK$, $I< \infty$ such that $\calK \subseteq  \bigcup_{i=1}^{I} B_r(\xi^i)$ where we recall that $B_r(\xi^i) = \{\xi \in \calE \ : \ |\xi-\xi_i| \le r\}$. Now fix $t\in \calT$ and  write $h(\xi) = f(t,\xi)$ for brevity.    As $h$ is l.s.c., there exist $\{r_i\}_{i=1}^I \subset (0,\infty)$ satisfying 
    \begin{equation}\label{eq:lscIota}
        h(\xi^i) \le h(\xi') + \iota, \quad \forall \ \xi'\in B_{r_i}(\xi^i), \quad i =1,\ldots,I. 
    \end{equation}
If we set $\delta_t = \frac{1}{M} \min_i r_i^2>0$,  $M = \lVert h \rVert_{L^\infty(\calK)}$, then  $\sqrt{\delta_t M} \le r_i$ for all $i=1,\ldots,I$. For each $i\in \{1,\ldots,I\}$, take a minimizer  $\xi^i_{\delta_t}$  achieving  $h_{\delta_t}^{\calK}(\xi^i)$ in \eqref{eq:infconvCpctDef}.  
In view of  \cref{cor:lsc},  $\xi^i_{\delta_t}$ belongs to  $B_{\sqrt{\delta_t M}}(\xi^i)$. But $B_{\sqrt{\delta_t M}}(\xi^i)\subseteq B_{r_i}(\xi^i)$, hence 
$$h_{\delta_t}^{\calK}(\xi^i) = h(\xi^i_{\delta_t}) + \frac{1}{\delta_t}|\xi^i - \xi^i_{\delta_t}|^2 \ge h(\xi^i_{\delta_t})  \overset{\eqref{eq:lscIota}}{\ge}  h(\xi^i) - \iota. $$
Consequently,  $0\le h(\xi^i) - h_{\delta_t}^{\calK}(\xi^i) \le \iota$ for all $i=1,\ldots,I$. To finish off, define the quantization map 
$$\underline{\psi}: \calK \to \{\xi^1,\ldots,\xi^{I}\}, \quad \underline{\psi}(\xi) =  \underset{\xi^1,\ldots,\xi^{I}} {\text{argmin}} \ |\xi-\xi^i|. $$
If there are several elements in $\{\xi^1,\ldots,\xi^{I}\}$ achieving $\min_{\xi^1,\ldots,\xi^{I}} \ |\xi-\xi^i|$, we simply choose the one with smallest index. 
It is clear that $|\underline{\psi}(\xi) - \xi| \le r$ for all $\xi \in \calK$, hence $\underline{\psi} \in \Psi_{r}^{\calK}$. %since $(B_{r}(\xi^i))_{i=1}^I$ covers $\calK$. 
As $|h(\xi^i) - h_{\delta_t}^{\calK}(\xi^i)| \le \iota$ for all $i=1,\ldots,I$, we conclude that 
$$\inf_{\psi \in \Psi_{r}^{\calK}} \lVert h\circ \psi -  h_{\delta_t}^{\calK}\circ \psi \rVert_{L^\infty(\calK)} \le \lVert h\circ \underline{\psi} -  h_{\delta_t}^{\calK}\circ \underline{\psi} \rVert_{L^\infty(\calK)} \le \iota.$$
 The proof is complete after setting $\delta = \min_{t\in \calT} \delta_t >0$.
 \end{proof} 

The next approximation result follows immediately. 
\begin{theorem} \textnormal{\textbf{(Universal approximation of lower semicontinuous functions)}}
\label{thm:LSCUAT}\\
   Let  $ \frakN \subseteq \frakF_c$ be a hypothesis space satisfying Assumption \ref{asm:UAP}. Then for all $f \in \frakF$, $ \iota >0$, and compact set $\calK \subset \subset \calE$ such that $f$ is  bounded in $\calK$, there exists  $g\in \frakN$ such that  $d_{\calK,\calT}(f,g) \le \iota$. 
\end{theorem}

\begin{proof}
Fix $r,\iota' > 0$,  $\calK \subset \subset \calE$, and $\xi \in \calK$. Using \cref{lem:infCovApprox}, then $d_{\calK,\calT}(f,f_{\delta}^{\calK}) \le \iota'$ for some $\delta > 0$. 
 For every $\gamma>0$, one can find $\psi_{\gamma} \in \Psi_{r}^{\calK}$ such that 
 $$\lVert f(t,\cdot) \circ \psi_{\gamma} - f_{\delta}^{\calK}(t,\cdot) \circ \psi_{\gamma} \rVert_{L^{\infty}(\calK)} \le d_{\calK}(f(t,\cdot),f_{\delta}^{\calK}(t,\cdot)) + \gamma \le \iota' + \gamma, \qquad \forall \ t\in \calT.  $$
    Moreover, as $f_{\delta}^{\calK}(t,\xi)$ is continuous in $\xi$,  we can invoke Assumption \ref{asm:UAP} giving the existence of   $g\in \frakN  \subseteq \frakF_c$ such that $\lVert f_{\delta}^{\calK} - g \rVert_{L^{\infty}(\calT \times \calK)} \le \iota'$.
The triangular inequality therefore yields 
 \begin{align*}
     \lVert f(t,\cdot) \circ \psi_{\gamma} - g(t,\cdot) \circ \psi_{\gamma} \rVert_{L^{\infty}(\calK)} \le  2\iota' + \gamma, \qquad \forall \ t\in \calT. 
 \end{align*}
As $r$ is arbitrary, we conclude that  $d_{\calK,\calT}(f,g) \le 2\iota' + \gamma$. Choosing $\iota' = \frac{\iota}{2}$ and  letting $\gamma \downarrow 0$ proves the result.  
\end{proof}

At last, this leads us to the following   convergence result for lower semicontinuous  boundaries. 
\begin{theorem}
   Let $\frakN \subset \frakF_c$  be a family of universal approximators.  Under Assumption \ref{asm:absCont}, for every $\delta>0$, there exists $\varepsilon=\varepsilon(\delta), \gamma=\gamma(\delta)>0$  such that any $g^{\varepsilon,\gamma} \in \frakN$ with the property $ v(\mu^{\varepsilon}_{g^{\varepsilon,\gamma}}) \ge \underset{g \in   \frakN}{\sup} \  v(\mu^{\varepsilon}_g) - \gamma$ also satisfies,
 $v(\tau_{g^{\varepsilon,\gamma}})\ge v^{\diamond} - \delta$. 
\end{theorem}

\begin{proof} Let $\delta'>0 $ be arbitrary. Using \cref{thm:lscV}, there exist $\delta''>0$, $\calK \subset \subset \calE$,  and $\iota>0$ such that
\begin{equation}\label{eq:contV}
    d_{\calK,\calT}(f,f') \le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho(\iota) + \delta''}\le \delta', \quad \forall f,f'\in \frakF.  
\end{equation}
As $f^{\diamond}$ is locally bounded, we can apply  \cref{thm:LSCUAT} giving the existence of    $g^{\diamond} \in \frakN$ such that 
$ d_{\calK,\calT}(f^{\diamond} ,g^{\diamond}) \le \iota. $
We conclude  from \eqref{eq:contV}  that $v(\tau_{g^{\diamond}}) \ge v^{\diamond} - \delta'$. As $g^{\diamond}$ is continuous, we can follow Step 2, 3, and 4 in the proof of \cref{thm:convCont}. 
\end{proof}

\section{Conclusion}\label{sec:conclusion}
We analyze  hitting times of boundaries arising in optimal stopping. 
 After introducing relaxed stopping rules and establishing preliminary results, the continuity of the value functional $f\mapsto v(\tau_f)$ is shown with respect to the topology of uniform convergence and the novel relaxed $L^{\infty}$ distance. 
  The main results are later applied   to study the convergence of  the neural optimal stopping boundary method \cite{ReppenSonerTissotFB}. When the optimal stopping boundary is continuous, we can directly invoke the universal approximation theorem of neural networks and obtain a convergence theorem. When the optimal stopping boundary is strictly semicontinuous,  inf/sup convolutions are combined  with the relaxed $L^{\infty}$ distance, leading to a more general  result. 

A natural extension of the present work would be to show similar continuity and relaxation results for optimal stopping problems in continuous time. In particular, it would be worth investigating the convergence of the neural optimal stopping method for \textit{American} options, namely when $\calT = [0,T]$. %as the number of time steps to discretize $\calT$ goes to infinity.  

%This would require technical tools 

\appendix 

\section{Proof of \cref{prop:relaxOS}}
\label{app:relaxedproblem}

\begin{proof}
   We write $\underline{v}^{\diamond}:=  \sup_{\mu \in \underline{\vartheta}(\calT)} v(\mu)$ and show that  $\underline{v}^{\diamond} = v^{\diamond}$ by induction on $N = |\calT|$. If $N=1$,  then $\calT$ is a singleton, hence $\underline{\vartheta}(\calT) = \vartheta(\calT)$. We now suppose the result true for $N\ge 1$ and prove the claim for $N+1$. Let $\calT = \{t_1<\ldots < t_{N+1}\}\subset [0,T]$ and fix  $\mu = \sum_{t\in \calT} P_t \ \delta_t \in \underline{\vartheta}(\calT)$ where each $P_t:\Omega \to [0,1]$ is $\calF_t-$measurable.  Next,  write $\calT_{\! +} = \calT \setminus  \{t_1\}$ and consider the continuation value functional  
    $$v_1(\mu_{+},x) = \E^{\Q}\left[\int_{\calT_{\! +}} \varphi(t,X_{t}) \mu_{+}(dt)  \ \big | \ X_{t_1} = x\right], \quad \mu_{+}  \in \underline{\vartheta}(\calT_{\! +}). $$
    Since $|\calT_{\! +}| = N$, we have by induction that 
\begin{equation}\label{eq:induction}
        v_1(\mu_{+},x) \le v_1^{\diamond}(x) := \sup_{\tau \in \vartheta(\calT_{\! +})} \E^{\Q}[ \varphi(\tau,X_{\tau}) \ | \ X_{t_1} = x], \quad \forall \ \mu_{+}  \in \underline{\vartheta}(\calT_{\! +}). %v(\tau,x).
    \end{equation}
    Then, the tower property of conditional expectations implies that %conditioning on $\calF_{t_0}$
\begin{align}
        v(\mu) &= \E^{\Q}\left[P_{t_1} \varphi(t_1,X_{t_1}) + \int_{\calT_{\! +}} \varphi(t,X_{t}) \mu(dt)   \right]\nonumber  \\[0.5em]
        &= 
    \E^{\Q}\left[ P_{t_1} \varphi(t_1,X_{t_1}) + (1-P_{t_1})\int_{\calT_{\! +}} \varphi(t,X_{t}) \mu_{+}(dt)\right] \nonumber\\[0.5em] 
        &= 
    \E^{\Q}\left[ P_{t_1} \varphi(t_1,X_{t_1}) + (1-P_{t_1})v_1(\mu_{+},X_{t_1}) \right], \label{eq:trick}    
    \end{align} 
    with the relaxed stopping rule 
    $$\mu_{+}(\omega) = \sum_{t\in \calT_{\! +}}\frac{P_t(\omega)}{1-P_{t_1}(\omega)} \ \delta_t \ \in \  \underline{\vartheta}(\calT_{\! +}), \qquad P_{t_1} <  1.$$ Note that if $P_{t_1}(\omega) = 1$, then $\mu_{+}(\omega)$ would not appear in \eqref{eq:trick}. 
    Together with \eqref{eq:induction}, we obtain 
    \begin{align}
     v(\mu) &\le \E^{\Q}\left[ P_{t_1} \varphi(t_1,X_{t_1}) + (1-P_{t_1})v_1^{\diamond}(X_{t_1}) \right] \nonumber \\[1em]
     &=\E^{\Q}\left[ P_{t_1} (\varphi(t_1,X_{t_1}) - v_1^{\diamond}(X_{t_1})) \right] + \E^{\Q}\left[v_1^{\diamond}(X_{t_1}) \right].\label{eq:induction2}
     \end{align}
    We can now maximize the first term in \eqref{eq:induction2}  over all $\calF_{t_1}-$measurable functions $P_{t_1}:\Omega \to [0,1]$. 
  It is straightforward to see and also   classical in  optimal stopping \cite{PeskirShiryaev} 
  that the unique maximizer is given by\footnote{In financial terms, this  means that one should exercise a Bermudan contract whenever  the intrinsic value $\varphi(t_1,X_{t_1})$ exceeds the continuation value $v_1^{\diamond}(X_{t_1})$.}   
  $$P_{t_1}^{\diamond}(\omega) = \begin{cases} 1, \quad & \text{if } \varphi(t_1,X_{t_1}(\omega)) \  \ge \ v_1^{\diamond}(X_{t_1}(\omega)), \\ 
  0,\ & \text{otherwise}.\end{cases}$$ %\mathds{1}_{\{\varphi(t_1,X_{t_1}) \  \ge \ v_1^{\diamond}(X_{t_1}) \}}.$$ 
  In particular, it is $\{0,1\}-$valued. 
This leads to  the dynamic programming equation 
  $$v^{\diamond} = \E^{\Q}\left[ P_{t_1}^{\diamond} (\varphi(t_1,X_{t_1}) - v_1^{\diamond}(X_{t_1})) \right] + \E^{\Q}\left[v_1^{\diamond}(X_{t_1}) \right] = \E^{\Q}\left[  \varphi(t_1,X_{t_1}) \vee v_1^{\diamond}(X_{t_1}) \right] \ge v(\mu). $$
  As
   $v^{\diamond}\le \underline{v}^{\diamond}$ is evident, \eqref{eq:OSvsRelax}  follows. 
Moving to the second assertion,  the induction hypothesis implies that  every optimal relaxed stopping rule of $\sup_{\mu_{+} \in \underline{\vartheta}(\calT_{\!+})} v_1(\mu_{+},x)$ is in fact  a genuine stopping time, say $\tau_{+}$. Together with the above arguments, we gather  that the same holds true when adding back the first exercise date $t_1$. Precisely, we have $v(\tau^{\diamond}) = \underline{v}^{\diamond}$ with the stopping time 
$\tau^{\diamond} = P_{t_1}^{\diamond} t_1  + (1-P_{t_1}^{\diamond}) \tau_{+}$.   
\end{proof}





==> FinancialExamples.tex <==
\section{Financial Examples}
\label{sec:finExamples}

\begin{example}\label{ex:mincall}
    (Min-call option) This corresponds to $\eta =1$ and  $\alpha(x) = \min_{i=1,...,m}x^i$. Not that the corresponding payoff function is \textit{not} convex in $x$. As shown in \cite{DetempleMin}, the function $[1,\infty) \ni \xi \to f(t,\xi)$ is  \textit{discontinuous} at $\xi = 1$. Therefore, the universal theorem for neural networks does not apply. A remedy is given in \cref{sec:lscBoundary}.  
\end{example}

\begin{example}\label{ex:maxcall}
    (Max-call option) This corresponds to $\eta =1$ and  $\alpha(x) = \max_{i=1,...,m}x^i$. Let $\calX = \R_+^2$. By symmetry we can focus on  $\calS^{(1)}_t = \calS_t \cap \  \{x\in \calX \ : \ x_2 \ge x_1\}$. Then there exists $f:\calT\times [0,1] \to \R_+$ such that $\calS^{(1)}_t = \{x_2 \ge f(t,x_1/x_2)\} $.   In \citet[Proposition 2.4.]{BroadieDetemple} it is shown that there exists $\lambda_1 < 1 < \lambda_2$ such that $\calS_t$ does not intersect the cone $$\frakC_{\lambda_1,\lambda_2} = \left\{x \ : \  x_2/x_1 \in (\lambda_1,\lambda_2)\right \}.$$ 
    %$$\calS_t \cap \ \underbrace{\left\{x \ : \  x_2/x_1 \in (\lambda_1,\lambda_2)\right \}}_{ = \ \frakC_{\lambda_1,\lambda_2}} = \varnothing. $$ 
    This implies that $\exists \ \xi^* \in [0, 1/\lambda_2]$ such that $\lim_{\xi \uparrow \xi^*}f(t,\xi^*) = \infty$ and $f(t,\xi) = \infty$ for all $\xi \in [\xi^*,1]$. In particular, the  distance $d_{\text{ray}}(x,\frakS_t(f))$ is infinite inside  $\frakC_{\lambda_1,\lambda_2}$.
\end{example}

==> OLD/04-06-2025/Algorithm.tex <==
\section{Application to neural  stopping boundaries} \label{sec:NOSB}

%\subsection{Universal Approximators and Stochastic Optimization}
%\label{sec:UAP_SO}
\rr{In this section, we apply the continuity results to prove the convergence 
of the \textit{Neural Optimal Stopping Boundary method}   developed in
\cite{ReppenSonerTissotFB}.  We outline the algorithm for the convenience of the reader.} Under a suitable coordinate system  $(\alpha,\Xi)$ as in Assumption \ref{asm:star}, the algorithm looks for a \textit{neural stopping boundary}, namely a feedforward neural network $g^{\theta}: \calT \times \calE \to \R_+ $  in a (sufficiently large) hypothesis space $\frakN$ % = \{g^{\theta}: \calT \times \calE \to \R_+ \ : \ \theta \in \Theta\}$ 
such that $$v(\tau_{g^{\theta}}) \approx \sup_{f\in \frakF}
v(\tau_f) \  = v^{\diamond}.$$ %Because of this approximation  capability and available libraries such as Tensorflow and Pytorch to efficiently "train" the parameters, neural networks give a natural choice for $\frakN$. 
Additional details on the  architecture and  size of the neural networks 
for this problem are given in \cite{ReppenSonerTissotFB}.
The parameter vector $\theta$ is thereafter trained using stochastic gradient ascent. As explained at the beginning of \cref{sec:relaxation}, the  stopping rule needs to be relaxed to avoid vanishing gradient issues. 
For some fixed fuzzy region width $\varepsilon>0$, we therefore 
aim to 
\begin{equation}
\label{eq:OSNNRelax}
\text{maximize}
\ \ 
v(\mu_g^{\varepsilon}) =  \E^{\Q}\left[ \int_{\calT}\varphi(t,X_{t})\mu_g^{\varepsilon}(dt)\right]
\qquad
\text{over}\  g\in \frakN,
 %\sup_{g\in \frakN} v(\mu_g^{\varepsilon}), 
\end{equation} 
with the relaxed stopping rule $\mu_g^{\varepsilon}$ given in \eqref{eq:relaxedRule}.  
The vanishing gradient problem is henceforth resolved and owing to well-known convergence results in stochastic optimization \cite{RobbinsMonro,RobbinsSiegmund}, we can find for every $\gamma > 0$ %using stochastic gradient ascent 
an 
$\gamma-$\textit{maximizer} 
$g^{\varepsilon,\gamma} \in \frakN$, that is %  of the relaxed problem with fuzzy parameter $\varepsilon$, that is  
\begin{equation}\label{eq:fuzzytraining}
   v(\mu^{\varepsilon}_{g^{\varepsilon,\gamma}})\ge \sup_{g \in \frakN} \  v(\mu^{\varepsilon}_g) - \gamma.  
\end{equation} 
Finally, the value of the optimal stopping problem is computed using  the strict stopping rule $\tau_{g^{\varepsilon,\gamma}}$ instead of  $\mu^{\varepsilon}_{g^{\varepsilon,\gamma}}$. %$v(\tau_{g^{\varepsilon,\gamma}})$. 
The method is summarized in  \cref{alg:NOSB}. 
For further details, see Appendix C in \cite{ReppenSonerTissotFB}.  The goal of this section is to show that $
   v(\tau_{g^{\varepsilon,\gamma}})$ can be made arbitrarily close to the optimal value $ v^{\diamond} 
$ when   $\varepsilon, \gamma$ are small enough. 

\begin{remark}\label{rem:MC}
When computing the value associated to the trained stopping rule, say $\tau_{g}$,  an additional inaccuracy comes  from the Monte Carlo simulations of the process; see step III in \cref{alg:NOSB}. There is nevertheless a clear  control of this error.  Indeed, it is classical that 
$$|v(\tau_{g}) - \hat{v}_J(\tau_{g})| = \calO(J^{-1/2}),$$
 when the random reward $\varphi(\tau_{g},X_{\tau_{g}})$ is  square integrable. Under Assumption \ref{asm:absCont}, this is indeed the case (see also the proof of \cref{lem:TV}). 
   % In the analysis, we omit the Monte Carlo error when analyzing the convergence   of the trained boundary $v(\tau_{g^{\varepsilon,\gamma}})$  (see step III in \cref{alg:NOSB}). This is because 
\end{remark}


 
\begin{remark}
In \cite{ReppenSonerTissotFB},  a two-sided fuzzy region is considered, namely 
  $ \{ x\in \calX \ : \  |d(t,x;f)| < \varepsilon \},$ 
where $d(t,\cdot;f)$ is the  \textit{signed distance function} to  $\partial \frakS_t(f)$. 
Although the two representations are equivalent, one-sided fuzzy regions are  more practical towards a convergence analysis.
\end{remark}

\begin{algorithm}[t]
\caption{Neural Optimal Stopping Boundary Algorithm (summary) }\label{alg:NOSB}

\vspace{1mm}
\textbf{Given}: $\varphi=$ payoff, $ \calT =$ exercise dates, $\Theta=$ parameter set, $I =  \#$ training iterations,  $\zeta=$ learning rate process,  $\varepsilon=$ fuzzy region width, $B = $ batch size, $J= \#$ simulations for the value  \\[-0.8em]  \hrule

\begin{itemize}
 \setlength \itemsep{-0.1em}
\item[I.] \textbf{Initialize} $\theta_0 \in \Theta$
\item[II.] For $i = 0,\ldots,I-1$:
    \begin{enumerate}
    \setlength \itemsep{0.5em}
        \item \textbf{Simulate} $X(\omega_b) = \{X_t(\omega_b)\}_{t\in \calT}$, $\omega_b \in \Omega $, $b=1,\ldots, B$
        \item \textbf{Compute}  $ \hat{v}_B(\mu^{\varepsilon}_{g^{\theta_i}}) :=\frac{1}{B}\sum\limits_{b=1}^B \int_{\calT}  \varphi(t,X_{t}(\omega_b)) \ \mu^{\varepsilon}_{g^{\theta_i}}(\omega_b)(dt) $ % $ \hat{v}(\mu^{\varepsilon}_{g^{\theta_i}}) :=\frac{1}{B}\sum\limits_{j=1}^B \sum\limits_{t\in \calT} P_{g^{\theta_i},t}^{\varepsilon}(\omega_j) \ \varphi(t,X_{t}(\omega_j)) $
\item \textbf{Gradient step}: $\theta_{i+1} = \theta_{i} + \zeta_i \nabla_\theta \hat{v}_B(\mu^{\varepsilon}_{g^{\theta_i}}) $
   \end{enumerate}
\item[III.] \textbf{Return} $g = g^{\theta_{I}}$ and $\hat{v}_J(\tau_{g}) := \frac{1}{J}\sum\limits_{j=1}^J \varphi(\tau_{g}(\omega_j),X_{\tau_{g}}(\omega_j)), \  \omega_j \in \Omega $, $\ j=1,\ldots, J$
\end{itemize}
\vspace{-3mm}
\end{algorithm}

\subsection{Convergence analysis: continuous boundaries}

We first outline our strategy to prove convergence of the Neural Optimal Stopping Boundary method when the optimal stopping boundary $f^{\diamond}$ is continuous. First, the hypothesis space $\frakN$ (neural networks in this case) must satisfy a universal approximation property; see Assumption \ref{asm:UAP} below. Thus, there exists $g^{\diamond} \in \frakN$ arbitrarily close to $f^{\diamond}$ in compact sets. We can  therefore invoke our first continuity result  (\cref{thm:unifcontV}) to ensure that the values of the stopping strategies $\tau_{f^{\diamond}}$, $\tau_{g^{\diamond}}$ are close as well. Next, we relax the problem and use \cref{cor:relaxUnif}  to guarantee that $v(\mu^{\varepsilon}_{g^{\diamond}}) \approx  v(\tau_{g^{\diamond}})$ for small fuzzy parameter $\varepsilon$. We then train the neural boundary  %from classical results in stochastic optimization \cite{RobbinsMonro,RobbinsSiegmund} 
to construct $g^{\varepsilon,\gamma} \in \frakN$ such that $v(\mu^{\varepsilon}_{g^{\diamond}}) \approx v(\mu^{\varepsilon}_{g^{\varepsilon,\gamma}})$ and finally  conclude that $v(\mu_{g^{\varepsilon,\gamma}}^{\varepsilon}) \approx  v(\tau_{g^{\varepsilon,\gamma}})$  in view of   \cref{cor:relaxUnif}.  The above steps can be summarized as follows: %in the following sequence:
\begin{align*}
    v^{\diamond} &= v(\tau_{f^{\diamond}}) && \\  
&\approx v(\tau_{g^{\diamond}}) && \longleftarrow \ \textnormal{approximation and continuity (Assumption \ref{asm:UAP} and \cref{thm:unifcontV})}\\ 
&\approx  v(\mu_{g^{\diamond}}^{\varepsilon}) && \longleftarrow \ \textnormal{relaxation (\cref{cor:relaxUnif})} \\ 
&\approx  v(\mu_{g^{\varepsilon,\gamma}}^{\varepsilon}) && \longleftarrow \ \textnormal{stochastic optimization  \cite{RobbinsMonro,RobbinsSiegmund}} \\ 
&\approx v(\tau_{g^{\varepsilon,\gamma}}). && \longleftarrow \ \textnormal{relaxation (\cref{cor:relaxUnif})}
\end{align*}
We start with the approximation of $f^{\diamond}$. Let $\frakF_c  = \{f \in \frakF :  f(t,\cdot) \in \calC(\calE) \; \forall t\in \calT\}$ denotes the set of continuous boundaries and consider  a  hypothesis space $\frakN \subset \frakF_c$ satisfying the following assumption which can be seen as the \textit{universal approximation property}. 
\begin{asm}\label{asm:UAP}
For all 
$f\in \frakF_c$, compact set  $\calK \subset \subset \calE$  and $\iota >0$, there exists  $g\in \frakN$ such that  
\begin{equation}\label{eq:UAP}
    \lVert f - g \rVert_{L^{\infty}(\calT \times \calK )} \le \iota. 
\end{equation}
\end{asm}

We refer to elements in a family $\frakN \subset \frakF_c$ such that 
Assumption \ref{asm:UAP} holds as \textit{universal approximators}. The Stone-Weierstrass theorem gives an example of  universal approximators, namely the polynomials. This class, however, is  numerically unsuitable when the Hausdorff dimension of $\calE$ is large. In our case, $\frakN$ is evidently the family of all feedforward neural networks $g^\theta:\calT\times \  \calE \to \R_+$ with finite-dimensional parameter vector $\theta$. %s $\theta \in \R^{p}$ for some $p\in \N$. 
Assumption \ref{asm:UAP} follows classically from the 
 Universal Approximation Theorem (UAT) for neural networks \cite{Cybenko,Hornik}. 
 %Importantly, neural networks do not suffer much from the  curse of dimensionality; see, e.g., \cite{Gonon}. 

% If the optimal boundary $f^{\diamond}$ belongs to $\frakF_c$, we can  invoke the universal approximation property of $\frakN$ giving the existence of $g^{\diamond}$ arbitrarily close to $f^{\diamond}$ in some compact set. 
% This is no longer the case when $f^{\diamond}$ is  strictly lower semicontinuous; a remedy will be given in \cref{sec:lscBoundary}. 
In this section, we assume that $f^{\diamond}(t,\xi)$ is  continuous in $\xi$, i.e. $f^{\diamond} \in \frakF_c$. We can therefore directly use $f^{\diamond}$ in Assumption \ref{asm:UAP}. Together with the results from \cref{sec:continuity}, the next convergence theorem follows naturally. 
\begin{theorem}\label{thm:convCont}
   Consider $\frakN \subset \frakF_c$  satisfying Assumption \ref{asm:UAP}, $f^{\diamond}\in \frakF_c$, and suppose that Assumption  \ref{asm:absCont} holds.  Then, for every $\delta >0$,   there exists $\varepsilon=\varepsilon(\delta), \gamma=\gamma(\delta)>0$  such that any $g^{\varepsilon,\gamma} \in \frakN$ with the property $ v(\mu^{\varepsilon}_{g^{\varepsilon,\gamma}}) \ge \underset{g \in   \frakN}{\sup} \  v(\mu^{\varepsilon}_g) - \gamma$ also satisfies,
   \begin{equation}\label{eq:UpperBound}
    v(\tau_{g^{\varepsilon,\gamma}})\ge v^{\diamond} - \delta.  
\end{equation} 
\end{theorem}

\begin{proof} \underline{\textit{Step ${1}$.}}  Let $\delta'>0 $ be arbitrary. From  \cref{thm:unifcontV}, there exist $\delta''>0$, $\calK\subseteq \calE$ compact,  and $\iota>0$ such that
\begin{equation}\label{eq:contV}
    \lVert f - f' \rVert_{L^{\infty}(\calT \times \calK)}\le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho(\iota) + \delta''}\le \delta'. 
\end{equation}
Invoking Assumption \ref{asm:UAP}, there exists   $g^{\diamond} \in \frakN$ such that 
$\lVert f^{\diamond} - g^{\diamond} \rVert_{L^{\infty}(\calT \times \calK)}\le \iota. $
We conclude  from \cref{thm:unifcontV}  that $v(\tau_{g^{\diamond}}) \ge v^{\diamond} - \delta'$. \\[-1em]

   \underline{\textit{Step ${2}$.}} Define  $v^{\varepsilon} =\underset{g \ \in \  \frakN}{\sup} \  v(\mu^{\varepsilon}_g),$ \  $\varepsilon >0$.  For any  $f \in \frakF$, \cref{cor:relaxUnif} implies that 
    $v(\mu^{\varepsilon}_f) \to v(\tau_f)$  as $\varepsilon \to 0$. 
    In particular, taking $f=g^{\diamond}$ from Step 1 yields 
    $$\liminf_{\varepsilon \to 0 } v^{\varepsilon} \ge  \liminf_{\varepsilon \to 0 } v(\mu_{g^{\diamond}}^{\varepsilon}) = v(\tau_{g^{\diamond}}) . $$
    Thus, one can pick $ \bar{\varepsilon}  >0$ such that $v^{\varepsilon} \ge v(\tau_{g^{\diamond}})  - \delta'$ for all $\varepsilon \in (0,\bar{\varepsilon})$. \\[-1em]
    
     \underline{\textit{Step ${3}$.}}  Using again \cref{cor:relaxUnif}, there exists  $ \ \varepsilon \in (0,\bar{\varepsilon})$ such that for all $f \in \frakF$,    \begin{equation}\label{eq:step3}
      |v(\tau_{f}) - v(\mu^{\varepsilon}_{f})| \le C\sqrt{\rho(\varepsilon)} \le  \delta'.
     \end{equation} 
     Consequently, if  $g^{\varepsilon,\gamma} \in \frakN$ is a $\gamma-$maximizer of $v^{\varepsilon}$, then 
     $$v(\tau_{g^{\varepsilon,\gamma}}) \ge v(\mu^{\varepsilon}_{g^{\varepsilon,\gamma}}) - \delta' \ge v^{\varepsilon} - \gamma-\delta'. $$
   \underline{\textit{Step ${4}$.}}
Collecting the above inequalities, we obtain
\begin{align*}
    v(\tau_{g^{\varepsilon,\gamma}})  
    \ge v^{\varepsilon} - \gamma-\delta'  
    \ge  v(\tau_{g^{\diamond}}) - \gamma - 2 \delta'
    \ge v^{\diamond}- \gamma - 3\delta'.
\end{align*}
We can therefore set $\delta' = \gamma = \frac{\delta}{4}$.  
\end{proof}



==> OLD/04-06-2025/AlgorithmLSC.tex <==
\subsection{Convergence analysis: semicontinuous boundaries}\label{sec:convLSC}

This section consider optimal boundaries $f^{\diamond} = f^{\diamond}(t,\xi)$ that are only lower continuous in $\xi$. To project $f^{\diamond}$ onto $\frakN$, we  first carefully construct a sequence of \textit{continuous} boundaries converging to $f^{\diamond}$. These continuous boundaries can thereafter be approximated by elements in $\frakN$. To construct such sequence,  we utilize the notion of \textit{inf/sup convolution},  which is central in the theory of viscosity solutions; see \cite[Section V.5]{FS} and \cite{LasryLions}.   

Let $h:\calE \to \R_+$ be a  lower semicontinuous function and define its \textit{inf convolution}  as
\begin{equation}\label{eq:infconvDef}
      h_\delta(\xi) := \inf_{\xi' \in  \calE}\left[h(\xi') + \frac{1}{\delta} |\xi'-\xi|^2 \right] , \quad \delta >0. 
\end{equation}
    It is easily seen that $h_\delta$ is semiconcave, hence continuous.    
For $f \in \frakF$, the inf convolution of $f$ is understood as $f_{\delta}(t,\cdot) = f(t,\cdot)_{\delta}$   for each $t\in \calT$.  The next proposition shows that $f_{\delta} \uparrow f$ as $\delta \to 0$ as illustrated in \cref{fig:infconv}. In particular, the hitting time $\tau_{f_{\delta}}$ of   $\frakS(f_{\delta})$ increases to $\tau_{f}$.    

\begin{figure}[t]
    \centering
    \caption{Inf convolution of $f(t,\cdot)$ for some $t\in \calT$. The monotonicity of $\delta \to f_{\delta}$ implies that the hitting time $\tau_{f_{\delta}}$ %of the moving epigraph $(\frakS_t(f_{\delta})$ 
    increases  to $\tau_{f}$ (pathwise) as $\delta \downarrow 0$.  }
    \includegraphics[width = 2.9in,height = 2.0in]{Figures/infConvFillPaper.pdf}
    \label{fig:infconv}
\end{figure}

\begin{proposition}\label{prop:lsc}
    Let $h: \calE \to \R_+$ be lower semicontinuous and $h_\delta$ be its inf convolution with parameter $\delta$ as in \eqref{eq:infconvDef}. 
    Then  $h_\delta \uparrow h$ pointwise. 
\end{proposition}
\begin{proof}
It is clear that $h_\delta$ increases with $\delta$, hence any sequence $(h_{\delta_l})$ with $ \delta_{l} \downarrow 0$  is non-decreasing. 
Let $\xi_l$ be a $\delta_l-$minimizer of $h_{\delta_l}(\xi)$, i.e. $h(\xi_l) + \frac{1}{\delta_l} |\xi - \xi_l|^2 \le h_{\delta_l}(\xi)+ \delta_l$. Then, 
    $$h(\xi) \ge h_{\delta_l}(\xi) \ge h(\xi_l) + \frac{1}{\delta_l} |\xi - \xi_l|^2 -\delta_l\ge \frac{1}{\delta_l} |\xi - \xi_l|^2 -\delta_l,$$
    which implies that $|\xi - \xi_l|^2 \le \delta_l (\delta_l + h(\xi))$. Therefore $\xi_l \to \xi$, and  the lower semicontinuity of $h$ gives
    $$h(\xi) \le \liminf_{l\to \infty} h(\xi_l)\le \liminf_{l\to \infty} \left[ h(\xi_l) + \frac{1}{\delta_l} |\xi - \xi_l|^2 \right]\le \liminf_{l\to \infty} \left[ h_{\delta_l}(\xi) + \delta_l \right]\le h(\xi). $$
\end{proof}
More can be said when restricting l.s.c. boundaries to a compact set. Accordingly, we define
\begin{equation}\label{eq:infconvCpctDef}
      h_{\delta}^{\calK} (\xi) := \inf_{\xi' \in \calK}\left[h(\xi') + \frac{1}{\delta} |\xi'-\xi|^2 \right], \quad \delta >0, \quad \xi \in \calK \subset \subset \calE. 
\end{equation}
The inf convolution of $f \in \frakF$ in $\calK$ is understood as $f_{\delta}^{\calK}(t,\cdot) = f(t,\cdot)_{\delta}^{\calK}$   for each $t\in \calT$.  
Since $\xi' \mapsto h(\xi') + \frac{1}{\delta} |\xi'-\xi|^2$ is also l.s.c., it attains its minimum on  $\calK$.   
This leads us to the following corollary. Throughout, we write $B_{r}(\xi)$   for the  closed ball  of radius $r\ge 0$ centered at $\xi \in \calE$.   
\begin{corollary}\label{cor:lsc}
    Let  $\calK \subset \subset \calE$ and a lower semicontinuous function $h:\calE \to \R_+$  such that $ M := \lVert h  \rVert_{L^{\infty}(\calK)} < \infty$. Then $\forall \ \delta>0$, $\xi \in \calK$, any minimizer achieving $h_{\delta}^{\calK}(\xi)$ in \eqref{eq:infconvCpctDef} is contained in $B_{\sqrt{\delta M}}(\xi)$. 
\end{corollary}
\begin{proof}
Let $\xi_{\delta} \in \calK$ be any minimizer in \eqref{eq:infconvCpctDef}, i.e. $h_{\delta}^{\calK}(\xi)  = h(\xi_{\delta}) + \frac{1}{\delta} |\xi_{\delta}-\xi|^2$. Then
    $$M\ge h(\xi) \ge h_{\delta}^{\calK}(\xi)  =  h(\xi_{\delta}) + \frac{1}{\delta} |\xi_{\delta}-\xi|^2 \ge \frac{1}{\delta} |\xi_{\delta}-\xi|^2. $$\end{proof}


\begin{remark}
    When the stopping region is the hypograph of the optimal boundary ($\eta =-1$ in \ref{asm:star}) one can employ \textit{sup convolutions} instead, that is
        $$h^{\delta}(\xi) := \sup_{\xi' \in \ \calE}\left[h(\xi') - \frac{1}{\delta} |\xi'-\xi|^2 \right] \ge h(\xi), \quad \delta >0. $$
        We may also define the restriction $h^{\delta}_{\calK}$ to some compact  $\calK\subset \subset \calE$. This case is simpler since u.s.c functions are automatically bounded above in compact sets. 
\end{remark}

The next lemma states that inf convolutions approximate lower semicontinuous functions arbitrarily well with respect to the relaxed $L^\infty$ distance seen in \cref{def:relaxedSupDist}.  
%{\rr{METE:  This is not true.  Take the function $f(x)=1$ for $x \neq 0$ and $f(0)=0$.  It is l.s.c.  The inf-convolution is $f_\delta(x)=\min\{1,x^2/\delta\}$.  The way we defined the norm, the distance between $f-f_\delta$ is always one.  If you define the norm as in $J_1$, then you would get convergence.}}

\begin{lemma}\label{lem:infCovApprox}
          Let $\iota >0$ and $\calK \subset \subset \calE$. If  $f \in \frakF$ is bounded in $\calT\times \calK$, then there exists $\delta>0$ such that 
          $$\rr{d_{\calK} (f,f_{\delta}^{\calK}) \le \iota.}$$
          %$d_{\calK,\calT}(f,f_{\delta}^{\calK}) \le \iota.$
\end{lemma}
\begin{proof}
    Let $\iota >0$. Since $\calK$ is compact, one can choose $(\xi^n)_{n=1}^{N} \subseteq  \calK$, $N< \infty$ such that $\calK \subseteq  \bigcup_{n=1}^{N} B_{\iota /2}(\xi^n)$, where we recall that $B_r(\xi^n) = \{\xi \in \calE \ : \ |\xi-\xi^n| \le r\}$, $r\ge 0$. Fix also $t\in \calT$ and  write $h(\xi) = f(t,\xi)$ for brevity.    As $h$ is l.s.c., there exist $\{r_n\}_{n=1}^N \subset (0,\infty)$ satisfying 
    \begin{equation}\label{eq:lscIota}
        h(\xi^n) \le h(\xi) + \iota/2, \quad \forall \ \xi\in B_{r_n}(\xi^n), \quad n =1,\ldots,N. 
    \end{equation}
If we set $\delta_t = \frac{1}{M} \min_n r_n^2>0$,  $M = \lVert h \rVert_{L^\infty(\calK)}$, then  $\sqrt{\delta_t M} \le r_n$ for all $n$. Consider also for each $n$ a minimizer  $\xi^n_{\delta_t}$  achieving  $h_{\delta_t}^{\calK}(\xi^n)$ in \eqref{eq:infconvCpctDef}.  
In view of  \cref{cor:lsc},  $\xi^n_{\delta_t}$ belongs to  $B_{\sqrt{\delta_t M}}(\xi^n)$. But $B_{\sqrt{\delta_t M}}(\xi^n)\subseteq B_{r_n}(\xi^n)$, which yields 
$$h_{\delta_t}^{\calK}(\xi^n) = h(\xi^n_{\delta_t}) + \frac{1}{\delta_t}|\xi^n - \xi^n_{\delta_t}|^2 \ge h(\xi^n_{\delta_t})  \overset{\eqref{eq:lscIota}}{\ge}  h(\xi^n) - \iota/2. $$
Consequently,  $0\le h(\xi^n) - h_{\delta_t}^{\calK}(\xi^n) \le \iota / 2$ for all $n$. Next, define the quantization map 
$$\psi: \calK \to \{\xi^1,\ldots,\xi^N\}, \quad \psi(\xi) =  \underset{\xi^n} {\text{argmin}} \ |\xi-\xi^n|. $$
If there are several elements in $\{\xi^1,\ldots,\xi^N\}$ achieving $\min_{\xi^n} \ |\xi-\xi^n|$, we  choose the one with smallest index. 
From $\calK \subseteq  \bigcup_{i=1}^{I} B_{\iota /2}(\xi^n)$, it is clear  that $|\psi(\xi) - \xi| \le \iota/2$  for all $\xi \in \calK$, and %, hence $\psi \in \Psi_{r}$. %since $(B_{r}(\xi^n))_{i=1}^I$ covers $\calK$. 
together with  $|h(\xi^n) - h_{\delta_t}^{\calK}(\xi^n)| \le \iota/2$, we conclude that 
$$d_{\calK} (h,  h_{\delta_t}^{\calK}) \le \lVert h\circ \psi -  h_{\delta_t}^{\calK}\circ \psi \rVert_{L^\infty(\calK)} + \lVert  \psi - \text{id}\rVert_{L^\infty(\calK)} \le \iota.$$
Setting $\delta = \min_{t\in \calT} \delta_t >0$ completes the proof.
 \end{proof} 

The next approximation result follows immediately. 
\begin{theorem} \textnormal{\textbf{(Universal approximation of lower semicontinuous functions)}}
\label{thm:LSCUAT}\\
   Let  $ \frakN \subseteq \frakF_c$ be a hypothesis space satisfying Assumption \ref{asm:UAP}. Then for all $f \in \frakF$, $ \iota >0$, and  $\calK \subset \subset \calE$ such that $f$ is  bounded in $\calK \times \calT$, there exists  $g\in \frakN$ such that \rr{$d_{\calK} (f , g) \le \iota.$} % $d_{\calK,\calT}(f,g) \le \iota$. 
\end{theorem}

\begin{proof}
Fix $r,\iota' > 0$,  $\calK \subset \subset \calE$, and $\xi \in \calK$. Using \cref{lem:infCovApprox}, 
$d_{\calK} (f , f_{\delta}^{\calK})\le \iota$ 
for some $\delta > 0$. 
 For every $\gamma>0$, there exists $\psi \in \Psi$ such that 
 $$\lVert f(t,\cdot) \circ \psi - f_{\delta}^{\calK}(t,\cdot) \circ \psi \rVert_{L^{\infty}(\calK)} +  \lVert \psi - \text{id}\rVert_{L^{\infty}(\calK)}\le d_{\calK} (f(t,\cdot), f_{\delta}^{\calK}(t,\cdot)) + \gamma \le \iota' + \gamma, \qquad \forall \ t\in \calT.  $$
    Moreover, as $f_{\delta}^{\calK}(t,\xi)$ is continuous in $\xi$,  we can invoke Assumption \ref{asm:UAP} giving the existence of   $g\in \frakN  \subseteq \frakF_c$ such that $\lVert f_{\delta}^{\calK} - g \rVert_{L^{\infty}(\calT \times \calK)} \le \iota'$.
The triangular inequality therefore yields 
 \begin{align*}
     \lVert f(t,\cdot) \circ \psi - g(t,\cdot) \circ \psi \rVert_{L^{\infty}(\calK)} \le  2\iota' + \gamma, \qquad \forall \ t\in \calT. 
 \end{align*}
Hence,   $d_{\calK}(f,g) \le 2\iota' + \gamma$. Letting $\iota' = \frac{\iota}{2}$ and  $\gamma \downarrow 0$ proves the result.  
\end{proof}

At last, we obtain the following   convergence theorem for lower semicontinuous  boundaries. 
\begin{theorem}\rr{[UPDATE]}
   Let $\frakN \subset \frakF_c$  be a family of universal approximators.  Under Assumption \ref{asm:absCont}, for every $\delta>0$, there exists $\varepsilon=\varepsilon(\delta), \gamma=\gamma(\delta)>0$  such that any $g^{\varepsilon,\gamma} \in \frakN$ with the property $ v(\mu^{\varepsilon}_{g^{\varepsilon,\gamma}}) \ge \underset{g \in   \frakN}{\sup} \  v(\mu^{\varepsilon}_g) - \gamma$ also satisfies,
 $v(\tau_{g^{\varepsilon,\gamma}})\ge v^{\diamond} - \delta$. 
\end{theorem}

\begin{proof} Let $\delta'>0 $ be arbitrary. Using \cref{thm:lscV}, there exist $\delta''>0$, $\calK \subset \subset \calE$, $\iota>0$ such that
\begin{equation}\label{eq:contV}
   \lVert f - f' \rVert_{\widetilde{L^{\infty}}(\calT \times \calK)}\le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho(\iota) + \delta''}\le \delta', \quad \forall f,f'\in \frakF.  
\end{equation}
As $f^{\diamond}$ is locally bounded, we can apply  \cref{thm:LSCUAT} giving the existence of    $g^{\diamond} \in \frakN$ such that 
$\lVert f^{\diamond}  - g^{\diamond} \rVert_{\widetilde{L^{\infty}}(\calT \times \calK)}\le \iota$. 
We conclude  from \eqref{eq:contV}  that $v(\tau_{g^{\diamond}}) \ge v^{\diamond} - \delta'$. As $g^{\diamond}$ is continuous, we can follow Step 2, 3, and 4 in the proof of \cref{thm:convCont}. 
\end{proof}

==> OLD/04-06-2025/Continuity.tex <==
\section{Continuity of the value functional}\label{sec:continuity}
%and consequences
First, we need a distributional assumption on  the process  $\alpha(X) = (\alpha(X_t))_{t\in \calT}$. 
\begin{asm}
\label{asm:absCont}
For every $t\in \calT$, the conditional law of $\alpha(X_t)$  given $\Xi(X_t)$
is absolutely continuous with respect to the Lebesgue measure,
and admits  a  modulus of continuity $\rho_t:[0,\infty) \to [0,1]$ satisfying,
$$
 \Q(\alpha(X_t)\in [a,a+\iota] \ \large{|}\ \Xi(X_t)) \le \rho_t(\iota), \qquad \Q-a.s, \; \forall a, \iota \ge 0.
 $$
\end{asm}
%============ verification of above assumption =========%
\rr{
\begin{example}  Let us verify  Assumption \ref{asm:absCont} for max-call options on $d=2$ assets seen in \cref{ex:maxcall}, namely $\alpha(x) = x_1\vee x_2$ and $\Xi(x) = \frac{x}{\alpha(x)}$. We also suppose that  the  law of $X_t = (X_t^1,X_t^2)$ has no atoms and denote the joint density of $X_t$ by $\phi_t$. If  $\Xi(X_t) \in \calE_b:= \{(1,\xi_2) : \xi_2 \le b \}$, then $\alpha(X_t) = X_t^1$ so that 
\begin{align*}
    \Q(\alpha(X_t)\le a \ \large{|}\ \Xi(X_t) \in \calE_b ) = \Q(X_t^1\le a \ \large{|}\ X_t^2 \le b X_t^1 ) 
    = \frac{1}{\Q(X_t^2 \le b X_t^1)} \int_0^a\int_{0}^{bx_1} \phi_t(x_1,x_2)dx_2dx_1.%\int_{0}^{a} \Q(X_t^2 \le b x_1) \Q(X_t \in dx_1).
\end{align*}\
Hence  for all $b\in \R$ such that $\Q(X_t^2 \le b X_t^1)>0$, we have  $\Q(\alpha(X_t)\in [a,a+\iota] \ \large{|}\ \Xi(X_t) \in  \calE_b) \le \rho_t(\iota)$ as claimed. 
%If $\Xi(X_t) = \xi =  (1,\xi_2)$, $\xi_2\le 1$,  then $\alpha(X_t) = X_t^1$ so that 
% \begin{align*}
%     \Q(\alpha(X_t)\in [a,a+\iota] \ \large{|}\ \Xi(X_t) = \xi ) = \Q(X_t^1\in [a,a+\iota] \ \large{|}\ X_t^2 = \xi_2 X_t^1 ) 
%     = \int_{0}^{\iota} \mathds{1}_{\{x_2 = \xi_2 x_1\} } \Q(X_t \in dx).
% \end{align*}
%If the joint law of $X_t^1,X_t^2$ has no atoms, we conclude that $\Q(\alpha(X_t)\in [a,a+\iota] \ \large{|}\ \Xi(X_t) = \xi ) \le \rho_t(\iota)$ as claimed. 
\end{example}
}
%==========================================%
We are now ready to  state our first  continuity result. Throughout, we adopt the notation $\calK \subset \subset \calE$ if $\calK$ is a compact subset of $\calE$. 
\begin{theorem}\label{thm:unifcontV}
%\textnormal{\textbf{(Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}}
   Let  $C \in (0,\infty)$ given in \cref{lem:TV} and fix $\delta > 0$. Then under Assumptions \ref{asm:absCont},  
    there exists a compact set $\calK \subset \subset \calE$  such that for all $\iota >0$ and  $f,f'\in \frakF$, 
    \begin{equation}\label{eq:unifcontV}
        \lVert f - f' \rVert_{L^{\infty}(\calT \times \calK)}
        \le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho (\iota) + \delta},
    \end{equation}
    where $\rho_t$ is the modulus of continuity of $a \mapsto \Q(\alpha(X_t) \in [0,a] \ | \ \Xi(X_t))$  and $\rho(\iota) = \sum_{t\in\calT} \rho_t(\iota) $.  \rr{If $\calE$ is compact, then $f \mapsto v(\tau_f)$ is uniformly continuous in  the supremum distance. }
\end{theorem}

\begin{remark}\label{rem:bdedDensity}
If Assumption \ref{asm:absCont} holds and for all $t\in \calT$, 
 the density $\phi_t(x)dx := \Q(\alpha(X_t)\in dx)$  is  bounded,  then the cumulative distribution function of $\alpha(X_t)$ is Lipschitz continuous. In particular, its modulus of continuity satisfies $\rho_t(\iota) \le  \lVert \phi_t \rVert_{L^{\infty}(\R)} \iota$. Defining $c = \sum_{t\in \calT}\lVert \phi_t \rVert_{L^{\infty}(\R)}$, we can thus rewrite the right side of \eqref{eq:unifcontV}   as 
    \begin{equation} \label{eq:valueLip}
       \lVert f - f' \rVert_{L^{\infty}(\calT \times \calK)}\le \iota \; \Longrightarrow \; |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{c \ \iota + \delta}. 
    \end{equation}
\end{remark}

\begin{figure}[t]
    \centering
    \caption{Illustration of  
    the symmetric difference between the stopping regions $\frakS_t(f)$ and  $\frakS_t(f')$ (purple region) contained in the interval $[f \wedge f',f \wedge f'+\iota)$ (orange region); see proof of \cref{thm:unifcontV}. The stopping decisions with respect to $f$ and $f'$ coincide in the red (stop) and blue (continue) region. }
    \vspace{-1mm}
    \includegraphics[width = 2.7in,height = 2.0in]{Figures/Viz_Lemma_Paper.pdf}
    
    \label{fig:symdiff}
\end{figure}

\begin{proof} (\cref{thm:convCont}) \underline{\textit{Step ${1}$.}} 
 Since $\calE = \Xi(\calX)$   is locally compact (being the continuous image of a Euclidean space), 
 every finite Borel measure on it 
 is tight. 
Hence,  there exists $\calK \subset \subset \calE$ such that 
 \begin{equation}\label{eq:OmegaK}
   \Q(\Omega_{\calK}) \ge 1-\delta, \quad \Omega_{\calK} := \{\omega \in \Omega \ : \ \Xi(X_t(\omega)) \in \calK  \; \ \forall t\in \calT\}.
\end{equation} 
 \underline{\textit{Step ${2}$.}} Fix $\iota>0$ and $f,f'\in \frakF$ such that   $\lVert f - f' \rVert_{L^{\infty}(\calT \times \calK)}\le \iota$. Using \cref{lem:TV}, then 
$$|v(\tau_{f})-v(\tau_{f'})| \le C \Q(\tau_{f} \ne \tau_{f'})^{1/2},$$
so it remains to find the appropriate upper bound for $\Q(\tau_{f} \ne \tau_{f'})$.   
      First, note that the event $  \{\tau_{f} \ne \tau_{f'}\}$ is contained in   
      $$\tilde{\Omega} = \{\omega \in \Omega  : X_t(\omega) \in \frakS_t(f) \triangle \frakS_t(f')   \ \text{ for some } t\in \calT\}.  $$   
Indeed, for $\omega \notin \tilde{\Omega}$,
the sets $\{t \in \calT  :  X_t(\omega) \in  \frakS_t(f) \}$ and $\{t \in \calT  : X_t(\omega) \in  \frakS_t(f') \}$  are identical. Hence $\tau_{f}(\omega) = \tau_{f'}(\omega)$, which shows that $\Omega \setminus \tilde{\Omega} \subseteq \{\tau_f = \tau_{f'}\}$. 
Next, notice that 
\begin{align*}
     x &\in \frakS_t(f) \triangle \frakS_t(f')   \, \Longleftrightarrow \alpha(x) \in I(t,\Xi(x)), \quad x \in \calX, 
\end{align*}
with the interval $I(t,\xi) := [(f \wedge f')(t,\xi), (f \vee f')(t,\xi))$.   
Since $\lVert f - f' \rVert_{L^{\infty}(\calT \times \calK)}\le \iota$, then  
 $I(t,\xi)$ has  length at most  $\iota$ %$|f(t,\xi)-f'(t,\xi)|  \le \iota$ 
 for every $(t,\xi) \in \calT \times \calK$. See \cref{fig:symdiff} for an illustration.   
Using Assumption \ref{asm:absCont} and recalling that 
$\rho_t$ is the modulus of continuity of $a \mapsto \Q(\alpha(X_t) \in [0,a] \ | \  \Xi(X_t))$, then  %(\rr{METE:  not correct, see below})
\begin{equation}\label{eq:absCont}
   \Q(\alpha(X_t) \in I(t,\Xi(X_t)) )  \le  \rho_t(\iota).
\end{equation}
% {\rr{What we have is the set $\{ \alpha(X_t) \in [A,A+\iota)\}$, 
% for the random variable $A=(f \wedge f')(t,\Xi(X_t))$.  Then, I cannot estimate it as above.  For instance, if $A$ were to be equal to $\alpha(X_t)$ the probability would be one.  Correlations make a difference.  I think better way to go is to observe that this probability would go to zero as $\iota$ goes to zero. }}
We conclude from \eqref{eq:absCont} and 
the union bound  that 
\begin{align*}
    \Q( \tilde{\Omega} \cap   \Omega_{\calK})
    \le \sum_{t\in \calT} \Q(\{\alpha(X_t)\in I(t,\Xi(X_t))\} \cap \Omega_{\calK}  )
    \le \sum_{t\in \calT} \rho_t(\iota) 
    &=  \rho(\iota).
\end{align*}
Combining Step 1 with the above observations, we finally  obtain
\begin{equation*}
  \Q(\tau_{f} \ne  \tau_{f'}) \le   \Q(\{\tau_{f} \ne  \tau_{f'}\} \cap \Omega_{\calK})  + \Q(\Omega \setminus \Omega_{\calK}) \le  \Q( \tilde{\Omega} \cap   \Omega_{\calK})  + \delta 
    \le \rho(\iota) + \delta . 
\end{equation*}  
\end{proof} 

We have the following corollary of \cref{thm:unifcontV}, already stated in \eqref{eq:relaxConv}, proving the  convergence of the values obtained by the relaxed stopping rules to the strict ones. 
\begin{corollary}
    \label{cor:relaxUnif}
Under Assumptions \ref{asm:growth} and \ref{asm:absCont}, for all $\varepsilon >0$ and  $f\in \frakF$, 
    \begin{equation}\label{eq:relaxUnif}
   |v(\mu_{f}^{\varepsilon}) - v(\tau_{f})| \le C\sqrt{\rho (\varepsilon)} ,
\end{equation}
    with $\rho, C$ given in \cref{thm:unifcontV,lem:TV}, respectively. % and  $C \in (0,\infty)$ in \cref{lem:TV}.  
\end{corollary}

\begin{remark}
Under the additional assumption given in \cref{rem:bdedDensity}, equation  \eqref{eq:relaxUnif} becomes, 
    \begin{equation} \label{eq:relaxUnif2}
        |v(\mu_{f}^{\varepsilon}) - v(\tau_{f})| \le \tilde{C}\sqrt{\varepsilon}, 
    \end{equation}
    where $\tilde{C} = C c$ and $c$ defined in \cref{rem:bdedDensity}. We therefore obtain a rate of convergence equal to $1/2$ for the value associated to $\mu_f^{\varepsilon}$ as $\varepsilon \to 0$. 
    \end{remark}

 \begin{proof} (\cref{cor:relaxUnif}) 
  In view of \cref{lem:TV},  $|v(\mu_{f}^{\varepsilon}) - v(\tau_{f})| \le C  \| \textnormal{TV}(\mu_{f}^{\varepsilon},\delta_{\tau_f}) \lVert_{L^2(\Q)}.$ 
  Also by the definition of $\mu_{f}^{\varepsilon}$ in  \eqref{eq:relaxedRule} and the fact that  $\delta_{\tau_f}$ is a (random)  Dirac measure,  the total variation distance simplifies to 
\begin{align}
     \text{TV}(\mu_{f}^{\varepsilon},\delta_{\tau_f}) &= \frac{1}{2} \Big[ 1 - P_{f,\tau_{f}}^{\varepsilon} +  \sum_{t\in \calT\setminus\{\tau_{f}\}} P_{f,t}^{\varepsilon} \Big] = 1 - P_{f,\tau_{f}}^{\varepsilon} \le \mathds{1}_{\{\mu_{f}^{\varepsilon} \ \ne \ \delta_{\tau_{f}}\}} \quad \Q-\text{a.s.} 
\end{align}
     We now claim that  $\{\tau_{(f-\varepsilon)} = \tau_{f}\} \subseteq  \{\mu_{f}^{\varepsilon} = \delta_{\tau_{f}}\}$. Indeed,  if  $\tau_{(f-\varepsilon)}(\omega) = \tau_{f}(\omega)$,  the discrete path $(X_{t}(\omega))_{t\in \calT}$ never enters the fuzzy region  $\frakB_t^{\varepsilon}(f) = \frakS_t(f-\varepsilon) \setminus \frakS_t(f)$ prior to $\tau_f(\omega)$. Thus, the relaxed stopping rule 
     $\mu_f^{\varepsilon}(\omega)$ coincide with $\tau_f(\omega)$. Consequently, %we have 
     $$  
     \lVert \textnormal{TV}(\mu_{f}^{\varepsilon},\delta_{\tau_f}) \lVert_{L^2(\Q)}^2  \le \Q(  \mu_{f}^{\varepsilon} \ \ne \ \delta_{\tau_{f}}) \le   \Q(  \tau_{(f-\varepsilon)} \ne \tau_{f}  ). 
     $$
  We now follow Step 2 in the proof of \cref{thm:unifcontV}  with  $f' = f-\varepsilon$, $\iota =\varepsilon$ to conclude that  $\Q(  \tau_{f-\varepsilon} \ne \tau_{f}  ) \le \rho(\varepsilon)$. We note that as $\lVert f-f'\rVert_{L^{\infty}(\calT\times \calE)} = \varepsilon$, no localization is needed here as done in the proof of \cref{thm:unifcontV}.  
 \end{proof}

==> OLD/04-06-2025/Introduction.tex <==
\section{Introduction}

The  optimal stopping problem, given {in its} simplest form  by
\begin{equation}\label{eq:OS0}
  \sup \left\{ v(\tau) := \E^{\Q}[ \varphi(\tau,X_{\tau})] \ : \ \tau = \text{ stopping time}\right\},
\end{equation}
for a {stochastic} process $X $ and  
a reward function $\varphi$,  
plays a central role in stochastic  optimal control and has applications  
{in numerous quantitative fields}. 
{In mathematical statistics, the theory of optimal stopping 
can be utilized to address sequential tests, such as the quickest detection of a Wiener process} 
\cite{ShiryaevStat, PeskirShiryaev}. 
In mathematical finance, optimal stopping problems emerge naturally from 
the pricing of American or Bermudan contingent claims 
\cite{elKarouiPardouxQuenez,Karatzas,PeskirShiryaev,Schweizer}. 
In this context, $\varphi$ is  the payoff of the claim, $X$ describes 
the price evolution of the underlying asset, and the optimal value in 
\eqref{eq:OS0} gives the initial price of the contract. 
{While the initial} motivation of this paper is to provide 
a convergence study of the neural  stopping boundary
algorithm of  \cite{ReppenSonerTissotDF,ReppenSonerTissotFB},
{our analysis is essentially applicable to all scenarios 
where the exit times play a central role. Consequently,
we present our findings in this broader context, then
analyze the mentioned algorithm using these general results.}

{The unifying structure is the approximate parameterization of 
the \textit{stopping boundaries} 
by feedforward artificial neural networks,
and  the central question revolves around their asymptotic effectiveness.
In fact, the algorithm developed in \cite{ReppenSonerTissotFB}
computes the \textit{stopping} (or \textit{exercise}) \textit{region} 
for Bermudan options. 
Following \cite{ReppenSonerTissotFB},
we assume that in an appropriate coordinate system
the optimal stopping region is an epigraph (or a hypograph) 
of a function $f^{\diamond}$, and consequently, }
the hitting time of  $f^{\diamond}$ is  optimal for \eqref{eq:OS0}. 
Hence, we can restrict the set of stopping times in \eqref{eq:OS0} to hitting times of boundaries.
Namely,
\begin{equation}\label{eq:OS0f}
  \sup \left\{ v(\tau_f) := \E^{\Q}[ \varphi(\tau_f,X_{\tau_f})] \ : \ f = \text{ stopping boundary} \right\},
\end{equation}
where $\tau_f$ is the hitting time of the epigraph (or hypograph) of $f$.
{In the neural boundary algorithm, networks approximate $f^{\diamond}$,
and the convergence analysis of this method
relies mainly on the properties of the relaxation of the hitting times,
and the continuity of the map from the boundaries 
to the expected value of the corresponding stopping policy,
as proved in \cref{sec:relaxation,sec:continuity}, respectively.}

{It is well-known that, training with 
stochastic gradient descent of loss functions 
computed via hitting times results in vanishing gradient,
and as in the \textit{deep optimal stopping} of  \cite{Becker1,Becker2} and in \cite{ReppenSonerTissotFB},
relaxed stopping must be introduced.
Relegating the} 
technical details to \cref{sec:relaxation}, 
the relaxed version of problem \eqref{eq:OS0}  is given by,
\begin{equation}\label{eq:relax0}
    \sup\left\{ v(\mu) := \E^{\Q}\left[\int \varphi(t,X_{t}) \mu(dt) \right] \ : \ \mu =  \text{ random probability measure}\right\}.
\end{equation}

Also called \textit{convexification} \cite{Acikmese} or \textit{compactification}     
\cite{ElKaroui}, relaxation procedures such as \eqref{eq:relax0} are 
classically used in stochastic control problems to prove the existence of an optimal solution \cite{FlemingDomokos,Haussmann_Lepeltier,McShane}. 
Indeed, {relaxation convexifies the problem allowing 
for numerous methods and tools for its analysis. 
Moreover, as we prove in  \cref{prop:relaxOS},
both  \eqref{eq:OS0} and \eqref{eq:relax0} achieve the same optimal value. 
Indeed, this holds essentially in all other} contexts; 
see, e.g.,  \cite{Gyongy,Hobson} and \cite[Lemma 1.5.2.]{Krylov} 
for continuous time  optimal stopping, and 
\cite{ElKaroui,FlemingDomokos,Haussmann_Lepeltier} for general stochastic optimal control.  

In the neural optimal stopping boundary method,
the stopping policy is relaxed by introducing a \textit{fuzzy} region around the boundary
{with a small width  $\varepsilon>0$}. 
The stopping decision remains the same  outside the fuzzy region, while inside, 
the former is replaced by stopping intensities  proportional to the signed distance to the boundary. 
This procedure generates   \textit{relaxed} hitting times of boundaries$-$namely random  
probability measures supported  on the set of exercise dates. 
The relaxed problem \eqref{eq:relax0} thus becomes
\begin{equation}\label{eq:relax1}
\sup\left\{ v(\mu_f^\varepsilon) := \E^{\Q}\left[\int \varphi(t,X_{t}) 
{\mu_f^\varepsilon}(dt) \right] \ : \   {\mu_f^\varepsilon} =  \text{relaxed hitting time of $f$}\right\}.
\end{equation}
As shifting the boundary ever so slightly changes the stopping intensities inside the fuzzy region, the above relaxation makes stochastic gradient methods applicable. The fuzzy region is akin to the \textit{mushy zone} between two phases (typically solid and liquid) in phase-field models \cite{B-mushy,Soner,V-mushy}. The introduction of a  fuzzy  region is critical in other deep learning algorithms as well,  such as  occupation networks in  computer vision  \cite{OccupancyNN} or deep level-set functions for solving Stefan problems  \cite{SST}. 

{Our central results of continuity are proved in 
\cref{sec:continuity}}. In particular, \cref{thm:unifcontV,thm:lscV} establish the continuity
of the value functional $\frakF \ni f \mapsto v(\tau_f)$, 
where $\frakF$ is a set of stopping boundaries. 
Formally, these results are in the following form.

\begin{theorem*}\label{thm:unifcontV0}
\textnormal{\textbf{(Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}} 
Let $\lVert \cdot \rVert$ be a norm on $\frakF$. Then for all $\delta>0$, there exists $\iota  >0$ such that for all $f, f' \in \frakF$,
\begin{equation}\label{eq:unifcontV}
  \lVert f - f' \rVert \le \iota \ \Longrightarrow   \ |v(\tau_{f}) - v(\tau_{f'})| \le \delta. 
\end{equation}
\end{theorem*}

% \begin{theorem*}\label{thm:unifcontV0}
% \textnormal{\textbf{(Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}} 
% Let $\mathfrak{m}$ be a metric on $\frakF$. Then for all $\delta>0$, there exists $\iota  >0$ satisfying 
% \begin{equation}\label{eq:unifcontV}
% \forall f,f' \in \frakF \ \text{ such that } \  \mathfrak{m}( f,f') \le \iota \ \Longrightarrow   \ |v(\tau_{f}) - v(\tau_{f'})| \le \delta. 
% \end{equation}
% \end{theorem*}
\noindent
{Indeed, while \cref{thm:unifcontV} employs the supremum norm,
we consider a weaker topology induced by the 
\textit{relaxed $L^{\infty}$ norm}  %(see   \cref{def:relaxedSupDist})
in \cref{thm:lscV}
to accommodate  boundaries that are only semi-continuous}. \rr{Concretely, the relaxed $L^{\infty}$ norm is defined as %pseudometric  is given %for each time section 
 (see \cref{sec:relaxLinfty} %\cref{def:relaxedSupDist} 
 for a more precise definition)
  \begin{align}
          \varrho( f )
          &= 
          \inf_{\psi\in \Psi}  \ \lVert f\circ \psi\rVert_{\infty} + \lVert \psi - \text{id} \rVert_{\infty}, \label{eq:relaxDistH}
 \end{align}
 where $\Psi$ contains all endofunctions $\psi:\calE \to \calE$ and $\text{id}$
is the identity map. 
 Strictly speaking,  $\lVert \cdot \rVert_{\widetilde{L^{\infty}}}$ is a quasinorm since it is not subadditive. %[OR IS IT?]
The distance associated to the relaxed $L^{\infty}$ norm  thus uniformly compares  boundaries $f,f'\in \frakF$, possibly after a local transformation of the domain.  
This relaxation is 
similar to the Skorokhod $J1$ distance  for càdlàg processes. %This pseudometric 
The relaxed $L^{\infty}$ norm is also inspired by the inf/sup convolution,  which is an effective regularization 
tool widely used in the theory of viscosity solutions 
\cite{FS, LasryLions}. In particular, they provide a systematic way of approximating lower semi-continuous
functions from below. } 



An immediate corollary, \cref{cor:relaxUnif}, 
is the convergence  of the value \eqref{eq:relax1}
associated to the relaxed stopping times
to the value using the same interface  as the width $\varepsilon$ of the fuzzy region tends to zero.   

 In \cref{sec:NOSB}, we combine the above results and provide a convergence 
 analysis of the \textit{neural optimal stopping boundary} algorithm \cite{ReppenSonerTissotFB}. 
Briefly, this algorithm looks for a \textit{neural stopping boundary}, 
namely a \textit{feedforward neural network} $g^{\theta}$   
such that 
$$
{v(\mu_{g^\theta}^\varepsilon)} \approx v(\tau_{g^{\theta}}) \approx \sup_{f\in \frakF}
v(\tau_f) \  = v(\tau_{f^{\diamond}}).
$$ 
The parameter vector $\theta$ is then trained by 
maximizing the relaxed reward $v(\mu_{g^\theta}^\varepsilon)$ using stochastic gradient ascent.  
{The following result  (also see \cref{thm:convCont}) implies
the  convergence of the algorithm employed in \cite{ReppenSonerTissotFB}.}
\begin{theorem*}\label{thm:convCont0} \textnormal{\textbf{(Convergence)}}
For all  $\delta>0$,  there exists $\varepsilon>0$ and a feedforward  
neural network  $g^{\theta}$ such that ${v(\mu_{g^{\theta}}^\varepsilon)}\ge v(\tau_{f^{\diamond}}) - \delta$. 
\end{theorem*}
\noindent
When the optimal stopping boundary $f^{\diamond}$ is continuous, 
one can apply the  Universal Approximation 
Theorem \cite{Cybenko,Hornik} stating  that any continuous function can be 
approximated arbitrarily well by  feedforward neural networks in  compact sets. 
{This together} with the continuity of $f \mapsto v(\tau_f)$,
{implies the above result.}
{However}, the optimal stopping boundary $f^{\diamond}$ 
may fail to be continuous, preventing the use of the Universal Approximation Theorem. 
{Nevertheless,  under mild assumptions, the stopping boundary is  
shown to be semicontinuous in \cref{prop:lscBdry}.  

Motivated by this, we first extend in \cref{thm:LSCUAT} the Universal Approximation Theorem 
by proving that semicontinuous functions can be 
approximated by neural networks  in the 
\textit{relaxed $L^{\infty}$ distance} introduced in  Definition \ref{def:relaxedSupDist}. 
This is achieved through inf-sup convolutions
recalled in \cref{sec:convLSC}.   
%which is an effective regularization 
%tool widely used in the theory of viscosity solutions
%(see, for example,  \cite[Section V.5]{FS} and \cite{LasryLions}).
This approximation together
with  \cref{thm:lscV} and the semicontinuity of $f^\diamond$
enables us to prove the above 
theorem. 
Incidentally, we suggest that the universal approximation
proved in \cref{thm:LSCUAT},}
is an interesting result in its own right 
and can be applied to other tasks  involving the approximation of  semicontinuous functions.

There is a recent body of literature on the convergence of deep learning methods in stochastic optimal control:  \citet{Hure} study the convergence  of discrete time stochastic control problems involving policy and/or value iteration; \citet{LapeyreLelong} prove the convergence of the Longstaff-Schwartz algorithm \cite{LSMC} using neural networks to approximate the continuation value; 
\citet{Gonon} sheds light on the expressivity and maximal size  of   neural networks to produce optimal stopping rules.  
{Additionally,}  \cite[Proposition 4]{Becker1} of the \textit{deep optimal stopping} paper 
 provies the near optimality of deep stopping strategies. 
 {A common property used in all these papers is dynamic programming,
 while} the neural optimal stopping boundary algorithm 
  \cite{ReppenSonerTissotFB} constructs an optimal stopping rule in a forward fashion.
  Consequently, our convergence analysis  necessitates 
  other techniques and tools, and differs greatly from previous works.  

\textbf{Structure of the paper.} In \cref{sec:OS}, we introduce the optimal stopping problem,  our main structural assumption on the exercise region, and give financial examples. In \cref{sec:relaxation}, we define the fuzzy region and construct relaxed stopping rules. \cref{sec:continuity} establishes the  continuity of the map $f\mapsto v(\tau_f)$ as well as important consequences. In \cref{sec:NOSB}, we prove the convergence of the neural optimal stopping boundary method in the continuous and semicontinuous case, respectively.  \cref{sec:conclusion} provides  concluding remarks and \cref{app:relaxedproblem} contains the proof of \cref{prop:relaxOS}. 

==> OLD/04-06-2025/Problem.tex <==
\section{Optimal stopping}\label{sec:OS}
 Let $\calT \subset [0,\infty)$  a  finite subset of  time indices containing $0$ and
$(\Omega, \F = (\calF_t)_{t \in \calT},\Q)$ a filtered probability space. 
The state $X = (X_t)_{t\in \calT}$
is an $\F$-adapted, Markov process which take values in a Euclidean space $\calX$. We assume for concreteness that $\F$ is the  filtration generated by $X$.
 Given a \emph{reward (or payoff) function} $\varphi:\calT \times \calX \to \R$,  the associated \emph{optimal stopping problem}  is to 
\begin{equation}
\label{eq:OS}
\text{maximize}
\ \ 
v(\tau):=  \E^{\Q}[ \varphi(\tau,X_{\tau})],
\qquad
\text{over}\  \tau \, \in \, \vartheta(\calT),
\end{equation} 
where 
$\vartheta(\calT)$ is the set of 
$\calT$-valued $\F$-stopping times.
Problem $\eqref{eq:OS}$ is well-defined (and non-trivial) if   $\max_{t\in \calT}|\varphi(t,X_t)| \in L^1(\Q)$. We write $v^{\diamond}$ for the optimal  value of \eqref{eq:OS}. %We write $\tau^{\diamond}$ for the optimal stopping time,  with  corresponding value  $v^{\diamond} = v(\tau^{\diamond})$. 
The following assumption on $\varphi$ and the dynamics of $X$ will prove useful.  
\begin{asm}%{\rm{\bf{(Growth and continuity)}}}
\label{asm:growth}
There exists $a>0$ 
such that 
$\varphi(t,\cdot) \in \calL_a \ \forall \ t \in \calT$, where 
\be
\label{e.lca}
\calL_{a}:= \left\{ \phi \in \calC(\calX;\R) \ : \ 
|\phi(x) | \le C[1+|x|^a]\ \
\text{for some}\ C>0 \right\}.
\ee
Also, we suppose that $\phi \in \calL_a \Longrightarrow K_{t,s} \phi \in \calL_a$ $\forall \  t, s \in \calT$, with the transition semigroup
\begin{equation}\label{eq:semigroup}
    K_{t,s} \phi(x)=
\E[ \phi(X_{s}) \mid X_{t}=x], \quad x\in \calX, \quad t<s. 
\end{equation}
\end{asm}

Allowing the second component of  $K_{\cdot,\cdot}$  in \eqref{eq:semigroup} to be a stopping time,  
define  the value function  
\begin{equation}
    v^{\diamond}(t,x)= \sup_{t \le  \tau \in \vartheta(\calT )}
K_{t,\tau} \varphi(\cdot, x) \ , 
\end{equation}%\mathds{1}_{\{\tau\ge t\}}
and stopping region
$\calS_t = \{x\in \calX  :   \varphi(t,x) = v^{\diamond}(t,x)\}, \ t\in \calT. $
We then have the following result, proved in \cite{ReppenSonerTissotFB}. 
\begin{proposition}
\label{prop:closedStopRegion} Under Assumption \ref{asm:growth},
the value function $v(t,\cdot)$ belongs to $ \calL_a$ for each $ t\in \calT$. In particular, $v^{\diamond}(t,\cdot)$ is continuous and the stopping region $\calS_t$ is a relatively closed subset of $\calX$
.
\end{proposition}

Similar to   \cite{ReppenSonerTissotFB}, we make the following structural  assumption  %on the stopping region,
yielding the existence of a  \textit{stopping boundary} (or \textit{free boundary})   delimiting the stopping region in a problem specific coordinate system. 
\begin{asm}%{\rm{\bf{(Existence of a stopping boundary)}}}
\label{asm:star}
There exist  measurable functions
$$
\alpha: \calX \to \R_+,
\quad
\Xi: \calX \to \calE := \Xi(\calX),
\quad
 f^{\diamond}: \calT \times \ \calE \to [0,\infty],
 $$
 % \begin{align*}
 % &\alpha: \calX \to \R_+, \\ 
 % &\Xi: \calX \to \calE := \Xi(\calX), \\ 
 %     &f^{\diamond}: \calT \times \ \calE \to [0,\infty],
 % \end{align*}
 such that $A = (\Xi,\alpha): \calX \to  \calE \times \R_+$ is a homeomorphism
 and for every $t \in \calT$,
\be
\label{e.st}
\calS_t = \{  x \in  \calX \ :\
\eta \left(f^{\diamond}(t,\Xi(x))-\alpha(x)\right) \le 0  \}, \qquad \eta \in \{-1,1\}. 
\ee 
\end{asm}
We suppose that the \textit{latent space} $\calE$ is itself  a subset of a Euclidean space (e.g. $\R^m$ for some $m\ge 1$) and write $|\xi|$ for the norm of $\xi\in \calE$. 
 Under the above assumption, the \textit{optimal stopping boundary} is thus given by 
\begin{align}\label{eq:stopBdry}
    f^{\diamond}(t,\xi) = \begin{cases} 
    \inf\{a \ge 0 \ : \ A^{-1}(\xi,a) \in \calS_t\}, & \eta = 1, \\[0.5em]
    \sup\{a \ge 0 \ : \ A^{-1}(\xi,a) \in \calS_t\}, & \eta = -1.
    \end{cases}
\end{align}
\begin{figure}[t]
\caption{Stopping region of a max-call option on two symmetric assets. The upper connected component becomes an epigraph through $(\alpha,\Xi)$ \rr{(right panel), where we   identify $\Xi(x) = (\frac{x_1}{x_2},1) \in \R^2$ with its first component.} Figures adapted from \cite{ReppenSonerTissotFB}.  } 
\vspace{-2mm}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \caption{Stopping region in $\calX$}
    \includegraphics[height=2.0in,width=2.3in]{Figures/vizMaxCall.pdf}
    \label{fig:X}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \caption{Stopping region through $(\alpha,\Xi)$}
    \includegraphics[height=2.0in,width=2.3in]{Figures/vizMaxCallHomeo.pdf}
    \label{fig:homeo}
\end{subfigure}
\label{fig:homeomorphism}
\end{figure}  
%\noindent 
Consequently, the time $t$ section of the stopping region is the epigraph  of $f^{\diamond}(t,\cdot)$ when  $\eta =1$; see \cref{fig:homeomorphism}. Similarly, $\calS_t$ is the hypograph of $f^{\diamond}(t,\cdot)$ when $\eta =-1$. We refer the reader to \cite{BroadieDetemple} for further  information on the structure  of the stopping region and to \cite{Laurence} for a deep proof of the regularity of the boundary.  Additionally, classical books \cite{Velichkov,Petrosyan}  provide  a thorough treatment of the free boundary regularity in one-phase problems and respectively, in obstacle problems. 
For completeness, next we prove the following  simple properties  of $f^{\diamond}$. 
\begin{proposition} \label{prop:lscBdry}
    For every $t\in \calT$, the map $\xi \mapsto f^{\diamond}(t,\xi)$ is lower (respectively upper) semicontinuous when  $\eta =1$ (resp. $\eta = -1$). Moreover, if the payoff function $\varphi$ is convex in $x$, then $f^{\diamond}$ is locally Lipschitz continuous. % \bb{(convex if $\eta=1$ and concave if $\eta=-1$?).} 
\end{proposition}
\begin{proof}
   Fix $t\in \calT$ and prove the result for $\eta=1$. Similar arguments can be applied for the case   $\eta=-1$.  
    Let $\xi \in \calE$ and $(\xi_n) \subset \calE$ such that $\xi_n \to \xi$ and fix $\varepsilon >0$. In light of $\eqref{eq:stopBdry}$,    there exists $a_n \in \R_{+}$ such that $x_n := A^{-1}(\xi_n,a_n)\in \calS_t$ and $f^{\diamond}(t,\xi_n) \ge a_n - \varepsilon$ for every $n\in \N$.  Defining $a = \limsup_{n\to \infty} a_n,$ then %$\liminf_{n\to \infty} f^{\diamond}(t,\xi_n) \ge a - \varepsilon.$
    \begin{equation*}
        \liminf_{n\to \infty} f^{\diamond}(t,\xi_n) \ge a - \varepsilon. 
    \end{equation*}
    Next, the continuity of $A^{-1}$ yields  $\lim_{k\to \infty} x_{n_k} = x := A^{-1}(\xi,a) $ for a subsequence $(n_k)$ such that $a_{n_k} \to a$.  As $(x_{n_k}) \subset \calS_t$ and  $\calS_t$ is closed (see \cref{prop:closedStopRegion}), then  $x \in \calS_t$. Therefore $a \ge f^{\diamond}(t,\xi)$, giving  
    $\liminf_{n\to \infty} f^{\diamond}(t,\xi_n) \ge f^{\diamond}(t,\xi) - \varepsilon.$ 
   Letting $\varepsilon\to 0$ indeed shows the lower semicontinuity of  $\xi \mapsto f^{\diamond}(t,\xi)$. 
    
For the second assertion, it is shown in \cite{BroadieDetemple} that the convexity of  $x \mapsto \varphi(t,x)$ carries over to $\calS_t$.  In particular,  $f^{\diamond}$ is   locally Lipschitz continuous.
\end{proof}

In the remainder of the paper, 
to simplify the exposition we assume  that $\eta =1$, and the case $\eta = -1$ follows \emph{mutadis mutandis}. For fixed maps $(\Xi,\alpha)$ that satisfies Assumption \ref{asm:star} with $\eta =1$,  the corresponding optimal stopping boundary $f^{\diamond}(t,\xi)$ is therefore  lower semicontinuous (l.s.c.)~in $\xi$ for all $t\in \calT$, and we set 
$$
\frakF := \{f:\calT \times \ \calE \to [0,\infty], \;  f(t,\cdot) \text{ l.s.c. } \forall t \ \in \calT\}.
$$ 
We associate to each $f\in \frakF$ the \emph{stopping region}
\begin{equation}
    \frakS_t(f) = \{x\in \calX \ : \ \alpha(x) \ge f(t,\Xi(x)) \},
\end{equation}
and  the \emph{hitting time}
$\tau_f = \inf\{t \in \calT  :  X_t \in \frakS_t(f)\}$.  Assumption \ref{asm:star} implies in particular that it is enough to consider hitting times of  boundaries to achieve the optimal value in  \eqref{eq:OS}. Namely,
$$
v^{\diamond} = \sup_{f\in \frakF}v(\tau_f)  = v(\tau_{f^{\diamond}}),
$$  
as already shown in \cite[Lemma 2.3]{ReppenSonerTissotFB}. Problem \eqref{eq:OS} is therefore  equivalent to finding $f\in \frakF$ such that $\frakS_t(f) = \calS_t$ for all $t \in \calT$. %Indeed, \cref{asm:star} guarantees the existence of an optimal  boundary 

\subsection{Financial examples}\label{sec:finEx}
Suppose that $X = (X^1,\ldots,X^m)$ describes the price process of $m\ge 2$ financial assets. The state space is  therefore  $\calX = \R^m_+$.   Moreover,  consider payoff functions of the form 
\begin{equation}
\varphi(t,x) = e^{-rt}(\alpha(x)-\kappa)^+,
\end{equation}
where $r\ge 0$ is a constant interest rate, $\kappa>0$ is the \textit{strike} of the option,  and $\alpha:\calX\to [0,\infty]$ is a statistic of the underlying prices.  
For this class of contracts,    Assumption \ref{asm:star} holds  with  $\eta=1$, and the homeomorphism $A = (\Xi,\alpha)$,  $\Xi(x)=\frac{x}{\alpha(x)}$. See Theorem 4.1 in \cite{ReppenSonerTissotFB} for a  complete  statement. %The stopping region and its image through $(\alpha,\Xi)$ is displayed in \cref{fig:homeomorphism} for a max-call option (see \cref{ex:maxcall}) on $m=2$ symmetric assets. %Similarly, one can consider payoffs of the form $\varphi(t,x) = e^{-rt}(\kappa - \alpha(x))^+$ and apply the same homeomorphism. 

\begin{example}\label{ex:maxcall}
     Consider a \textit{max-call option}, which is obtained by choosing  $\alpha(x)  = \max_{i=1,...,m}x^i$. Hence $\varphi$ is convex in $x$, and \cref{prop:lscBdry} tells us that the stopping boundary is locally Lipschitz continuous.   Moreover, we have the latent space   $\calE =  \{\xi \in [0,1]^m  :  \max_{i=1,...,m}\xi_i=1  \}$; see  Assumption \ref{asm:star}. In particular, it is compact. Interestingly, the stopping region consists of $m$ connected components, as can be seen in \cref{fig:X} in the case of $m=2$ assets. The right panel (\cref{fig:homeo}) displays  the image through $(\alpha,\Xi)$ of the upper connected component of the stopping region in \cref{fig:X}. Although $\calE$ is a subset of $[0,1]^2$, we can    identify $\Xi(x) = (\frac{x_1}{x_2},1)$ with its first component when $x_2 \ge x_1$, as depicted in \cref{fig:homeo}.  %and  only display the one-dimensional quantity ratio $\frac{x_1}{x_2} \in [0,1]$ 
     
     
     Max-call options are popular benchmark examples for numerical methods addressing high-dimensional optimal stopping problems; see \cite[Section 8]{ReppenSonerTissotFB} and the references therein. Indeed,  the maximum function in the payoff makes the problem  truly high-dimensional in the sense that the process $\alpha(X)$ cannot be replaced by a one-dimensional diffusion with identical law. 
\end{example}

\begin{example} \label{ex:minmax} 

If $\alpha(x) = \min_{i=1,...,m}x^i$, then the associated contract is  a so-called \textit{min-call option}.  
Note that the payoff $\varphi(t,x)$ is \textit{not} convex in $x$, leading to pathological properties of the stopping region prior to maturity as  
 studied by \citet{DetempleMin} in the case $m=2$. In particular,   $\partial \calS_t$ contains a nonempty singular set given by a segment on the diagonal $\{x_1 = x_2\}$; see \cref{fig:minX}.
%Setting $\Xi(x) = \frac{x_1 \vee x_2}{x_1 \wedge x_2} \in \calE = [1,\infty)$ for simplicity,
Consequently, the boundary $\xi \mapsto f^{\diamond}(t,\xi)$ is discontinuous at $\xi = (1,1)$, hence strictly (lower) semicontinuous; see \cref{fig:minae}. % The lower semicontinuity of the stopping boundary  may therefore  be strict, even for seemingly simple examples. 
\end{example}

\begin{figure}[H]
\caption{Stopping region of a min-call option on two symmetric assets (one time section). We note that the stopping boundary is discontinuous at $\Xi(x) = (1,1)$. }%strictly lower semicontinuous in the $(\alpha,\Xi)$ coordinate (right chart).  } 
\vspace{-2mm}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \caption{Stopping region in $\calX$}
    \includegraphics[height=2.0in,width=2.3in]{Figures/vizMinCall 2.pdf}
    \label{fig:minX}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \caption{Stopping region through $(\alpha,\Xi)$}
    \includegraphics[height=2.0in,width=2.3in]{Figures/vizMinCallXiA 2.pdf}
    \label{fig:minae}
\end{subfigure}
\label{fig:mincall}
\end{figure}  

==> OLD/04-06-2025/Relaxation.tex <==
\section{Relaxed stopping rules}\label{sec:relaxation}

%Consequently, $v(\tau_{f^{\diamond}}) = v(\tau^{\diamond})  = v^{\diamond} $. % as well.  

To find an optimal boundary with stochastic gradient techniques as  in \cref{sec:NOSB}, the optimal stopping problem needs to be relaxed. Indeed, the map $f \mapsto \tau_f(\omega)$ is piecewise constant for $\Q$-almost every $\omega \in \Omega$ as the hitting time of $f$, taking values in the discrete set $\calT$,   is typically unchanged when  the stopping  boundary varies slightly. This in turn leads to severe vanishing gradient problems. We overcome this difficulty by approximating $\tau_f(\omega)$ by a sequence of relaxed  stopping rules based on \textit{fuzzy regions} parametrized by $\varepsilon>0$, 
\begin{equation}\label{eq:fuzzy1S}
\frakB_t^{\varepsilon}(f) := \frakS_t(f-\varepsilon) \setminus \frakS_t(f) = \{x\in \calX \ : \ d(t,x;f) \in (0, \varepsilon] \}, 
\end{equation}
where $d:\calT\times \calX \times \frakF \to [0,\infty]$ is the distance from $x$ to $\frakS_t(f)$ in the coordinate system $(\Xi,\alpha)$,
\begin{equation}\label{eq:distFct}
    d(t,x;f) =   (f(t,\Xi(x)) - \alpha(x))^{+}, \quad (t,x,f)\in \calT \times \calX \times \frakF,  
\end{equation} 
and an illustration is given in the left panel of \cref{fig:fuzzy&phaseIndicator}. 

We continue by first defining the general relaxed stopping rules, and then  the specific one induced by the fuzzy region. Let $\calP(\calT)$ be the set of probability measures on $\calT$ and $\underline{\vartheta}(\calT)$ denotes the set of $\calP(\calT)-$valued  random variables $$\mu(\omega) = \sum_{t\in \calT} P_t(\omega) \delta_t, \quad \omega \in \Omega, \qquad (\delta_t: \text{Dirac measure at $t$})$$ 
such that the process $(P_t)_{t\in \calT}$ is  $\F$-adapted. 
%such that the process $$t\mapsto \mu(\omega)(\calT_t), \quad  \calT_t := \calT \cap \ [0,t],$$ is  $\F$-adapted. %$ \omega \mapsto \mu(\omega)(\{t\})$ is $\calF_t-$measurable for all $t\in \calT$. 
In this context, $\underline{\vartheta}(\calT)$ is the set of \textit{relaxed} (or \textit{randomized}) $\F$-stopping times taking values in $\calT$. If we identify $\tau \in \vartheta(\calT)$ with %the Dirac measure 
$\delta_{\tau} \in \underline{\vartheta}(\calT)$, then   $\underline{\vartheta}(\calT)$ contains all  $\F$-stopping times. Indeed, this procedure is effectively  a \textit{convexification} of the stopping times as every relaxed stopping rule is  a random convex combination of the Dirac measures $(\delta_t)_{t\in \calT}$.  
We can now define the value functional
\begin{equation}\label{eq:relaxValue}
v(\mu) = \E^{\Q}\left[\int_{\calT} \varphi(t,X_{t}) \mu(dt) \right],\quad  \mu \in \underline{\vartheta}(\calT).
\end{equation}
%If $\mu = \sum_{t\in \calT} P_t \delta_t$, then \eqref{eq:relaxValue} reads 
%$$v(\mu) = \E^{\Q}\left[\sum_{t\in \calT} P_t \varphi(t,X_t) \right]. $$
The \emph{relaxed optimal stopping problem} amounts to maximizing $v(\mu)$ over all $\mu \in \underline{\vartheta}(\calT)$. 
Importantly,  the  relaxed  problem and classical one   \eqref{eq:OS} achieve the same optimal value as we prove in the next proposition. 
Similar results in continuous time can be found in \cite{Gyongy}, \cite{Hobson} and \cite[Lemma 1.5.2]{Krylov}. %, that is $\sup_{\mu \in \underline{\vartheta}(\calT)} v(\mu) = v^{\diamond}$. 

\begin{proposition}\label{prop:relaxOS}
Let $v^{\diamond}$ be the  value of the classical optimal stopping problem \eqref{eq:OS}. 
Then, 
\begin{equation}\label{eq:OSvsRelax}
      \sup_{\mu \in \underline{\vartheta}(\calT)} v(\mu)  = v^{\diamond}.
\end{equation}
 Moreover, any maximizer $\mu^{\diamond}$
 of $ \mu \mapsto v(\mu)$ is a  stopping time, i.e. $\mu^{\diamond} = \delta_{\tau^{\diamond}} $ for some $\tau^{\diamond} \in \vartheta(\calT)$. 
\end{proposition}
\begin{proof}
See \cref{app:relaxedproblem}.
\end{proof}
  
We next construct a relaxed stopping rule from a given boundary $f\in \frakF$ and a fuzziness parameter $\varepsilon>0$. Set $\calT_{t-} = \calT \cap \  [0,t)\ $ for $t>0$ and $\calT_{0-} = \varnothing$, and recursively define the $[0,1]-$valued  stochastic process $P^{\varepsilon}_f = (P_{f,t}^{\varepsilon})_{t\in \calT}$  representing  stopping probabilities by,
\begin{align}\label{eq:stopProb}
     P^{\varepsilon}_{f,t} = \underbrace{p_{f,t}^{\varepsilon}}_{\text{stop at $t$}} \ \ \underbrace{\Big(1- \sum_{s \in \calT_{t-}} P_{f,s}^{\varepsilon}  \Big)}_{\text{continue until $t$}}, \qquad 
     p_{f,t}^{\varepsilon} = (\chi^{\varepsilon}\circ d)(t,X_t;f), 
\end{align}
with the relaxed phase indicator function $\chi^{\varepsilon}(\delta) = (1 - \delta/\varepsilon)^+ \wedge 1$. 
Specifically, $\chi^{\varepsilon}$ is equal to one in the stopping region $\frakS_t(f)$, it is linearly decreasing in the fuzzy region $\frakB_t^{\varepsilon}(f)$, and is zero otherwise. The right panel of \cref{fig:fuzzy&phaseIndicator} displays the composition $\chi^{\varepsilon} \circ d$ in the space $\Xi(\calX) \times \alpha(\calX)$. 
We can now define the relaxed stopping rule associated to $f$ as 
\begin{equation}\label{eq:relaxedRule}
    \mu^{\varepsilon}_f(\omega) = \sum_{t\in \calT} P^{\varepsilon}_{f,t}(\omega) \  \delta_{t}. 
\end{equation}

\begin{figure}[t]
\caption{Left panel: fuzzy region (purple) separating the interior of the continuation region (blue) from the stopping region (red). Right panel: Illustration of $\chi^{\varepsilon} \circ d(\cdot; f)$ in the coordinates $(\Xi,\alpha)$, where $d(\cdot; f)$ is the distance function to $\frakS_t(f)$ and  $\chi^{\varepsilon}(\delta) = (1 - \delta/\varepsilon)^+ \wedge 1$.} 
\vspace{-1mm}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[height=2.0in,width=2.5in]{Figures/fuzzy_Bdry_Paper.pdf}
    \label{fig:fuzzybrdy}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
    \centering
         \includegraphics[height = 2.0in,width = 2.5in]{Figures/fuzzy_3D_Paper.png}
     \label{fig:hFunction}
\end{subfigure}
\label{fig:fuzzy&phaseIndicator}
\end{figure}  
\noindent
Using \eqref{eq:stopProb}, we directly verify that $\mu_f^{\varepsilon}(\omega)(\calT) = 1$. Additionally, as for each $t$, $P^{\varepsilon}_{f,t}$ depends only on $\{X_s \ : \ s \in \calT\cap \  [0,t] \}$, $P^{\varepsilon}_{f}$ is adapted to $\F$. Hence,  $\mu_f^{\varepsilon}$ is a relaxed $\F-$stopping time.

To complete the approximation, in \cref{cor:relaxUnif} we prove the following convergence which was already argued in \cite[Lemma B.1]{ReppenSonerTissotFB},
\begin{equation}\label{eq:relaxConv}
    v(\mu_{f}^{\varepsilon}) \longrightarrow v(\tau_{f}) \quad \text{as } \ \varepsilon \downarrow 0.
\end{equation}
That is, the value of the relaxed stopping rule  $\mu_f^{\varepsilon}$ converges to the expected reward  from  the hitting time of $f$ when the fuzzy parameter $\varepsilon$ decreases to zero. 

The above result is  a byproduct of the continuity of  $f\mapsto v(\tau_f)$, proved in the next section.   
Towards our main results \cref{thm:unifcontV,thm:lscV}, we start with a  
continuity lemma for relaxed stopping rules with respect to  
the \textit{total variation distance} of probability measures, 
$$  \textnormal{TV}(\mu,\mu') = \frac{1}{2}\sum_{t\in \calT} |\mu(\{t\}) - \mu'(\{t\})|\in [0,1], \qquad \mu, \mu' \in \calP(\calT).$$
Note that when  $\mu,\mu' \in \underline{\vartheta}(\calT)$, then  $\textnormal{TV}(\mu,\mu')$ is the random variable  $ \omega \mapsto \textnormal{TV}(\mu(\omega),\mu'(\omega))$. 
\begin{lemma}\label{lem:TV}
Under Assumption \ref{asm:growth}, there exists $C \in (0,\infty)$ depending on  $\varphi$ such that 
\begin{equation}
    |v(\mu)-v(\mu')| \le C \ \lVert \textnormal{TV}(\mu,\mu') \rVert_{L^2(\Q)}, \quad \forall \ \mu,\mu' \in \underline{\vartheta}(\calT). 
\end{equation}
In particular, 
$|v(\tau)-v(\tau')| \le C \Q(\tau \ne \tau')^{1/2}$  for any stopping times $\tau, \tau' \in  \vartheta(\calT)$.
\end{lemma}
\begin{proof}
      Define  $\Phi =  \sum_{t\in \calT} |\varphi(t,X_{t})| $ and  
      recall from Assumption \ref{asm:growth} that   $\varphi(t,\cdot) \in  \calL_a$ for some $a>0$. Since  $\phi 
    \in \calL_{a}$ implies $\phi^2 
    \in \calL_{2a}$, we obtain for some constant $C\in (0,\infty)$ that   
$$\E[\Phi^2] \le |\calT|  \sum_{t\in \calT} \E^{\Q}[\varphi(t,X_{t})^2] =   |\calT|  \sum_{t\in \calT} \underbrace{K_{0,t}\varphi^2(t,x_0)}_{\in \  \calL_{2a}} \le  C\sum_{t\in \calT}  [1+|x_0|^{2a}] < \infty. $$ 
Thus  $\Phi \in L^2(\Q)$. Next, observe that 
\begin{align*}
    |v(\mu) - v(\mu')| \le \E^{\Q}\left[  \int_0^T |\varphi(t,X_{t})|\  |\mu-\mu'|(dt) \right]
    \le 2 \E^{\Q}\left[  \Phi\  \text{TV}(\mu,\mu') \right].
\end{align*}
As $\text{TV}(\mu,\mu') \le 1 \in L^2(\Q)$, the result follows from the Cauchy-Schwarz inequality and  setting $C =  2 \lVert\Phi \rVert_{L^{2}(\Q)}$. For the second claim, it suffices to observe that  $\text{TV}(\delta_{\tau},\delta_{\tau'}) = \mathds{1}_{\{\tau \ne \tau'\}}$. 
\end{proof}

\begin{remark} Set $\overline{\textnormal{TV}}_2(\mu,\mu') := \lVert \textnormal{TV}(\mu,\mu') \lVert_{L^2(\Q)}$ for relaxed stopping rules $\mu,\mu' \in  \underline{\vartheta}(\calT)$. Then,  \cref{lem:TV} states that $ \mu \mapsto v(\mu)$ is Lipschitz continuous with respect to $\overline{\textnormal{TV}}_2$. 
\end{remark}

==> OLD/04-06-2025/convSequential.tex <==
\subsection{Relaxed $L^{\infty}$ norm and second continuity result} 
\label{sec:relaxLinfty}

The continuity result in \cref{thm:unifcontV} only applies when boundaries are close in the $L^{\infty}$ sense. Although reasonable for continuous boundaries, this condition is typically too restrictive for semicontinuous boundaries. We therefore introduce a weaker topology \rr{induced by the following norm}. 

\begin{definition}\label{def:relaxedSupDist} Given a function $h: \calE\to \R$, the \textit{relaxed $L^{\infty}$ norm}   is defined as 
 % \begin{equation} \label{eq:relaxDistH}
 %      \vertiii h  = \sup_{r>0} \ \inf_{\psi \in \Psi_{r} }\ \lVert h\circ \psi  \rVert_{L^\infty(\calK)}, \quad h: \calE\to \R,  
 % \end{equation}
 \begin{align}
          \varrho( h )
          &= 
          \inf_{\psi\in \Psi}  \ \lVert h\circ \psi\rVert_{L^{\infty}(\calE)} + \lVert \psi - \text{id} \rVert_{L^{\infty}(\calE)}, \label{eq:relaxDistH},
 \end{align}
 where $\Psi$ contains all endofunctions $\psi:\calE \to \calE$ and $\text{id}$ denotes  the identity map. % on $\calE$. 
 For  $f\in 
\frakF$, we write with a slight abuse of notations,  
\begin{equation}\label{eq:relaxDistF}
    \varrho(f)  = \max_{t \in \calT}  \varrho( f(t,\cdot)). 
\end{equation}
\end{definition}
The relaxed $L^{\infty}$ norm comes as a natural notion for  semicontinuous functions and is closely related to \textit{inf convolutions} discussed in \cref{sec:convLSC}. 
We shall also call the distance induced by $\varrho$ the \textit{relaxed $L^{\infty}$ distance}, that is 
\begin{equation}
    d(h,h') := \varrho(h-h') = \inf_{\psi\in \Psi}  \ \lVert h\circ \psi - h' \circ \psi\rVert_{L^{\infty}(\calE)} + \lVert \psi - \text{id} \rVert_{L^{\infty}(\calE)}, \quad h,h': \calE \to \R,
\end{equation}
and similarly $d(f,f') = \varrho(f-f')$,  $f,f'\in \frakF$. 
%Importantly, we prove in \cref{thm:lscV} that the %space-time 
%relaxed $L^{\infty}$ distance 
%yields a continuity type result  as well, thus extending \cref{thm:unifcontV}. % to boundaries which are only lower semicontinuous. 
The transformations  in $\Psi$ echo the  reparametrization maps appearing in the  Skorokhod $J1$ distance for càdlàg processes. 
 On the other hand, a notable difference is that unlike the Skorokhod metric,  $\psi$ needs not be invertible. %\bb{[+ property of $\varrho$ if we adopt this one]}
%Notice that \cref{prop:RelaxedInfProps}, 3. implies that $\lVert \cdot \rVert_{\widetilde{L^{\infty}}(\calE)}$ satisfies a point separating property under the equivalence relation $h\sim h' \ \Longleftrightarrow |h-h'|_* = 0$. 
%Property 3. in the above Proposition implies that $\lVert h \rVert_{\widetilde{L^{\infty}}(\calE)}$ $\lVert h \rVert_{\widetilde{L^{\infty}}(\calE)} = 0$ implies that $|h-h'|_{*} \equiv 0$.

Next, we adapt \cref{thm:unifcontV} to obtain a continuity type result of $f\mapsto v(\tau_f)$ with respect to  the relaxed $L^{\infty}$ distance. We also denote the relaxed $L^\infty$ distance on any compact subset $\calK$ by $d_{\calK}(h,h') = \varrho ((h -h')\mathds{1}_{\calK})$ and similarly $d_{\calK}(f,f')  = \max_{t \in \calT}  \ d_{\calK}(f(t,\cdot),f'(t,\cdot))$. 

\begin{theorem}\label{thm:lscV}%\textnormal{\textbf{(Sequential Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}}
   Let  $C \in (0,\infty)$ given in \cref{lem:TV} and fix $\delta > 0$. Then under Assumptions \ref{asm:absCont},  
    there exists 
 $\calK \subset \subset \calE$  such that for all  $f \in \frakF$ and sequence $(f_n)\subset \frakF$, we have 
    % $$
    % d_{\calK}(f,f_n)
    % \to 0 \; \; \Longrightarrow \; \; |v(\tau_{f}) - v(\tau_{f_n})|\to 0, \quad \text{ as } n\to \infty.$$
   $$
    \lim_{n\to \infty }d_{\calK}(f,f_n)
    = 0 \; \; \Longrightarrow \; \; \limsup_{n\to \infty }\ |v(\tau_{f}) - v(\tau_{f_n})|\le C\sqrt{\delta}.$$
   % with $\rho(\iota) = \sum_{t\in\calT} \rho_t(\iota)$,  and  $(\rho_t)_{t\in \calT}$ the moduli of continuity of $(a \mapsto \Q(\alpha(X_t) \in [0,a]\ | \ \Xi(X_t)))_{t\in \calT}$.   
\rr{If $\calE$ is compact, then $f\mapsto v(\tau_f)$ is sequentially continuous.}
\end{theorem}

\begin{proof}  As  in the proof of  \cref{thm:unifcontV}, there exists   $\calK \subset \subset \calE$  such that 
 \begin{equation*}
   \Q(\Omega_{\calK}) \ge 1-\delta, \quad \Omega_{\calK} = \{\omega \in \Omega \ : \ \Xi(X_t(\omega)) \in \calK  \; \ \forall t\in \calT\}.
\end{equation*} 
       \underline{\textit{Step ${1}$.}} 
Let $f\in \frakF$ and $(f_n)\subset \frakF$ such that $\iota_n:= d_{\calK}(f , f_n)\to 0$ as $n\to \infty$. %Without loss of generality, assume that $d_{\calK}(f , f_n) \le \frac{1}{2n}$. 
Then,  there exists $\psi_n: \calT \times \calE \to \calT \times \calE$, namely $\psi_n(t,\cdot) \in \Psi$ for all $t\in \calT$, such that 
\begin{equation}\label{eq:contLSCStep1}
    \lVert (f-f_n) \circ \psi_n\rVert_{L^{\infty}(\calT \times \calK)} + \lVert \psi_n - \text{id} \rVert_{L^{\infty}(\calT \times \calK)} \le d_{\calK}(f , f_n) + \iota_n = 2\iota_n, \quad \forall t \in \calT.
\end{equation}
% Consequently, 
% \begin{align}
%     &\lVert (f-f')\circ \psi   \rVert_{L^{\infty}(\calT \times \calK)} \le \iota, \quad  \ k\ge 1, \label{eq:unifPsi}\\[0.7em] 
%      &\lVert \psi(t,\cdot) - \text{id} \rVert_{L^{\infty}(\calK)} \le 1/k, \qquad\forall \ t\in \calT. \qquad (\text{$\text{id}(\xi) = \xi$})\label{eq:psiId}
% \end{align}
Similar to the proof of \cref{thm:unifcontV}, observe that  
\begin{align*}
    \{\tau_{f} \ne \tau_{f_n}\} \subseteq  \Omega_n : = \bigcup_{t\in \calT}\big\{ X_t\in \frakS_t(f) \triangle \frakS_t(f_n) \big\} = \bigcup_{t\in \calT}\big\{\alpha(X_t) \in I_n(t,\Xi(X_t))  \big\},
\end{align*}
% \begin{align*}
%     \{\tau_{f} \ne \tau_{f_n}\} \subseteq  \Omega_n :\!\! &= \{\omega \in \Omega  : X_t(\omega) \in \frakS_t(f) \triangle \frakS_t(f_n)   \ \text{for some } t\in \calT\}, \\[0.5em]
%     &=\{\omega \in \Omega  : \alpha(X_t(\omega)) \in I_n(t,\Xi(X_t(\omega)))   \ \text{for some } t\in \calT\},
% \end{align*}
%and also, 
%$$X_t \in \frakS_t(f) \triangle \frakS_t(f_n) \; \Longrightarrow \; \alpha(X_t) \in I_n(t,\Xi(X_t)),$$
with  $I_n(t,\xi) = [\underline{f_n}(t,\xi) , \overline{f_n}(t,\xi) )$ and the functions    $\underline{f_n} = f \wedge f_n$, $\overline{f_n} = f \vee f_n$. \rr{Noting the sublevel sets $\{\underline{f_n}  \le a\}$  $\{\overline{f_n}  \le a\}$  are closed for all $a$ (given  respectively by the union and intersection of the closed sets $\{f_n  \le a\}, \{f  \le a\}$),  we conclude that $\underline{f_n}, \overline{f_n} $ are lower semicontinuous as well.} %\rr{Since the sublevel sets $\{\underline{f_n}  \le a\}$ (respectively $\{\overline{f_n}  \le a\}$)  are closed for all $a$, being the union (resp. intersection) of the closed sets $\{f_n  \le a\}, \{f  \le a\}$, we conclude that $\underline{f_n}, \overline{f_n} $ are lower semicontinuous as well.} %It is easily seen that $\underline{f_n}, \overline{f_n} $ are also lower semicontinuous in $\xi$, namely $\underline{f_n}, \overline{f_n} \in \frakF$. 
\\[-0.5em]

\underline{\textit{Step ${2}$.}} 
Fix $\xi\in \calK$ and $t\in \calT$. Since $\underline{f_n}, \overline{f_n} \in \frakF$ and $| \psi_n(t,\xi)  -\xi| \le 2\iota_n \to 0$  as $n\to \infty$, there exists $ \underline{\gamma_n},\overline{\gamma_n}: \calE \to \R_+$ such that $\underline{\gamma_n},\overline{\gamma_n}\to 0$ pointwise and 
\begin{align*}
   \rr{\underline{f_n}(t,\psi_n(t,\xi)) \le  \underline{f_n}(t,\xi) + \underline{\gamma_n}(\xi)}, \qquad 
   \overline{f_n}(t,\xi) \le  \overline{f_n}(t,\psi_n(t,\xi)) + \overline{\gamma_n}(\xi). 
\end{align*}
The above inequalities naturally holds with $\gamma_n  := \underline{\gamma_n} \vee \overline{\gamma_n}$, which also satisfies $\gamma_n(\xi) \to 0$ for all $\xi$. 
%Importantly, $\gamma_n$ depends on $\xi$. %
%\rr{[should be instead $ \underline{f_n}(t,\xi) \le \underline{f_n}(t,\psi_n(t,\xi)) + \gamma_n$, but maybe we can still conclude.]} 
\rr{[@ Mete: Actually the first inequality above looks fine since $\gamma_n$ depends on $\xi$, so we can swap $\psi_n(t,\xi)$ and $\xi$. Back to your example: if $f(t,\xi) = \mathds{1}_{\R\setminus \{0\}}$, then $\underline{f_n}(\xi) = f_n(\xi) = n|\xi|^2 \wedge 1$, $\iota_n = d_{\calK}(f , f_n) = 1/\sqrt{n}$, $\psi_n(t,\xi) = \xi \mathds{1}_{\{|\xi| \ge 1/\sqrt{n}\}}$ (using inf-convolutions with $\delta = 1/n$) so we can take $\gamma_n(\xi) = f(\xi) - f_n(\xi)  \to 0.$]}
This implies that  
$$I_n(t,\xi) \subseteq I_{n}^{\gamma_n}(t,\psi_n(t,\xi)) := [\underline{f_n}(t,\psi_n(t,\xi)) - \gamma_n(\xi), \overline{f_n}(t,\psi_n(t,\xi)) + \gamma_n(\xi)).$$
%, where for an interval $I = [\underline{a},\overline{a})$, we define $I^{\gamma} = [\underline{a}-\gamma,\overline{a}+\gamma)$.  
In light of \eqref{eq:contLSCStep1},  $I_{n}^{\gamma_n}(t,\psi_n(t,\xi))$ has length at most $ 2\iota_n + 2\gamma_n(\xi)$. %for all $(t,\xi) \in \calT \times \calK$. 
Together with the absolute continuity of $\Q(\alpha(X_t) \in \cdot \ | \ \Xi(X_t))$ and the bounded convergence theorem, we have 
\begin{align*}
    \limsup_{n\to \infty }\ \Q(\Omega_n \cap \Omega_{\calK}) &\le   \limsup_{n\to \infty }\  \sum_{t\in \calT} \Q(\{\alpha(X_t) \in I_{n}^{\gamma_n}(t,\psi_n(t,\Xi(X_t)) \}\cap \Omega_{\calK})\\
    &\le     \limsup_{n\to \infty }\ \sum_{t\in \calT}\E^{\Q}[\rho_t(2\iota_n + 2\gamma_n(\Xi(X_t)))] = 0.
\end{align*}
Following   the same rationale as in the proof of  \cref{thm:unifcontV}, we conclude  that 
 %$$|v(\tau_f)-v(\tau_{f'})|\le C\Q(\tau_f \ne \tau_{f'})^{1/2} \le C\left[\Q(\tilde{\Omega} \cap \Omega_{\calK}) + \delta\right]^{1/2} \le C\sqrt{\rho(\iota)+ \delta}.$$
 \begin{align*}
    \limsup_{n\to \infty }\ |v(\tau_{f})-v(\tau_{f_n})| &\le  \limsup_{n\to \infty }\  C\left[\Q(\Omega_n \cap \Omega_{\calK}) + \delta\right]^{1/2} = C\sqrt{\delta}. 
\end{align*}
\end{proof}

==> OLD/ConvHausdorff.tex <==

\subsection{Convergence using the Hausdorff distance between epigraphs \\ \rr{(may be too weak)}} \label{sec:HausdorffConvergence}
%\subsection{Universal Approximation Theorem for semicontinuous Functions}

We first need a metric to compare l.s.c. boundaries.   
For $f\in \frakF$ and $\calK\subseteq \Xi(\calX)$ compact, write $\calG_{t,\calK}(f)$  for the  epigraph of $f$ restricted to $\calK$ in the coordinate system induced by $A = (\Xi,\alpha)$, that is 
%$\frakS_{\calK,t}(f) = \bigcup_{\xi \in \calK} [f(\xi),\infty)$. 
$$\calG_{t,\calK}(f)  = \{(\xi,a) \in \calK \times \R_+ \ : \ a\ge f(t,\xi)\}. $$ %A(\frakS_t(f) \cap \Xi^{-1}(\calK))=
Note in particular that $(\xi,a)\in \calG_{t,\calK}(f)$ if and only if $\xi\in \calK$ and $A^{-1}(\xi,a) \in \frakS_{t}(f)$.   
%When $f$ is l.s.c.,  then $\calG_{t,\calK}(f)$ is a closed subset. This motivates to consider a metric on closed subsets of 
%$$\calG_t^{A}(f) = \{(\xi,a) \ : \ a\ge f(t,\xi)\} \subseteq A(\calX) := \Xi(\calX)\times \R_+.$$ 
Next, we endow  $\calK \times \R_+$ with  the Chebyshev metric, namely 
$$d_{\calC}((\xi,a),(\xi',a')) := |\xi-\xi'| \vee |a-a'|, \quad  (\xi,a), \ (\xi',a')\in \calK \times \R_+.$$
Moreover, we employ the Hausdorff distance between subsets of $\calK \times \R_+$, namely 
%with the Hausdorff distance 
$$d_{\calH}(F,G) = \inf\{\varepsilon > 0 \ : \ F \cup G \subseteq F^{\varepsilon} \cap G^{\varepsilon} \}, \quad F,G\subseteq \calK \times \R_+, $$
with the $\varepsilon-$neighborhood $F^{\varepsilon}  = \{y \in \R_+ \times \calK \ : \ d_{\calC}(y,F)<\varepsilon\}$. %$F^{\varepsilon} =\bigcup_{y\in F} \{y' \in \R_+ \times \calK \ : \ d_{\calC}(y,y') \le \varepsilon\}. $ 
% $$d_{\calC}(y,y') := |\xi-\xi'| \vee |a-a'|, \quad y = (\xi,a), \ y' = (\xi',a')$ in $\calK \times \R_+$$.
%The distance between points $y = (\xi,a), \ y' = (\xi',a')$ in  $\calK \times \R_+$ is measured through the Chebyshev metric, namely $d_{\calC}(y,y') := |\xi-\xi'| \vee |a-a'|$. 
 % $C^{\gamma} = \bigcup_{y\in C} B_{\gamma}(y)$.  and the  %$C^{\gamma} =\{(a,\xi) \ : \ \inf_{(a',\xi') \in C} |\xi-\xi'| \vee |a-a'| \le \gamma \}$ and the Chebyshev distance .  %
 
%$$ B_{\varepsilon,\calC}(y), \qquad B_{\varepsilon,\calC}(y) = \{y' \in \R_+ \times \calK \ : \ d_{\calC}(y,y') \le \varepsilon\}.$$ %$\{y \in \R_+\times \calK \ : \ \inf_{y' \in C} d_{\calC}(y,y') \le \varepsilon \}$.
\begin{proposition}
The mapping $d_{\calK}:\frakF \times \frakF \to \R_+$, given by 
 \begin{equation}\label{eq:lscDist}
  d_{\calK}(f,f') := \max_{t\in \calT} \ d_{\calH}(\calG_{t,\calK}(f)  ,\calG_{t,\calK}(f')  ), \quad f,f'\in \frakF, 
\end{equation} 
     is a well-defined metric. 
\end{proposition}
\begin{proof}
    Clearly, $d_{\calK}$ is symmetric, $ d_{\calK}(f,f) = 0$, and inherits the  triangular inequality property from the Hausdorff distance.  Hence $d_{\calK}$ is a pseudometric.  %Since $f,f'$ are l.s.c., %then $\calG_{t,\calK}(f)$, $\calG_{t,\calK}(f')$ are closed and 
%$d_{\calK}$ is in fact a metric. 
We finally show that $d_{\calK}$ distinguishes points. Indeed, if $d_{\calK}(f,f') =0$, then for all $t\in \calT$, $(\xi,a) \in \calG_{t,\calK}(f)$, and $k\in \N$, there exists $(\xi_k,a_k) \in \calG_{t,\calK}(f')$ such that $d_{\calC}((\xi,a),(\xi_k,a_k)) \le \frac{1}{k}$. %$|\xi-\xi_k| \vee |a-a_k| \le \frac{1}{k}$. 
Hence $(\xi_k,a_k)$ converges to $(\xi,a).$ 
Because $f'$ is l.s.c., $\calG_{t,\calK}(f')$ is closed and thus $(\xi,a) \in \calG_{t,\calK}(f')$. This shows that  $\calG_{t,\calK}(f) \subseteq \calG_{t,\calK}(f')$ and similarly $\calG_{t,\calK}(f') \subseteq \calG_{t,\calK}(f)$. Hence, $\calG_{t,\calK}(f') = \calG_{t,\calK}(f)$ from which we easily conclude that $f=f'$. 
%$$f(t,\xi) = \inf\{a \ : \ (\xi,a) \in \calG_{t,\calK}(f) \} = \inf\{a \ : \ (\xi,a) \in \calG_{t,\calK}(f') \} = f'(t,\xi), \quad \forall \ (t,\xi)\in \calT \times \calK.$$
\end{proof}
Note that a metric similar to $d_{\calK}$ was defined in \cite{BeerUSC,BeerLattice} for upper semicontinuous functions and permitting a generalization of the Stone-Weierstrass theorem for this class of functions. 

We now show that the inf convolution of some $f\in\frakF$ converges to $f$ in the metric $d_{\calK}.$

\begin{lemma}\label{lem:infCovApprox}
          Let $f \in \frakF$ such that $M= \lVert f \Vert_{L^{\infty}(\calT\times \calK)}< \infty$. Then 
          ${d}_{\calK}(f,f_{\delta,\calK}) \to 0$ as $\delta \downarrow 0$. 
\end{lemma}
\begin{proof}
Let $\varepsilon >0$ be arbitrary, fix $t\in \calT$, and write $f(\cdot)$ instead of $f(t,\xi)$. Since $f_\delta \le f$, then the epigraph of $f$ is contained in the one of $f_\delta$. Therefore, it is enough find  $\delta >0$ such that 
for all $y=(\xi,a) \in \calG_{t,\calK}(f_{\delta,\calK})$, there exists  $y'\in \calG_{t,\calK}(f)$ with $d_{\calC}(y,y')\le \varepsilon$. 
Without loss of generality, we prove the claim for $y = (\xi,f_{\delta,\calK}(\xi)) \in \partial \calG_{t,\calK}(f_{\delta,\calK})$. Indeed, if   $y_* = (\xi_{*},a_{*})\in \calG_{t,\calK}(f)$ satisfies $d_{\calC}(y,y_*)\le \varepsilon$, then  for  $a>  f_{\delta,\calK}(\xi)$, setting $y' =  y_* + (0,a - f_{\delta,\calK}(\xi))$ indeed gives $d_{\calC}((\xi,a),y')\le \varepsilon$. %$(\xi',a') =(\xi_*,a_* + a - f_{\delta,\calK}(\xi)) $.

Next, choose   $\delta = \frac{\varepsilon^2}{M}$ and consider a minimizer $\xi_{*} \in \calK$ for the inf convolution $f_\delta(\xi)$  in \eqref{eq:infconvCpctDef}. In view of  \cref{cor:lsc},  
$\xi_{*} \in \bar{B}_{\sqrt{\delta M}}(\xi)$, hence   $|\xi -\xi_*|\le \varepsilon$. %Since $f_{\delta,\calK}(\xi) = f(\xi_*) + \frac{1}{\delta}|\xi -\xi_*|^2$, then
Finally, note that 
\begin{align*}
     a_*  := f_{\delta,\calK}(\xi) = f(\xi_*) + \frac{1}{\delta}|\xi -\xi_*|^2 \ge  f(\xi_*).  
 \end{align*}
 Thus $y_*=(\xi_*,a_*)  \in \calG_{t,\calK}(f_{\delta,\calK})$ %belongs to the epigraph of $f$ 
 and $d_{\calC}(y,y_*) = |\xi - \xi_*| \le \varepsilon$ as desired. 
% Next, consider an $\varepsilon-$minimizer $\xi' \in \calK$ of $f_\delta(\xi)$. In view of  \cref{cor:lsc},  
% $\xi' \in B_{r(\delta)}(\xi)$ with $r(\delta) = \sqrt{\delta(M+1)}$. We can therefore set $\delta = \frac{\varepsilon^2}{M+1}$  to obtain that   $|\xi -\xi'|\le \varepsilon$.  Moreover, 
% \begin{align*}
%      f_{\delta,\calK}(\xi) + \varepsilon \ge f(\xi') + \frac{1}{\delta}|\xi - \xi'|^2 \ge f(\xi') \ge f_{\delta,\calK}(\xi')
% \end{align*}
% Using the uniform continuity of $f(t,\cdot)$ in $\calK$, then $f_{\delta}(\xi') \ge f_{\delta}(\xi) - \varepsilon$ (?)
% Or set $a' = f(\xi') + \frac{1}{\delta}|\xi - \xi'|^2$?
\end{proof}
The next result follows immediately. 
\begin{theorem} \textnormal{\textbf{(Universal Approximation of l.s.c. Functions)}}\label{thm:LSCUAT}
    For all $f \in \frakF$, $ \iota \in (0,1]$, and compact set $\calK \subseteq \Xi(\calX)$ such that $f$ is bounded in $\calK$, there exists a hypothesis space  $ \frakN \subseteq \frakF_c$ and $g\in \frakN$ such that  $d_{\calK}(f,g) \le \iota$. 
\end{theorem}

\begin{proof}
Let $\iota'$ be arbitrary. First, \cref{lem:infCovApprox} implies that $d_{\calK}(f,f_{\delta}) \le \iota'$ for some $\delta > 0$.  Moreover, the universal approximation theorem for continuous boundaries guarantees the existence of $g\in \frakN$ such that $\lVert f_{\delta}-g\rVert_{L^{\infty}(\calT \times \calK)} \le \iota'$.  Hence, 
 $$d_{\calK}(f,g) \le d_{\calK}(f,f_{\delta}) + d_{\calK}(f_{\delta},g) \le d_{\calK}(f_{\delta},g)  + \iota'. $$
 Since $\calG_{t,\calK}(f'-\varepsilon) \subseteq \calG_{t,\calK}(f')^{\varepsilon}  $ for any $f'\in \frakF$, we have for each $t\in \calT$ that 
  \begin{align*}
      d_{\calH}(\calG_{t,\calK}(f_\delta)  ,\calG_{t,\calK}(g)  ) 
      &\le \inf\{\varepsilon > 0 \ : \ \calG_{t,\calK}(f_{\delta}) \cup    \calG_{t,\calK}(g) \subseteq \calG_{t,\calK}(f_{\delta}-\varepsilon) \cap \calG_{t,\calK}(g-\varepsilon) \} \\
      &=\inf\{\varepsilon > 0 \ : \ \calG_{t,\calK}(f_{\delta}\wedge g)   \subseteq \calG_{t,\calK}((f_{\delta} \vee g) -\varepsilon)  \} \\
     %  &=\inf\{\varepsilon > 0 \ : \ (f_{\delta}\wedge g)(t,\xi) \ge   (f_{\delta} \vee g)(t,\xi) -\varepsilon \ \  \forall \xi \in \calK \} \\
       &=\inf\{\varepsilon > 0 \ : \ |f_{\delta}(t,\xi) - g(t,\xi)| \le \varepsilon  \ \  \forall \xi \in \calK\} \\
       &= \lVert f_{\delta}(t,\cdot)-g(t,\cdot)\rVert_{L^{\infty}(\calK)}. 
  \end{align*}
  Hence, $d_{\calK}(f_{\delta},g) \le \lVert f_{\delta}-g\rVert_{L^{\infty}(\calT \times \calK)}$ and the result thus follows by choosing $\iota' = \iota/2$. 
\end{proof}

\begin{remark}[\bb{to be checked}]
    We can easily derive a universal approximation theorem for upper semicontinuous (u.s.c.) functions by considering  hypographs instead of epigraphs. % [\bb{replace epigraph by hypo}] 
    Indeed, if $f$ is u.s.c. with $f(\calK) \subseteq   [0,M]$ for some compact set $\calK\subseteq \Xi(\calX)$,  
   then $f' = M - f$ is l.s.c. and also satisfies $f'(\calK) \subseteq   [0,M]$. 
    We can thus  apply \cref{thm:LSCUAT} to $f'$,  giving  the existence of $g' \in \frakN$ such that $d_{\calK}(f',g') \le \iota$. Noting that,  $d_{\calK}(f',g'\wedge M) \le d_{\calK}(f',g')$, %since $f' \le M$, 
    we can without loss of generality that $g'\le M$.  Now   setting $ g := M-g' \in \frakN$ gives  $f-g = f'-g'$,  so  $d_{\calK}(f,g) = d_{\calK}(f',g') \le \iota$ as desired.  
\end{remark}
%============= UAT OLD ============%
% \begin{theorem} \textnormal{\textbf{(Universal Approximation of l.s.c. Functions)}}\label{thm:LSCUAT}
%     For all $f \in \frakF$, $r>0, \ \iota \in (0,1]$, and compact set $\calK \subseteq \Xi(\calX)$ such that $f$ is uniformly bounded in $\calK$, there exists a hypothesis space  $ \frakN \subseteq \frakF_c$ and $g\in \frakN$ such that  $d_{\calK,r}(f,g) \le \iota$. 
% \end{theorem}
% \begin{proof}
% Fix $\iota_0 > 0$,  $\calK \subseteq \Xi(\calX)$ compact, and $\xi \in \calK$. Using \cref{lem:infCovApprox}, then $d_{\calK,r}(f,f_{\delta}) \le \iota_0$ for some $\delta > 0$. 
%  For every $\gamma>0$, one can find $\xi_{\gamma} \in B_{r}(\xi)$ such that $$|f(t,\xi_{\gamma}) - f_{\delta}(t,\xi_{\gamma})| \le \inf_{\xi'\in B_{r}(\xi)} |f(t,\xi') - f_{\delta}(t,\xi')| + \gamma \le \iota_0 + \gamma. $$
%     Moreover, as $f_{\delta}$ is continuous,  we can invoke the  UAT giving the existence of   $g\in \frakN  \subseteq \frakF_c$ such that $\lVert f_{\delta} - g \rVert_{L^{\infty}(\calT \times \calK)} \le \iota_0$.
%     %$$\sup_{(t,\xi) \in \calT \times \calK}  \ |f_{\delta}(t,\xi) - f_k(t,\xi)| \le \iota_0. $$
% Next, the triangular inequality yields 
%  \begin{align*}
%      |f(t,\xi_{\gamma}) - g(t,\xi_{\gamma})| &\le |f(t,\xi_{\gamma}) - f_{\delta}(t,\xi_{\gamma})|  + |f_{\delta}(t,\xi_{\gamma}) - g(t,\xi_{\gamma})| \le  2\iota_0 + \gamma.
%  \end{align*}
% Thus, 
%  $ \inf_{\xi'\in B_{r}(\xi)} |f(t,\xi') - g(t,\xi')|  \le 2\iota_0 + \gamma$ and the result follows by choosing  $\iota_0 = \frac{\iota}{2}$ and letting $\gamma \to 0$.  
% \end{proof}
%============= END UAT OLD ============%

% \begin{proof}
% Fix $\iota_0 > 0$,  $\calK \subseteq \Xi(\calX)$ compact, and $\xi \in \calK$. Using \cref{lem:infCovApprox}, there exists $C>0$  such that $d_{\calK,C\sqrt{\delta}}(f_{\delta},f) \le \iota$ for all $\delta >0$. 
% % Fix $\iota_0 > 0$,  $\calK \subseteq \Xi(\calX)$ compact, and $\xi \in \calK$. Using \cref{lem:infCovApprox}, there exists $C, \bar{\delta}>0$  such that $d_{\calK,C\sqrt{\delta}}(f,f_{\delta}) \le \iota$ for all $\delta \in (0, \bar{\delta} \ ]$. 
%     %$$\sup_{\xi \in \calK} \ \inf_{\xi'\in B_{c\sqrt{\delta}}(\xi)} \ |f_{\delta}(t,\xi') - f(t,\xi)| \le \iota_0, \quad \forall t \in \calT.   $$
%    This is notably true for  $\delta $  such that $C\sqrt{\delta} \le r$, that is   $\delta \le \frac{r^2}{C^2} $.  For concreteness, let us set $\delta = \frac{r^2}{C^2}$. % \wedge \bar{\delta}$. % in what follows. 
   
%  For every $\gamma>0$, one can find $\bar{\xi} \in B_{C\sqrt{\delta}}(\xi)$ such that $$|f_{\delta}(t,\bar{\xi}) - f(t,\xi)| \le \inf_{\xi'\in B_{C\sqrt{\delta}}(\xi)} |f_{\delta}(t,\xi') - f(t,\xi)| + \gamma \le \iota_0 + \gamma. $$
    
%     Moreover, as $f_{\delta}$ is continuous,  we can invoke the  UAT giving the existence of  $k$ and $f_k\in \frakN_k $ such that $\lVert f_{\delta} - f_k \rVert_{L^{\infty}(\calT \times \calK)} \le \iota_0$.
%     %$$\sup_{(t,\xi) \in \calT \times \calK}  \ |f_{\delta}(t,\xi) - f_k(t,\xi)| \le \iota_0. $$
% Next, the triangular inequality yields 
%  \begin{align*}
%      |f(t,\xi) - f_k(t,\bar{\xi})| &\le |f(t,\xi) - f_{\delta}(t,\bar{\xi})|  + |f_{\delta}(t,\bar{\xi}) - f_k(t,\bar{\xi})| \le  2\iota_0 + \gamma.
%  \end{align*}
%  Recalling that $r\ge C\sqrt{\delta}$, we have 
%  $$ \inf_{\xi'\in B_{r}(\xi)} |f_{\delta}(t,\xi') - f(t,\xi)| \le \inf_{\xi'\in B_{C\sqrt{\delta}}(\xi)} |f_{\delta}(t,\xi') - f(t,\xi)| \le  |f(t,\xi) - f_k(t,\bar{\xi})| \le 2\iota_0 + \gamma,$$ and the result follows by choosing  $\iota_0 = \frac{\iota}{2}$ and letting $\gamma \to 0$.  
 
% \end{proof}

%\subsection{Convergence Result}
Next, we need an adaptation of  \cref{lem:unifcontV}. 

\begin{lemma}\label{lem:lscV} \rr{(Conjecture)}
   % There exists $\psi:\R_+ \to \R_+$, $\lim_{\delta \to 0}\psi(\delta) = 0$, 
   Let  $C \in (0,\infty)$ given in \cref{lem:TV} and fix $\delta > 0$. Then under Assumptions \ref{asm:absCont},  
    there exists  %$r>0$ and
    a  compact set $\calK\subseteq \Xi(\calX)$  such that for all $\iota >0$ and  $f, f'\in \frakF$,  %\bb{and $f'\in \frakF_c$}, 
    $$d_{\calK}(f,f')\le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho (\iota) + \delta}, $$
    for some modulus $\psi:[0,\infty] \to[0,\infty]  $ with $\lim_{\iota \to 0}\psi(\iota) = 0$. 
\end{lemma}
%======== LEMMA 4 ========%
\begin{proof} \rr{(incomplete)} Let $\delta'$ be arbitrary. As in Step 1 in the proof of  \cref{lem:unifcontV}, there exists   a compact set $\calK \subseteq \Xi(\calX)$ such that 
 \begin{equation}\label{eq:OmegaK}
   \Q(\Omega_{\calK}) \ge 1-\delta', \quad \Omega_{\calK} = \{\omega \in \Omega \ : \ \Xi(X_t(\omega)) \in \calK  \; \ \forall t\in \calT\}.
\end{equation} 

%Following from $d_{\calK}(f,f')\le \iota$ and the definition of $d_{\calK}$, we can construct 
Fix $\iota>0$ and let  $\underline{f}(t,\xi) = \inf\{a\ge 0 \ : \ (\xi,a) \in \calG_{t,\calK}(f)^{\iota}\}$.
Then  $d_{\calK}(f,f')\le \iota$ if and only if $f'\le \underline{f}$ and  $f\le \underline{f'}$. %, i.e. $f\vee f'\le \underline{f} \wedge \underline{f'}$. 
Since $\calG_{t,\calK}(f') \setminus \calG_{t,\calK}(f) \subseteq \calG_{t,\calK}(f)^{\iota}\setminus \calG_{t,\calK}(f)$ same for $f',f$, 
\begin{align*}
    \Q(\{X_t \in \frakS_t(f) \triangle \frakS_t(f')\}\cap \Omega_{\Kappa}) &= \Q(A(X_t) \in \calG_{t,\calK}(f) \triangle \calG_{t,\calK}(f')) \\ 
    &\le \Q(A(X_t) \in \calG_{t,\calK}(f)^{\iota}\setminus \calG_{t,\calK}(f) ) + ...\\
    &= \Q(\alpha(X_t) \in \underline{\calI}(t,\Xi(X_t))) + ... 
\end{align*}
with $\underline{\calI}(t,\xi) =  [\underline{f}(t,\xi),f(t,\xi)) $. If $f(t,\cdot)$ is (uniformly) continuous on $ \calK$ with modulus $\varrho_f$, then 
$$|\underline{\calI}(t,\xi)| \le f(t,\xi) - \inf_{\xi'\in B_{\iota}(\xi)}f(t,\xi') + \iota \le \varrho_f(\iota) + \iota. $$
Hence, 
$$\Q(\alpha(X_t) \in \underline{\calI}(t,\Xi(X_t))) \le \rho_t(\varrho_f(\iota) + \iota). $$
\rr{However, when $f$ is strictly l.s.c.}, $|\underline{\calI}(t,\xi)|$ may not be controlled by $\iota$ around discontinuity points. \\


\bb{One workaround:} Look at the "size" of $\calG_{t,\calK}(f) \triangle \calG_{t,\calK}(f')$.  If $m= \text{dim}_{\calH}(\calK) $ notice that
\begin{align*}
    |\calG_{t,\calK}(f) \triangle \calG_{t,\calK}(f')| &= \int_{\calK\times \R_+} \mathds{1}_{[(f\wedge f')(t,\xi), (f\vee f')(t,\xi))}(a) \ da \calH^{m}(d\xi)  \\
    &= \lVert f(t,\cdot)-f'(t,\cdot)\rVert_{L^1(\calK)}.
\end{align*}
This suggests to look at $L^1$ approximations of the boundary. 
\end{proof}


%======== LEMMA 4 END ========%

% \begin{theorem}
%    Let $\delta>0$.  Under the same assumptions as in \cref{lem:lscV}, there exists $\varepsilon, \gamma>0$,  and  a family $\frakN \subset \frakF_c$ of neural networks such that $v(\tau_{g^{\varepsilon,\gamma}})\ge v^* - \delta$ for any $\gamma-$maximizer  $g^{\varepsilon,\gamma} \in \frakN$ of  $ \underset{g \ \in \  \frakN}{\sup} \  v(\mu^{\varepsilon}_g)$. 
% \end{theorem}

% \begin{proof}   Let $\delta'>0 $ be arbitrary. Using \cref{lem:unifcontV}, there exist $\delta''>0$, $\calK\subseteq \Xi(\calX)$ compact,  and $\iota>0$ such that
% \begin{equation}\label{eq:contV}
%     d_{\calK}(f,f') \le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho(\iota) + \delta''}\le \delta'. 
% \end{equation}
% Using \cref{thm:LSCUAT}, %\cite{Cybenko,Hornik}, 
% there exists a $\frakN \subset \frakF_c$ and  $g^* \in \frakN$ such that 
% $ d_{\calK}(f^* ,g^*) \le \iota. $
% We conclude  from \eqref{eq:contV}  that $v(\tau_{g^{*}}) \ge v^* - \delta'$. As $g^*$ is continuous, we can follow Steps 2, 3, 4 in the proof of \cref{thm:convCont}. 
% \end{proof}

==> OLD/ConvRelaxed.tex <==
\subsection{Relaxed $L^{\infty}$ norm and second continuity result} 
\label{sec:relaxLinfty}

The continuity result in \cref{thm:unifcontV} only applies when boundaries are close in the $L^{\infty}$ sense. Although reasonable for continuous boundaries, this condition is typically too restrictive for semicontinuous boundaries. We therefore introduce a weaker topology \rr{induced by the following norm}. 

\begin{definition}\label{def:relaxedSupDist} Given a function $h: \calE\to \R$, the \textit{relaxed $L^{\infty}$ norm}   is defined as 
 % \begin{equation} \label{eq:relaxDistH}
 %      \vertiii h  = \sup_{r>0} \ \inf_{\psi \in \Psi_{r} }\ \lVert h\circ \psi  \rVert_{L^\infty(\calK)}, \quad h: \calE\to \R,  
 % \end{equation}
 \begin{align}
          %\vertiii h 
          \lVert h \rVert_{\widetilde{L^{\infty}}(\calE)}
          &= \lim_{r\downarrow 0} \  
          %\sup_{r> 0} \ 
          \inf_{\psi\in \Psi_r}  \lVert h\circ \psi\rVert_{L^{\infty}(\calE)}, \label{eq:relaxDistH}\\[0.5em] %\{ \ \lVert h\circ \psi  \rVert_{L^{\infty}(\calE)},  \  \psi: \calE \to \calE, \ \lVert \psi - \text{id} \rVert_{L^{\infty}(\calE)}\le r \} \label{eq:relaxDistH}, %\  \lVert h \rVert_{\widetilde{L^{\infty}_r}(\calE)}, \label{eq:relaxDistH} %\\[1em] 
          %\lVert h \rVert_{\widetilde{L^{\infty}_r}(\calE)}&=  \inf \{ \ \lVert h\circ \psi  \rVert_{L^{\infty}(\calE)},  \  \psi: \calE \to \calE, \ \lVert \psi - \text{id} \rVert_{L^{\infty}(\calE)}\le r \}, \quad r\ge 0, 
          \Psi_r &= \{\psi: \calE \to \calE, \ \lVert \psi - \text{id} \rVert_{L^{\infty}(\calE)}\le r \}, \label{eq:localShifts}
 \end{align}
%where $\Psi_{r} = \{\psi: \calK \to \calK \ : \ \lVert \psi - \text{id} \rVert_{L^{\infty}(\calK) }\le r \}$ and 
with the identity map $\text{id}(\xi) = \xi$. %The \textit{relaxed $L^{\infty}$ distance} is then given by $d(h,h') =  \vertiii{h - h'}$. 
 For  $f\in 
\frakF$, we write similarly %the \textit{space-time relaxed $L^{\infty}$ distance} as
\begin{equation}\label{eq:relaxDistF}
    \lVert f \rVert_{\widetilde{L^{\infty}}(\calE \times \calT)}  = \max_{t \in \calT}  \  \lVert f(t,\cdot)\rVert_{\widetilde{L^{\infty}}(\calE)}. 
\end{equation}
\end{definition}


Since $\Psi_{r} \subset \Psi_{r'}$ when $r < r'$, we note that the limit in \eqref{eq:relaxDistH} %as $r\downarrow 0$ 
always exists and may be replaced by a supremum over $r>0$.
%It is immediate that  $\vertiii{\cdot}$ is dominated by the supremum norm. 
%\bb{Strictly speaking, ${d}_{\calK}$ is not a norm, as neither the triangular inequality  nor the positivity axiom are satisfied.} 
%This is nevertheless 
The relaxed $L^{\infty}$ norm comes as a natural notion for  semicontinuous functions and is closely related to \textit{inf convolutions} discussed in \cref{sec:convLSC}. 
\rr{We shall also call the distance induced by $\lVert \cdot \rVert_{\widetilde{L^{\infty}}(\calE)}$ the \textit{relaxed $L^{\infty}$ distance}.  Importantly, we prove in \cref{thm:lscV} that the %space-time 
relaxed $L^{\infty}$ distance 
yields a continuity type result  extending \cref{thm:unifcontV} to boundaries which are only lower semicontinuous. }

 In the above definition, the transformations  in $\Psi_r$ echo the  reparametrization maps appearing in the classical Skorokhod $J1$ distance for càdlàg processes. 
 On the other hand, a notable difference is that unlike the Skorokhod metric,  $\psi$ may not be invertible as we shall see in the proof of \cref{lem:infCovApprox}. 
% We finally stress that relaxed $L^{\infty}$ distance may be defined for general  subsets that are not necessarily compact. For our purposes, however, $d_{\calK}$ and $d_{\calK,\calT}$ will be exclusively used for compact sets, whence the assumption.  

\rr{Given $h:\calE\to \R$, we denote its \textit{lower semicontinuous envelope} by $h_*(\xi) = \liminf\limits_{\xi'\to \xi} h(\xi')$. We recall that $h_*$ is alternatively characterized as the largest lower semicontinuous function  dominated by $h$. 
 \begin{proposition}\label{prop:RelaxedInfProps}
     Let $h:\calE\to \R$. Then the relaxed $L^{\infty}$ satisfies the following properties: 
     \begin{enumerate}
         \item We have $\lVert  h \rVert_{\widetilde{L^{\infty}}(\calE)} \le \lVert  h \rVert_{L^{\infty}(\calE)}$, while the norms coincide when $h$ is uniformly continuous.  %with equality when $h$ is uniformly continuous. %, while the norms coincide when $h$ is uniformly continuous.  
        % Moreover, if $h$ is uniformly continuous, then $\lVert  h \rVert_{\widetilde{L^{\infty}}(\calE)} = \lVert  h \rVert_{L^{\infty}(\calE)}$.
     \item %(homogeneity) 
     $\lVert \gamma h \rVert_{\widetilde{L^{\infty}}(\calE)} = |\gamma| \cdot \lVert  h \rVert_{\widetilde{L^{\infty}}(\calE)}$ for all $\gamma\in \R$.
         \item %(positivity) 
         If $\lVert h \rVert_{\widetilde{L^{\infty}}(\calE)} = 0$, then $|h|_{*} \equiv 0$.  %Consequently, $\lVert h \rVert_{\widetilde{L^{\infty}}(\calE)} = 0$ implies that $|h-h'|_{*} \equiv 0$. 
     \end{enumerate}
 \end{proposition}}

 \begin{proof}
 \textit{1.} Since $\psi = \text{id}$ belongs to $\Psi_r$ for all $r>0$, then  $\inf_{\psi\in \Psi_r}  \lVert h\circ \psi\rVert_{L^{\infty}(\calE)} \le \lVert h\rVert_{L^{\infty}(\calE)}$ and the claim follows by letting $r\downarrow 0$. Now assume that $h$ is uniformly continuous and denote its modulus of continuity by $\rho:[0,\infty]\to [0,\infty]$. Let $\varepsilon > 0$. Then for all $r>0$, there exists $\psi_{r}\in \Psi_r$ such that $\lVert h\circ \psi_r\rVert_{L^{\infty}(\calE)} \le \inf_{\psi\in \Psi_r}  \lVert h\circ \psi\rVert_{L^{\infty}(\calE)} + \varepsilon$. Since $|h(\xi) - h(\psi_r(\xi))| \le \rho(|\xi - \psi_r(\xi)|)\le \rho(r)$ for all $\xi \in \calE$, we conclude that 
 $$\lVert h\rVert_{L^{\infty}(\calE)} \le \lVert h\circ \psi_r\rVert_{L^{\infty}(\calE)} + \lVert h -  h\circ \psi_r\rVert_{L^{\infty}(\calE)} \le \inf_{\psi\in \Psi_r}  \lVert h\circ \psi\rVert_{L^{\infty}(\calE)} + \varepsilon + \rho(r)\le \lVert h\rVert_{\widetilde{L^{\infty}}(\calE)}+ \varepsilon + \rho(r).$$
 The result follows by letting $r,\varepsilon \downarrow 0$.

\textit{2.} This is a direct consequence of the definition of $\lVert \cdot \rVert_{\widetilde{L^{\infty}}(\calE)}$.
 
     \textit{3.} Let $h$ such that  $\lVert h \rVert_{\widetilde{L^{\infty}}(\calE)} = 0$. %We prove the claim in several steps. 
     As $\lVert h \rVert_{\widetilde{L^{\infty}}(\calE)} = \lVert |h| \rVert_{\widetilde{L^{\infty}}(\calE)}$, we can assume without loss of generality that $h\ge 0$. Moreover,   $\lVert h_* \rVert_{\widetilde{L^{\infty}}(\calE)} \le \lVert h \rVert_{\widetilde{L^{\infty}}(\calE)}$ (recalling that $h_*\le h$) so we may further assume that $h$ is lower semicontinuous and show that $h\equiv 0$. 

     Fix $\xi\in \calE$. By definition of $\lVert \cdot \rVert_{\widetilde{L^{\infty}}(\calE)}$, there exists a sequence $\{\psi_k: \calE \to \calE\}_{k\ge 1 }$ such that $h(\psi_k(\xi))=0$ and $\psi_k\in \Psi_{1/k}$. Write $\xi_k = \psi_k(\xi)$. Then $\lVert \psi_k - \text{id} \rVert_{L^{\infty}(\calE)}\le 1/k$ $\forall k$ implies that $\xi_k \to \xi$, and from the lower semicontinuity of $h$, 
     $0\le h(\xi) \le \liminf_{k\to \infty}h(\xi_k) = 0. $ 
     Since $\xi$ was arbitrary, the claim follows. %$h\equiv = 0$ as desired. 
     
 \end{proof}
Notice that \cref{prop:RelaxedInfProps}, 3. implies that $\lVert \cdot \rVert_{\widetilde{L^{\infty}}(\calE)}$ satisfies a point separating property under the equivalence relation $h\sim h' \ \Longleftrightarrow |h-h'|_* = 0$. 
%Property 3. in the above Proposition implies that $\lVert h \rVert_{\widetilde{L^{\infty}}(\calE)}$ $\lVert h \rVert_{\widetilde{L^{\infty}}(\calE)} = 0$ implies that $|h-h'|_{*} \equiv 0$.

Next, we adapt \cref{thm:unifcontV} to obtain a continuity type result of $f\mapsto v(\tau_f)$ with respect to  the relaxed $L^{\infty}$ distance. We also denote the relaxed $L^\infty$ norm on any compact subset $\calK$ by $\lVert h \rVert_{\widetilde{L^{\infty}}(\calK)} = \lVert h \mathds{1}_{\calK}\rVert_{\widetilde{L^{\infty}}(\calE)}$ and similarly $\lVert f \rVert_{\widetilde{L^{\infty}}(\calK \times \calT)}  = \max_{t \in \calT}  \  \lVert f(t,\cdot)\rVert_{\widetilde{L^{\infty}}(\calK)}$. 

\begin{theorem}\label{thm:lscV}\textnormal{\textbf{(Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}}
   Let  $C \in (0,\infty)$ given in \cref{lem:TV} and fix $\delta > 0$. Then under Assumptions \ref{asm:absCont},  
    there exists 
 $\calK \subset \subset \calE$  such that for all $\iota >0$ and  $f, f'\in \frakF$, 
    $$
    \lVert f - f' \rVert_{\widetilde{L^{\infty}}(\calT \times \calK)}
    \le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho (\iota) + \delta}, $$
    with $\rho(\iota) = \sum_{t\in\calT} \rho_t(\iota)$,  and  $(\rho_t)_{t\in \calT}$ the moduli of continuity of $(a \mapsto \Q(\alpha(X_t) \in [0,a] ))_{t\in \calT}$.   
\end{theorem}

\begin{proof}  Let $\delta'$ be arbitrary. As in Step 1 in the proof of  \cref{thm:unifcontV}, there exists   $\calK \subset \subset \calE$  such that 
 \begin{equation*}
   \Q(\Omega_{\calK}) \ge 1-\delta', \quad \Omega_{\calK} = \{\omega \in \Omega \ : \ \Xi(X_t(\omega)) \in \calK  \; \ \forall t\in \calT\}.
\end{equation*} 
       \underline{\textit{Step ${1}$.}} 
Let $f,f' \in \frakF$ such that $ \lVert f - f' \rVert_{\widetilde{L^{\infty}}(\calT \times \calK)}\le \iota$. Then,  we can construct   a sequence $\{\psi_k:\calT\times \calK\to \calK\}_{k\ge 1 }$ such that $
    |f-f'|(t,\psi_k(t,\xi))\le \iota$ for all $\xi \in \calK$ and $\psi_k(t,\cdot) \in \Psi_{1/k}^{\calK}$ $\forall \ t \in \calT$. 
In other words, 
\begin{align}
    &\lVert (f-f')\circ \psi_k   \rVert_{L^{\infty}(\calT \times \calK)} \le \iota, \quad  \ k\ge 1, \label{eq:unifPsi}\\[0.7em] 
     &\lVert \psi_k(t,\cdot) - \text{id} \rVert_{L^{\infty}(\calK)} \le 1/k, \qquad\forall \ t\in \calT. \qquad (\text{$\text{id}(\xi) = \xi$})\label{eq:psiId}
\end{align}
Next, let $\calX_{\calK}  = \{x \in \calX \ : \ \Xi(x) \in \calK\}$ %\Xi^{-1}(\calK)$ 
and  consider the transformations 
$$\phi_k: \calT \times \calX_{\calK} \to \calX_{\calK},\quad \phi_k(t,x) = A^{-1}(\alpha(x),\psi_k(t,\Xi(x))) , \quad k\ge 1. $$
In light of \eqref{eq:psiId}, observe that $\phi_k(t,x) \to A^{-1}(\alpha(x),\Xi(x)) = x$ pointwise in $\calX_{\calK}$  since $A^{-1}$ is continuous. Noting  that $\omega \in \Omega_{\calK}$ if and only if $X_t(\omega) \in \calX_{\calK}$,   
the bounded convergence theorem yields for every $B\in \calB(\calX)$,
\begin{equation}\label{eq:BCTPsi}
    \lim_{k\to \infty}\Q(\{\phi_k(t,X_t)\in B\}\cap \Omega_{\calK}) 
    = \Q(\{X_t\in B\}\cap \Omega_{\calK}), \quad \forall \ t \in \calT.
\end{equation}
Thus for fixed  $\gamma>0$ and $t\in \calT$, there exists $ k\ge 1$ such that 
\begin{equation}\label{eq:boundPsi}
  \Q(\{\phi_{k}(t,X_t)\in B\}\cap \Omega_{\calK}) \ge  \Q(\{X_t\in B\}\cap \Omega_{\calK}) - \gamma.
\end{equation}

 \underline{\textit{Step ${2}$.}} Recall that   
      $$\{\tau_{f} \ne \tau_{f'}\} \subseteq  \tilde{\Omega} = \{\omega \in \Omega  : X_t(\omega) \in \frakS_t(f) \triangle \frakS_t(f')   \ \text{ for some } t\in \calT\}.  $$      
Choosing $B = \frakS_t(f) \triangle \frakS_t(f')$ for each $t\in \calT$ and $\gamma = \frac{\delta'}{|\calT|}$ in \eqref{eq:boundPsi}, we have for $k$ large enough  that  
\begin{align}\label{eq:obs1}
    \Q(\tilde{\Omega}\cap \Omega_{\calK}) &\le \delta' + \sum_{t\in \calT} \Q(\{\phi_{k}(t,X_t) \in \frakS_t(f) \triangle \frakS_t(f') \}\cap \Omega_{\calK}).
\end{align}
Defining $I_{f,f'}(t,\xi) = [(f \wedge f')(t,\xi), (f \vee f')(t,\xi))$ as in the proof of \cref{thm:unifcontV}, observe that 
\begin{align*}
     \phi_k(t,x) &\in \frakS_t(f) \triangle \frakS_t(f')   \, \Longleftrightarrow \alpha(x) \in I_{f,f'}(t,\psi_k(t,\Xi(x))), \quad x \in \calX. 
\end{align*}
   Because of \eqref{eq:unifPsi},  $I_{f,f'}(t,\psi_k(t,\xi))$ has length at most $\iota$ for all $(t,\xi) \in \calT \times \calK$. Together with the absolute continuity of $\Q(\alpha(X_t) \in \cdot)$, this yields
\begin{equation}\label{eq:obs2}
    \sum_{t\in \calT} \Q(\{\phi_{k}(t,X_t) \in \frakS_t(f) \triangle \frakS_t(f') \}\cap \Omega_{\calK}) \le \sum_{t\in \calT}\rho_t(\iota) = \rho(\iota).
\end{equation}
From \eqref{eq:obs1},\eqref{eq:obs2}, and  the rationale in the proof of  \cref{thm:unifcontV}, we conclude with $\delta' = \frac{\delta}{2}$ that 
 $$|v(\tau_f)-v(\tau_{f'})|\le C\Q(\tau_f \ne \tau_{f'})^{1/2} \le C\left[\Q(\tilde{\Omega} \cap \Omega_{\calK}) + \delta'\right]^{1/2} \le C\sqrt{\rho(\iota)+ \delta}.$$
\end{proof}



==> OLD/Junk.tex <==

% ABSTRACT
We study boundaries and their hitting times in the context of 
optimal stopping and Bermudan-style options. 
 We prove the continuity of the map linking the boundary to the value of its associated stopping  policy.  While the supremum norm is used to compare continuous boundaries, a weaker topology induced by the so-called \textit{relaxed $L^{\infty}$ distance} is used in the semicontinuous case. 
Relaxed stopping rules and their properties are also discussed. 
  Incidentally, we provide a convergence analysis  for neural stopping boundaries [Reppen, Soner, and Tissot-Daguette,  Neural Optimal Stopping Boundary, 2022] entailing the  universal approximation capability of neural networks and the notion of   inf/sup  convolution. 


  % INTRO



The  optimal stopping problem, whose simplest form is given by
% \begin{equation}\label{eq:OS0}
%   \sup_{\tau \in \vartheta(\calT)} \E^{\Q}[ \varphi(\tau,X_{\tau})],
% \end{equation}
\begin{equation}\label{eq:OS0}
  \sup \left\{ v(\tau) := \E^{\Q}[ \varphi(\tau,X_{\tau})] \ : \ \tau = \text{ stopping time}\right\},
\end{equation}
for a process $X $ and  reward function $\varphi$, %and exercise dates $\calT$, 
plays a central role in stochastic  optimal control and has applications in many quantitative disciplines. In mathematical statistics, sequential tests such as the    quickest detection of a Wiener process can be tackled using  the theory of  optimal stopping   \cite{ShiryaevStat, PeskirShiryaev}. 
In mathematical finance, optimal stopping problems emerge naturally from the pricing of American or Bermudan contingent claims \cite{elKarouiPardouxQuenez,Karatzas,PeskirShiryaev}. In this context, $\varphi$ is  the payoff of the claim, $X$ describes the price evolution of the underlying asset, and the optimal value in \eqref{eq:OS0} gives the initial price of the contract. 

The initial motivation of this paper is  to provide a convergence study of the  \textit{neural optimal stopping boundary} method \cite{ReppenSonerTissotFB} (see also \cite{ReppenSonerTissotDF}) to solve optimal stopping problems arising notably from American options. The boundary  delimiting the \textit{stopping} (or \textit{exercise}) \textit{region} is parameterized by a feedforward artificial neural network.  Further details on the algorithm are given in \cref{sec:NOSB} and at the end of this section. %We stress that a  discrete time framework is adopted throughout 
 The convergence analysis relies mainly on   relaxation and continuity results for hitting times of  boundaries, presented in \cref{sec:relaxation,sec:continuity}, respectively. We then realized that these findings can be used in more general stochastic control problems, hence  broadening the range of applications.  We stress that a   discrete time framework is adopted throughout, in line with 
the inevitable use of 
temporal discretization in numerical methods. Adapting the present results in continuous time is not straightforward and would certainly involve other interesting  techniques. This is, however, beyond the scope of this work.     

In \cref{sec:OS}, we introduce the optimal stopping problem in discrete time  and make  natural assumptions on the reward function and stopping region.  Importantly, we suppose that the state space of the underlying process can be transformed so as to represent the stopping region  as the epigraph (or hypograph) of a particular function$-$the \textit{optimal stopping boundary}$-$denoted by $f^{\diamond}$ throughout. Provided that the state process started outside the stopping  region, then the hitting time of  $f^{\diamond}$ is  an optimal stopping time for \eqref{eq:OS0}. 
This implies that one can restrict the set of stopping times in \eqref{eq:OS0} to hitting times of boundaries, namely 
\begin{equation}\label{eq:OS0f}
  \sup \left\{ v(\tau_f) := \E^{\Q}[ \varphi(\tau_f,X_{\tau_f})] \ : \ f = \text{ stopping boundary} \right\},
\end{equation}
where $\tau_f$ is the hitting time of the epigraph (or hypograph) of $f$.

%\subsection{Relaxed Stopping Rules}\label{sec:introRelax}
In \cref{sec:relaxation}, we discuss a relaxation of \eqref{eq:OS0f} which is essential for stochastic gradient-based algorithms in optimal stopping,  such as the \textit{deep optimal stopping} method \cite{Becker1,Becker2} and the neural optimal stopping boundary method \cite{ReppenSonerTissotFB}. 
Postponing  technical details to \cref{sec:relaxation}, the relaxed version of problem \eqref{eq:OS0} takes the form 
% \begin{equation}\label{eq:relax0}
%     \sup_{\mu \in \underline{\vartheta}(\calT)} \E^{\Q}\left[\int_{\calT} \varphi(t,X_{t}) \mu(dt) \right],
% \end{equation}
\begin{equation}\label{eq:relax0}
    \sup\left\{ v(\mu) := \E^{\Q}\left[\int \varphi(t,X_{t}) \mu(dt) \right] \ : \ \mu =  \text{ random probability measure}\right\}.
\end{equation}

%where $\underline{\vartheta}(\calT)$ is the set of random probability measures on $\calT$  adapted to the flow of information. % of the  problem. %In other words, $\mu(\{t\})$ is an $\calF_t-$measurable random variable for all $\mu \in \underline{\vartheta}(\calT)$, $t\in \calT$. 
Also called \textit{convexification} \cite{Acikmese} or \textit{compactification}     \cite{ElKaroui}, relaxation procedures such as \eqref{eq:relax0} are classically used in stochastic control problems to prove the existence of an optimal solution \cite{FlemingDomokos,Haussmann_Lepeltier,McShane}. Indeed, there may not exist an optimal control in the strict sense, e.g. when the  admissible set is not convex. 
Here,  convexification has the special advantage that it transforms optimal stopping problems into  a more classical formulation in  stochastic control, opening the door to numerous methods and tools. In addition, we shall see in  \cref{prop:relaxOS} that problems \eqref{eq:OS0} and \eqref{eq:relax0} achieve the same optimal value.  
This is a crucial property, valid in many contexts; see, e.g.,  \cite{Gyongy,Hobson} and \cite[Lemma 1.5.2.]{Krylov} in continuous time  optimal stopping and \cite{ElKaroui,FlemingDomokos,Haussmann_Lepeltier} in general stochastic optimal control.  
Other relaxation techniques have proved useful in  optimal stopping, such as  policies induced by occupation measure of the stopped process  \cite{Bouveret} or randomized exercise rates \cite{Bayer}.  We can also mention penalty methods for American options \cite{ForsythVetzal,HowisonReisinger} 
relaxing the otherwise constrained dominance of the value function (the \textit{price}) over the payoff $\varphi$.   
Unlike convexification, the penalty approach introduces a bias in the optimal value, which nonetheless vanishes in the limit.  

In the neural optimal stopping boundary method,
the stopping policy is relaxed by introducing a \textit{fuzzy} region around the   boundary. The stopping decision remains the same  outside the fuzzy region, while inside, the former is replaced by stopping intensities  proportional to the signed distance to the boundary. This procedure generates   \textit{relaxed} hitting times of boundaries$-$namely random  probability measures supported  on the set of exercise dates. % as in \eqref{eq:relax0}$-$. 
The relaxed problem \eqref{eq:relax0} thus becomes
\begin{equation}\label{eq:relax1}
    \sup\left\{ v(\mu_f) := \E^{\Q}\left[\int \varphi(t,X_{t}) \mu_f(dt) \right] \ : \ \mu_f =  \text{relaxed hitting time of $f$}\right\}.
\end{equation}
As shifting the boundary ever so slightly changes the stopping intensities inside the fuzzy region, the above relaxation makes stochastic gradient methods applicable. The fuzzy region is akin to the \textit{mushy zone} between two phases (typically solid and liquid) in phase-field models \cite{B-mushy,V-mushy,Soner}. The introduction of a  fuzzy  region is critical in other deep learning algorithms as well,  such as  occupation networks in  computer vision  \cite{OccupancyNN} or deep level-set functions for solving Stefan problems  \cite{SST}. 

\cref{sec:continuity} is devoted to  continuity results. In particular, \cref{thm:unifcontV,thm:lscV} establish the continuity % uniform continuity (in compact sets) 
of the value functional $\frakF \ni f \mapsto v(\tau_f)$, where $\frakF$ is a set of stopping boundaries. Let us  give a condensed statement. 

\begin{theorem*}\label{thm:unifcontV0}
\textnormal{\textbf{(Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}} 
 Let $\mathfrak{m}$ be a metric on $\frakF$. Then for all $\delta>0$, there exists $\iota  >0$ satisfying  %for every pair $f,f' \in \frakF$ of  stopping boundaries such that $d( f,f') \le \iota$, 
    \begin{equation}\label{eq:unifcontV}
     \forall f,f' \in \frakF \ \text{ such that } \  \mathfrak{m}( f,f') \le \iota \ \Longrightarrow   \ |v(\tau_{f}) - v(\tau_{f'})| \le \delta. 
    \end{equation}
\end{theorem*}
The first continuity theorem (\cref{thm:unifcontV}) implies  that the value   associated to the relaxed hitting time of boundaries as in \eqref{eq:relax1} converges to the value using the sharp interface  as the width of the fuzzy region tends to zero. This is the content of \cref{cor:relaxUnif}.  

When the boundaries are continuous in space, the metric in the above theorem will be the supremum norm in a fixed compact set. Otherwise,   a weaker topology induced by the so-called \textit{relaxed $L^{\infty}$ distance}  is considered; see   \cref{def:relaxedSupDist}. Loosely speaking, the relaxed $L^{\infty}$ distance  compares  boundaries $f,f'\in \frakF$  uniformly while 
giving the flexibility to   move to nearby points where $f,f'$ are closer to one another.  This is done through a transformation of the domain, similar to reparametrization maps    in the Skorokhod $J1$ distance  for càdlàg processes. 



 In \cref{sec:NOSB}, we combine the above results and provide a convergence analysis of the \textit{neural optimal stopping boundary} method \cite{ReppenSonerTissotFB}. 
For concreteness, we now summarize the algorithm while postponing the  details to \cref{sec:NOSB}. The algorithm looks for a \textit{neural stopping boundary}, namely a \textit{feedforward neural network} $g^{\theta}$   
such that $$v(\tau_{g^{\theta}}) \approx \sup_{f\in \frakF}
v(\tau_f) \  = v(\tau_{f^{\diamond}}).$$ 
The parameter vector $\theta$ is then trained by maximizing the relaxed reward $v(\mu_{g^{\theta}})$ using stochastic gradient ascent.  
When the optimal stopping boundary $f^{\diamond}$ is continuous, 
one can apply the celebrated Universal Approximation Theorem \cite{Cybenko,Hornik} stating  that any continuous function can be approximated arbitrarily well by  feedforward neural networks in  compact sets. 
Combined with the continuity of $f \mapsto v(\tau_f)$, we can derive a convergence result  (\cref{thm:convCont}) whose 
 statement is now summarized. 
% \begin{theorem*}\label{thm:convCont0} \textnormal{\textbf{(Convergence)}}
%    Let $\delta>0$, $\frakN$ be a family of universal approximators.   Then   there exists $\varepsilon, \gamma>0$  such that  any maximizer  $g^{\varepsilon} \in \frakN$ of  $ \underset{g  \in   \frakN}{\sup} \  v(\mu^{\varepsilon}_g)$ satisfies $v(\tau_{g^{\varepsilon}})\ge v^{\diamond} - \delta$. 
% \end{theorem*}

\begin{theorem*}\label{thm:convCont0} \textnormal{\textbf{(Convergence)}}
   For all  $\delta>0$,  there exists $\varepsilon>0$ and a feedforward  neural network  $g^{\theta}$ such that $v(\tau_{g^{\theta}})\ge v(\tau_{f^{\diamond}}) - \delta$. 
\end{theorem*}


 

% The lack of closed-form solutions  even for vanilla options  
% led to a myriad of numerical methods aiming to solve \eqref{eq:OS0}. Recently, the use of neural networks for this problem has attracted a fair amount of attention \cite{kohler,Becker1,Becker2,ReppenSonerTissotDF,ReppenSonerTissotFB}, especially in the high-dimensional setting. The validity of the algorithm is typically demonstrated through numerical experiments, but little has been done when it comes to theoretical results. \bb{[ref]} 


Generally, the optimal stopping boundary $f^{\diamond}$ may fail to be continuous, preventing the use of the Universal Approximation Theorem. Nevertheless,  it is shown in \cref{prop:lscBdry}   
that, under mild assumptions,  the stopping boundary is at least  semicontinuous. We then adopt the following strategy:  $(i)$ Construct a sequence of \textit{continuous} functions converging to $f^{\diamond}$, $(ii)$ Approximate each continuous function in $(i)$ by a neural network. We therefore expect that the sequence of neural networks converges to $f^{\diamond}$ in some suitable sense.  Regarding step $(i)$, we employ \textit{inf} (respectively \textit{sup}) \textit{convolutions}  when $f^{\diamond}$ is lower (resp. upper) semicontinuous.  Inf/sup convolutions, recalled in \cref{sec:convLSC}, are effective regularization tools popularized in the theory of viscosity solutions; see, e.g.,  \cite[Section V.5]{FS} and \cite{LasryLions}. As explained in \cref{thm:LSCUAT}, it turns out that lower semicontinuous functions can be approximated arbitrarily well by neural networks with respect to the relaxed $L^{\infty}$ distance mentioned earlier. This is an interesting result in its own right and can be applied to other tasks  involving the approximation of  semicontinuous functions. 

There is a recent body of literature on the convergence of deep learning methods in stochastic optimal control:  \citet{Hure} study the convergence  of discrete time stochastic control problems involving policy and/or value iteration; \citet{LapeyreLelong} prove the convergence of the Longstaff-Schwartz algorithm \cite{LSMC} using neural networks to approximate the continuation value; 
   \citet{Gonon} sheds light on the expressivity and maximal size  of   neural networks to produce optimal stopping rules.  
   Let us also mention a result given in the original    \textit{deep optimal stopping} paper \cite[Proposition 4]{Becker1} proving the near optimality of deep stopping strategies. While all the above algorithms  are  based on dynamic programming, the neural optimal stopping boundary method  \cite{ReppenSonerTissotFB}  finds an optimal stopping rule in a forward fashion. Consequently, our convergence analysis  necessitates other techniques and tools, hence   differs greatly from previous works.  

\textbf{Structure of the paper.} In \cref{sec:OS}, we introduce the optimal stopping problem,  our main structural assumption on the exercise region, and give financial examples. In \cref{sec:relaxation}, we define the fuzzy region and construct relaxed stopping rules. \cref{sec:continuity} establishes the  continuity of the map $f\mapsto v(\tau_f)$ as well as important consequences. In \cref{sec:NOSB}, we prove the convergence of the neural optimal stopping boundary method in the continuous and semicontinuous case, respectively.  \cref{sec:conclusion} provides  concluding remarks and \cref{app:relaxedproblem} contains the proof of \cref{prop:relaxOS}. 


==> OLD/RelaxedLInfJunk.tex <==
\begin{definition}\label{def:relaxedSupDist} Given a compact set $\calK \subset \subset \calE$,  the \textit{relaxed $L^{\infty}$ distance} (in $\calK$)  is given by 
 \begin{equation} \label{eq:relaxDistH}
      {d}_{\calK}(h,h') = \sup_{r>0} \ \inf_{\psi \in \Psi_{r}^{\calK} }\ \lVert h\circ \psi -  h'\circ \psi \rVert_{L^\infty(\calK)}, \quad h,h': \calE\to \R,  
 \end{equation}
where $\Psi_{r}^{\calK} = \{\psi: \calK \to \calK \ : \ \lVert \psi - \text{id} \rVert_{L^{\infty}(\calK) }\le r \}$ and identity map $\text{id}(\xi) = \xi$. For  $f,f'\in 
\frakF$, we define similarly %the \textit{space-time relaxed $L^{\infty}$ distance} as
\begin{equation}\label{eq:relaxDistF}
    d_{\calK,\calT}(f,f') = \max_{t \in \calT}  \ {d}_{\calK}(f(t,\cdot),f'(t,\cdot)). 
\end{equation}
\end{definition}
It is immediate that  $d_{\calK}$ is dominated by the $L^{\infty}$ distance. Strictly speaking, ${d}_{\calK}$ is not a distance, as neither the triangular inequality  nor the positivity axiom are satisfied. This is nevertheless a natural notion for  semicontinuous functions and closely related to the definition of \textit{inf convolutions} discussed in \cref{sec:convLSC}. Importantly, we prove in \cref{thm:lscV} that the space-time relaxed $L^{\infty}$ distance $d_{\calK,\calT}$ yields a continuity result  extending \cref{thm:unifcontV} to boundaries which are only lower semicontinuous. 

 In the above definition, the transformations $\psi:\calK \to \calK$ echo the  reparametrization maps appearing in the classical Skorokhod $J1$ distance for càdlàg processes. 
 On the other hand, a notable difference is that unlike the Skorokhod metric,  $\psi$ may not be invertible as we shall see in the proof of \cref{lem:infCovApprox}. 
 We finally stress that relaxed $L^{\infty}$ distance may be defined for general  subsets that are not necessarily compact. For our purposes, however, $d_{\calK}$ and $d_{\calK,\calT}$ will be exclusively used for compact sets, whence the assumption.  

We can now adapt \cref{thm:unifcontV} to obtain a continuity result of $f\mapsto v(\tau_f)$ with respect to  the relaxed $L^{\infty}$ distance. 

\begin{theorem}\label{thm:lscV}\textnormal{\textbf{(Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}}
   Let  $C \in (0,\infty)$ given in \cref{lem:TV} and fix $\delta > 0$. Then under Assumptions \ref{asm:absCont},  
    there exists 
 $\calK \subset \subset \calE$  such that for all $\iota >0$ and  $f, f'\in \frakF$, 
    $$d_{\calK,\calT}(f,f')\le \iota \ \Longrightarrow \ |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho (\iota) + \delta}, $$
    with $\rho(\iota) = \sum_{t\in\calT} \rho_t(\iota)$,  and  $(\rho_t)_{t\in \calT}$ the moduli of continuity of $(a \mapsto \Q(\alpha(X_t) \in [0,a] ))_{t\in \calT}$.   
\end{theorem}

\begin{proof}  Let $\delta'$ be arbitrary. As in Step 1 in the proof of  \cref{thm:unifcontV}, there exists   $\calK \subset \subset \calE$  such that 
 \begin{equation*}
   \Q(\Omega_{\calK}) \ge 1-\delta', \quad \Omega_{\calK} = \{\omega \in \Omega \ : \ \Xi(X_t(\omega)) \in \calK  \; \ \forall t\in \calT\}.
\end{equation*} 
       \underline{\textit{Step ${1}$.}} 
Let $f,f' \in \frakF$ such that $d_{\calK,\calT}(f,f')\le \iota$. From the definition of $d_{\calK,\calT}$,  we can construct   a sequence $\{\psi_k:\calT\times \calK\to \calK\}_{k\ge 1 }$ such that $
    |f(t,\psi_k(t,\xi)) - f'(t,\psi_k(t,\xi))|\le \iota$ for all $\xi \in \calK$ and $\psi_k(t,\cdot) \in \Psi_{1/k}^{\calK}$ $\forall \ t \in \calT$. 
In other words, 
\begin{align}
    &\lVert f\circ \psi_k -  f'\circ \psi_k  \rVert_{L^{\infty}(\calT \times \calK)} \le \iota, \quad  \ k\ge 1, \label{eq:unifPsi}\\[0.7em] 
     &\lVert \psi_k(t,\cdot) - \text{id} \rVert_{L^{\infty}(\calK)} \le 1/k, \qquad\forall \ t\in \calT. \qquad (\text{$\text{id}(\xi) = \xi$})\label{eq:psiId}
\end{align}
Next, let $\calX_{\calK}  = \{x \in \calX \ : \ \Xi(x) \in \calK\}$ %\Xi^{-1}(\calK)$ 
and  consider the transformations 
$$\phi_k: \calT \times \calX_{\calK} \to \calX_{\calK},\quad \phi_k(t,x) = A^{-1}(\alpha(x),\psi_k(t,\Xi(x))) , \quad k\ge 1. $$
In light of \eqref{eq:psiId}, observe that $\phi_k(t,x) \to A^{-1}(\alpha(x),\Xi(x)) = x$ pointwise in $\calX_{\calK}$  since $A^{-1}$ is continuous. Noting  that $\omega \in \Omega_{\calK}$ if and only if $X_t(\omega) \in \calX_{\calK}$,   
the bounded convergence theorem yields for every $B\in \calB(\calX)$,
\begin{equation}\label{eq:BCTPsi}
    \lim_{k\to \infty}\Q(\{\phi_k(t,X_t)\in B\}\cap \Omega_{\calK}) 
    = \Q(\{X_t\in B\}\cap \Omega_{\calK}), \quad \forall \ t \in \calT.
\end{equation}
Thus for fixed  $\gamma>0$ and $t\in \calT$, there exists $ k\ge 1$ such that 
\begin{equation}\label{eq:boundPsi}
  \Q(\{\phi_{k}(t,X_t)\in B\}\cap \Omega_{\calK}) \ge  \Q(\{X_t\in B\}\cap \Omega_{\calK}) - \gamma.
\end{equation}

 \underline{\textit{Step ${2}$.}} Recall that   
      $$\{\tau_{f} \ne \tau_{f'}\} \subseteq  \tilde{\Omega} = \{\omega \in \Omega  : X_t(\omega) \in \frakS_t(f) \triangle \frakS_t(f')   \ \text{ for some } t\in \calT\}.  $$      
Choosing $B = \frakS_t(f) \triangle \frakS_t(f')$ for each $t\in \calT$ and $\gamma = \frac{\delta'}{|\calT|}$ in \eqref{eq:boundPsi}, we have for $k$ large enough  that  
\begin{align}\label{eq:obs1}
    \Q(\tilde{\Omega}\cap \Omega_{\calK}) &\le \delta' + \sum_{t\in \calT} \Q(\{\phi_{k}(t,X_t) \in \frakS_t(f) \triangle \frakS_t(f') \}\cap \Omega_{\calK}).
\end{align}
Defining $I_{f,f'}(t,\xi) = [(f \wedge f')(t,\xi), (f \vee f')(t,\xi))$ as in the proof of \cref{thm:unifcontV}, observe that 
\begin{align*}
     \phi_k(t,x) &\in \frakS_t(f) \triangle \frakS_t(f')   \, \Longleftrightarrow \alpha(x) \in I_{f,f'}(t,\psi_k(t,\Xi(x))), \quad x \in \calX. 
\end{align*}
   Because of \eqref{eq:unifPsi},  $I_{f,f'}(t,\psi_k(t,\xi))$ has length at most $\iota$ for all $(t,\xi) \in \calT \times \calK$. Together with the absolute continuity of $\Q(\alpha(X_t) \in \cdot)$, this yields
\begin{equation}\label{eq:obs2}
    \sum_{t\in \calT} \Q(\{\phi_{k}(t,X_t) \in \frakS_t(f) \triangle \frakS_t(f') \}\cap \Omega_{\calK}) \le \sum_{t\in \calT}\rho_t(\iota) = \rho(\iota).
\end{equation}
From \eqref{eq:obs1},\eqref{eq:obs2}, and  the rationale in the proof of  \cref{thm:unifcontV}, we conclude with $\delta' = \frac{\delta}{2}$ that 
 $$|v(\tau_f)-v(\tau_{f'})|\le C\Q(\tau_f \ne \tau_{f'})^{1/2} \le C\left[\Q(\tilde{\Omega} \cap \Omega_{\calK}) + \delta'\right]^{1/2} \le C\sqrt{\rho(\iota)+ \delta}.$$
\end{proof}


==> OLD/convRelaxedNEW.tex <==
\subsection{Relaxed $L^{\infty}$ norm and second continuity result} 
\label{sec:relaxLinfty}

The continuity result in \cref{thm:unifcontV} only applies when boundaries are close in the $L^{\infty}$ sense. Although reasonable for continuous boundaries, this condition is typically too restrictive for semicontinuous boundaries. We therefore introduce a weaker topology \rr{induced by the following norm}. 

\begin{definition}\label{def:relaxedSupDist} Given a function $h: \calE\to \R$, the \textit{relaxed $L^{\infty}$ norm}   is defined as 
 % \begin{equation} \label{eq:relaxDistH}
 %      \vertiii h  = \sup_{r>0} \ \inf_{\psi \in \Psi_{r} }\ \lVert h\circ \psi  \rVert_{L^\infty(\calK)}, \quad h: \calE\to \R,  
 % \end{equation}
 \begin{align}
          \varrho( h )
          &= 
          \inf_{\psi\in \Psi}  \ \lVert h\circ \psi\rVert_{L^{\infty}(\calE)} + \lVert \psi - \text{id} \rVert_{L^{\infty}(\calE)}, \label{eq:relaxDistH},
 \end{align}
 where $\Psi$ contains all endofunctions $\psi:\calE \to \calE$ and $\text{id}$
is the identity on $\calE$. 
 For  $f\in 
\frakF$, we write with a slight abuse of notations,  
\begin{equation}\label{eq:relaxDistF}
    \varrho(f)  = \max_{t \in \calT}  \varrho( f(t,\cdot)). 
\end{equation}
\end{definition}
The relaxed $L^{\infty}$ norm comes as a natural notion for  semicontinuous functions and is closely related to \textit{inf convolutions} discussed in \cref{sec:convLSC}. 
We shall also call the distance induced by $\varrho$ the \textit{relaxed $L^{\infty}$ distance}, that is 
\begin{equation}
    d(h,h') := \varrho(h-h') = \inf_{\psi\in \Psi}  \ \lVert h\circ \psi - h' \circ \psi\rVert_{L^{\infty}(\calE)} + \lVert \psi - \text{id} \rVert_{L^{\infty}(\calE)}, \quad h,h': \calE \to \R,
\end{equation}
and similarly $d(f,f') = \varrho(f-f')$,  $f,f'\in \frakF$. 
Importantly, we prove in \cref{thm:lscV} that the %space-time 
relaxed $L^{\infty}$ distance 
yields a continuity type result  extending \cref{thm:unifcontV} to boundaries which are only lower semicontinuous. 
In the above definition, the transformations  in $\Psi$ echo the  reparametrization maps appearing in the  Skorokhod $J1$ distance for càdlàg processes. 
 On the other hand, a notable difference is that unlike the Skorokhod metric,  $\psi$ needs not be invertible. \bb{[+ property of $\varrho$ if we adopot this one]}
%Notice that \cref{prop:RelaxedInfProps}, 3. implies that $\lVert \cdot \rVert_{\widetilde{L^{\infty}}(\calE)}$ satisfies a point separating property under the equivalence relation $h\sim h' \ \Longleftrightarrow |h-h'|_* = 0$. 
%Property 3. in the above Proposition implies that $\lVert h \rVert_{\widetilde{L^{\infty}}(\calE)}$ $\lVert h \rVert_{\widetilde{L^{\infty}}(\calE)} = 0$ implies that $|h-h'|_{*} \equiv 0$.

Next, we adapt \cref{thm:unifcontV} to obtain a continuity type result of $f\mapsto v(\tau_f)$ with respect to  the relaxed $L^{\infty}$ distance. We also denote the relaxed $L^\infty$ distance on any compact subset $\calK$ by $d_{\calK}(h,h') = \varrho ((h -h')\mathds{1}_{\calK})$ and similarly $d_{\calK}(f,f')  = \max_{t \in \calT}  \ d_{\calK}(f(t,\cdot),f'(t,\cdot))$. We also make the following assumpation.
\begin{asm}
\label{asm:absCont2}
For every $t\in \calT$, the  law of $X_t$  
is absolutely continuous with respect to the Lebesgue measure on $\calX$
and admits  a  bounded density $\phi_{X_t}$
\end{asm}

\begin{theorem}\label{thm:lscV}\textnormal{\textbf{(Continuity of $\boldsymbol{f \mapsto v(\tau_f)}$)}}
   Let  $C \in (0,\infty)$ given in \cref{lem:TV} and fix $\delta > 0$. Then under Assumptions \ref{asm:absCont},  
    there exists 
 $\calK \subset \subset \calE$  such that for all $\iota >0$ and  $f, f'\in \frakF$, 
    $$
    d_{\calK}(f,f')
    \le \iota \; \Longrightarrow \; |v(\tau_{f}) - v(\tau_{f'})|\le C\sqrt{\rho (\iota) + \delta}, $$
    with $\rho(\iota) = \sum_{t\in\calT} \rho_t(\iota)$,  and  $(\rho_t)_{t\in \calT}$ the moduli of continuity of $(a \mapsto \Q(\alpha(X_t) \in [0,a]\ | \ \Xi(X_t)))_{t\in \calT}$.   
\end{theorem}

\begin{proof}  As in Step 1 in the proof of  \cref{thm:unifcontV}, there exists   $\calK \subset \subset \calE$  such that 
 \begin{equation*}
   \Q(\Omega_{\calK}) \ge 1-\delta, \quad \Omega_{\calK} = \{\omega \in \Omega \ : \ \Xi(X_t(\omega)) \in \calK  \; \ \forall t\in \calT\}.
\end{equation*} 
       \underline{\textit{Step ${1}$.}} 
Let $f,f' \in \frakF$ such that $d_{\calK}(f , f')\le \iota'$. Then,  there exists $\psi: \calT \times \calE \to \calT \times \calE$ such that 
\begin{equation}\label{eq:contLSCStep1}
    \lVert (f-f') \circ \psi\rVert_{L^{\infty}(\calT \times \calK)} + \lVert \psi - \text{id} \rVert_{L^{\infty}(\calT \times \calK)} \le d_{\calK}(f , f') + \iota' \le 2\iota', \quad \forall t \in \calT.
\end{equation}
% Consequently, 
% \begin{align}
%     &\lVert (f-f')\circ \psi   \rVert_{L^{\infty}(\calT \times \calK)} \le \iota, \quad  \ k\ge 1, \label{eq:unifPsi}\\[0.7em] 
%      &\lVert \psi(t,\cdot) - \text{id} \rVert_{L^{\infty}(\calK)} \le 1/k, \qquad\forall \ t\in \calT. \qquad (\text{$\text{id}(\xi) = \xi$})\label{eq:psiId}
% \end{align}
Next, let $\calX_{\calK}  = \{x \in \calX \ : \ \Xi(x) \in \calK\}$ %\Xi^{-1}(\calK)$ 
and  consider the transformation 
$$\zeta: \calT \times \calX_{\calK} \to \calX_{\calK},\quad \zeta(t,x) = A^{-1}(\alpha(x),\psi(t,\Xi(x))). $$
In light of \eqref{eq:contLSCStep1}, observe that for al $x \in \calX_{\calK}$, there exists $\gamma>0$ such that 
\begin{equation}\label{eq:contZeta}
    |\psi(t,\Xi(x)) - \Xi(x)| \le 2\iota',  \quad \Longrightarrow |\zeta(t,x)-x| \le \gamma, 
\end{equation}
since $A^{-1}$ is uniformly continuous on the compact $\calK \times \bigcup_{t\in \calT} (f(t,\calK)\cup f'(t,\calK))$.  \bb{[other way to get uniform continuity?]}
 Noting  that $\omega \in \Omega_{\calK}$ if and only if $X_t(\omega) \in \calX_{\calK}$, we then obtain for all Borel subset $B \subseteq \calX$ using \eqref{eq:contZeta} that 
\begin{align*}
    \Q(\{X_t\in B\}\cap \Omega_{\calK}) &\le \Q(\{ \zeta(t,X_t)\in B^\gamma\}\cap \Omega_{\calK}), \label{eq:probGamma} \\[1em]
    B^\gamma &= \{x \in \calX \ : \ |x-x'|\le \gamma \text{ for some } x' \in B\}. \nonumber
\end{align*}
% Using Assumption \ref{asm:absCont2}, we also note that \bb{[...]}
% \begin{align*}
%      \Q(\{ X_t\in B^\gamma\}\cap \Omega_{\calK}) &= \Q(X_t\in B^\gamma \cap \calX_{\calK}) \\
%      \int_{B^\gamma  \cap \calX_{\calK}} \phi_{X_t}(x)dx 
% \end{align*}
% Thus for fixed  $\gamma>0$ and $t\in \calT$, 
% \begin{equation}\label{eq:boundPsi}
%   \Q(\{\phi_{k}(t,X_t)\in B\}\cap \Omega_{\calK}) \ge  \Q(\{X_t\in B\}\cap \Omega_{\calK}) - \gamma.
% \end{equation}

 \underline{\textit{Step ${2}$.}} Recall that   
      $$\{\tau_{f} \ne \tau_{f'}\} \subseteq  \tilde{\Omega} = \{\omega \in \Omega  : X_t(\omega) \in \frakS_t(f) \triangle \frakS_t(f')   \ \text{ for some } t\in \calT\}.  $$      
Choosing $B = \frakS_t(f) \triangle \frakS_t(f')$ for each $t\in \calT$, we have  that  
\begin{align}\label{eq:obs1}
    \Q(\tilde{\Omega}\cap \Omega_{\calK}) &\le  \sum_{t\in \calT} \Q(\{\phi_{k}(t,X_t) \in (\frakS_t(f) \triangle \frakS_t(f'))^{\rr{\gamma}} \}\cap \Omega_{\calK}).
\end{align}
%Moreover, note that $\frakS_t(f)^{\rr{\gamma}}\subset \frakS_t(f-2\rr{\gamma})$ \. 
Defining $I_{f,f'}^{\rr{\gamma}}(t,\xi) = [(f \wedge f')(t,\xi) - \rr{\gamma} , (f \vee f')(t,\xi) + \rr{\gamma})$ as in the proof of \cref{thm:unifcontV}, observe that \bb{[to be double checked, maybe $I_{f,f'}^{\rr{2\gamma}}$ is needed]}
\begin{align*}
     \zeta(t,x) &\in (\frakS_t(f) \triangle \frakS_t(f'))^{\rr{\gamma}}   \, \Longrightarrow \alpha(x) \in I_{f,f'}^{\rr{\gamma}} (t,\psi(t,\Xi(x))), \quad x \in \calX. 
\end{align*}
   Because of \eqref{eq:contLSCStep1},  $I_{f,f'}^{\rr{\gamma}} (t,\psi(t,\xi))$ has length at most $2\iota' + \rr{2\gamma} $ for all $(t,\xi) \in \calT \times \calK$. Together with the absolute continuity of $\Q(\alpha(X_t) \in \cdot \ | \ \Xi(X_t))$, and choosing  $\iota' = \gamma = \frac{\delta}{4}$ this yields
\begin{equation}\label{eq:obs2}
    \sum_{t\in \calT} \Q(\{\phi_{k}(t,X_t) \in (\frakS_t(f) \triangle \frakS_t(f'))^{\rr{\gamma}} \}\cap \Omega_{\calK}) \le \sum_{t\in \calT}\rho_t(2\iota' + 2\gamma) = \rho(\iota).
\end{equation}
From \eqref{eq:obs1},\eqref{eq:obs2}, and  the rationale in the proof of  \cref{thm:unifcontV}, we conclude  that 
 $$|v(\tau_f)-v(\tau_{f'})|\le C\Q(\tau_f \ne \tau_{f'})^{1/2} \le C\left[\Q(\tilde{\Omega} \cap \Omega_{\calK}) + \delta\right]^{1/2} \le C\sqrt{\rho(\iota)+ \delta}.$$
\end{proof}


